SQuARM-SGD: Communication-Efficient Momentum SGD for Decentralized Optimization

In this paper, we propose and analyze SQuARM-SGD, a communication-efficient algorithm for decentralized training of large-scale machine learning models over a network. In SQuARM-SGD, each node performs a fixed number of local SGD steps using Nesterov's momentum and then sends sparsified and quantized updates to its neighbors regulated by a locally computable triggering criterion. We provide convergence guarantees of our algorithm for general (non-convex) and convex smooth objectives, which, to the best of our knowledge, is the first theoretical analysis for compressed decentralized SGD with momentum updates. We show that the convergence rate of SQuARM-SGD matches that of vanilla SGD. We empirically show that including momentum updates in SQuARM-SGD can lead to better test performance than the current state-of-the-art which does not consider momentum updates.

==> experiments_imagenet.tex <==

\allowdisplaybreaks
{

%--------------------------------------------------------------------
\TODO{Modify to exactly what we provide} In this section, we compare SQuARM-SGD with CHOCO-SGD
% \cite{koloskova_decentralized_2019-1,koloskova_decentralized_2019}
\cite{koloskova_decentralized_2019}
, which only employs compression (sparsification {\em or} quantization) and is the state-of-the-art in communication efficient decentralized training. We also provide additional plots for comparison of accuracy vs. wall-clock time and performance over other datasets in Appendix \ref{suppl_experiments}.
%{\bf Convex.}
%We run SQuARM-SGD on MNIST dataset and use multi-class cross-entropy loss to model the local objectives $f_i, i\in[n]$. We consider $n=60$ nodes connected in a ring topology, each processing a mini-batch size of 5 per iteration and having heterogeneous distribution of data across classes. We work with $\eta_t = 1/(t+100)$ (based on grid search) and synchronization index $H=5$. For SQuARM-SGD, we use the composed operator $SignTopK$ (\cite{basu_qsparse-local-sgd:_2019}) with $k=10$ (out of 7840 length vector for MNIST dataset)
%For our experiments, we set the triggering constant $c_0 = 5000$ in SQuARM-SGD (line 7) and keep it unchanged until a certain number of iterations and then increase it periodically;
%while still maintaining that $c_t \eta_t^2$ decreases with $t$ (as $c_t$ is  $o(t)$ ) .
%
%$\bullet$ {\bf Results.}
%In Figure \ref{fig:lo-cvx}, we observe SQuARM-SGD can reach a target test error in fewer communication rounds while converging at a rate similar to that of vanilla SGD. The advantage to SQuARM-SGD comes from the significant savings in the number of bits communicated to achieve a desired test error, as seen in Figure \ref{fig:te-logbits-cvx}: to achieve a test error of around 0.12, SQuARM-SGD gets 120$\times$ savings as compared to CHOCO-SGD with $Sign$ quantizer, around 10-15$\times$ savings than CHOCO-SGD with $TopK$ sparsifier, and around 1000$\times$ savings than vanilla decentralized SGD. We also provide a plot for using the composed $SignTopK$ operator without event-triggering titled `SQuARM-SGD (Sign-TopK)' for comparison.
%--------------------------------------------------------------------


%------------------------------------------------------------------
%%% ###EXPERIMENTS### (Original)
%\begin{figure*}[th]
%	\subfigure[] { \label{fig:lo-cvx} \includegraphics[width=0.24\textwidth]{cvx_testerr.png}} 
%	\subfigure[] { \label{fig:te-logbits-cvx} \includegraphics[width=0.24\textwidth]{cvx_testerr_logbits.png}} 
%	\subfigure[] { \label{fig:lo-noncvx} \includegraphics[width=0.24\textwidth]{noncvx_loss.png}} 
%	\subfigure[] { \label{fig:te-logbits-noncvx} \includegraphics[width=0.24\textwidth]{noncvx_tacc-logtotalbits.png}}
%	\caption{Figure \ref{fig:lo-cvx} and \ref{fig:te-logbits-cvx} are for convex objective and we plot test error vs number of communication rounds and test error vs total number of bits communicated, respectively, for different algorithms. Figure~\ref{fig:lo-noncvx} and \ref{fig:te-logbits-noncvx} are for non-convex objective where we plot training loss vs epochs and Top-1 accuracy vs total number of bits communicated, respectively.}
%	\label{fig:figures_cvx-noncvx}
%\end{figure*}

%%------------------------------------------------------------------
%% ###EXPERIMENTS 4 Figures###
%\begin{figure*}[th]
%	\centering
%	\subfigure[] { \label{fig:lo-noncvx} \includegraphics[width=0.23\textwidth]{imagenet_main_loss.png}}
%	\subfigure[] { \label{fig:lo-logbits-noncvx} \includegraphics[width=0.23\textwidth]{imagenet_main_loss-logtotalbits.png}}
%	\subfigure[] { \label{fig:te-noncvx} \includegraphics[width=0.23\textwidth]{imagenet_main_tacc.png}}
%	\subfigure[] { \label{fig:te-logbits-noncvx} \includegraphics[width=0.23\textwidth]{imagenet_main_tacc-logtotalbits.png}}
%	\caption{Figure~\ref{fig:lo-noncvx} and \ref{fig:te-logbits-noncvx} are for training of ResNet50 model on the ImageNet dataset where we plot training loss vs epochs and Top-1 accuracy vs total number of bits communicated, respectively.}
%	\label{fig:figures_cvx-noncvx}
%\end{figure*}
%%------------------------------------------------------------------

%%------------------------------------------------------------------
%% ###EXPERIMENTS 3 Figures###
\begin{figure*}[t]
	\centering
	\subfigure[] { \label{fig:lo-noncvx} \includegraphics[width=0.31\textwidth]{imagenet_main_loss.png}}
	\subfigure[] { \label{fig:lo-logbits-noncvx} \includegraphics[width=0.31\textwidth]{imagenet_main_loss-logtotalbits.png}}
	\subfigure[] { \label{fig:te-logbits-noncvx} \includegraphics[width=0.32\textwidth]{imagenet_main_tacc-logtotalbits.png}}
	\caption{\TODO{Add CONVEX EXPERIMENTS??} Figures~\ref{fig:lo-noncvx} and \ref{fig:lo-logbits-noncvx} correspond to the training loss for the ResNet50 model on the ImageNet dataset compared against no. of epochs and total communicated bits, respectively. Figure \ref{fig:te-logbits-noncvx} shows comparison for Top-1 test accuracy as function of total number of bits communicated.}
	\label{fig:figures_cvx-noncvx}
\end{figure*}
%%------------------------------------------------------------------




{\bf Setup.}
We compare our algorithm with CHOCO-SGD \cite{koloskova_decentralized_2019} on a large scale learning task of training ResNet50 \cite{he2015deep} model on ImageNet \cite{imagenet_cvpr09} dataset with $n=6$ nodes connected in a ring topology. Learning rate is initialized to $0.1$, following a schedule consisting of a warmup period of 5 epochs followed by piecewise decay of 5 at epochs 80,140, 170, and we stop training at epoch 200. The SGD algorithm is implemented with momentum with a factor of 0.9 and mini-batch size of 96. 
SQuARM-SGD consists of $H=5$ local iterations followed by checking for a triggering condition, and then communicating with the composed $SignTopK$ operator, % \cite{basu_qsparse-local-sgd:_2019}, 
where we take top 10\% elements of each tensor and only transmit the sign and norm of the result. The triggering threshold follows a schedule piecewise constant: initialized to 1.0 and increases by 0.25 after every 20 epochs till 100 epochs are complete; while maintaining that $c_t < \nicefrac{1}{\eta}$ for all $t$. We compare performance of SQuARM-SGD against CHOCO-SGD with $Sign$ and $TopK$ compression %(\cite{koloskova_decentralized_2019}) 
(taking top 10\% of elements of the tensor) and decentralized vanilla SGD. 
We also provide a plot for using the composed $SignTopK$ operator without event-triggering titled `SQuARM-SGD (Sign-TopK)' for comparison. 

{\bf Results.}
We plot global loss function evaluated at the average parameter vector across nodes vs.\ number of epochs in Figure \ref{fig:lo-noncvx}, where we observe SQuARM-SGD converging at a similar rate as CHOCO-SGD and vanilla decentralized SGD. Figure \ref{fig:lo-logbits-noncvx} shows the evolution of training loss as a function of number of bits, demonstrating that SQuARM-SGD uses significantly less bits than CHOCO-SGD or vanilla-SGD to train the model. Figure \ref{fig:te-logbits-noncvx} shows the performance for a given bit-budget, where we show the Top-1 test accuracy
% \footnote{Here, Top-1 accuracy corresponds to the percentage of test examples for which the correct label is equal to the label considered most probable by the model.} 
as a function of the total bits communicated. For Top-1 test accuracy of around $74.8\%$, SQuARM requires about $64 \times$ less bits than CHOCO with $Sign$ compression, about $190 \times$ less bits than CHOCO with $TopK$ compression, and around $2000 \times$ less bits than vanilla decentralized SGD to achieve the same Top-1 accuracy. 

\TODO{ADD CONVEX EXPERIMENTS???}


}

==> lemma_cvx_loc_global_err.tex <==
\allowdisplaybreaks
{

%\section{Proof of Lemma \ref{lem_cvx}} \label{proof_lem_dec_li_sgd}

%\begin{lemma*}[Restating Lemma \ref{lem_cvx}]
%	Let $ \{ \bx_t ^{(i)}  \}_{t=0}^{T-1} $ be generated according to Algorithm \ref{alg_dec_sgd_li} under assumptions of Theorem \ref{thm_cvx_li} with stepsize $\eta_t := \frac{b}{(a+t)}$ (where $a \geq \frac{5H}{p}, \, b > 0$), an increasing threshold fucntion $c_t \sim {o}(t)$ and define $\bar{\bx}_t = \frac{1}{n} \sum_{i=1}^{n} x_t^{(i)} $.
%	Consider the set of synchronization indices $\mathcal{I}_T$ =  $\{ I_{(1)},I_{(2)}, \hdots, I_{(t)}, \hdots  \}$. Then for any $I_{(t)} \in \mathcal{I}_T$, we have:
%	\begin{align*}
%	\mathbb{E}\sum_{j=1}^n \left\Vert \bar{\bx}^{I_{(t)}} - \bx^{I_{(t)}}_{j} \right\Vert^2 = \mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2  \leq \frac{20nA_{I_{(t)}}  \eta_{I_{(t)}}^2}{p^2},
%	\end{align*}
%where $A_{I_{(t)}}=\frac{pH}{2}\left(  8 H^2 G^2 \left( 1 + \frac{9\beta}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega Hc_{I_{(t)}} \right) $, where $p = \frac{\delta \gamma}{8} $, $\delta = 1 - | \lambda_2(\mathbf{W})|$, $\omega$ is compression parameter for operator $\C$, and $c_{I_{(t)}}$ and $\eta_{I_{(t)}}$ are respectively the triggering threshold and learning rate at time step $I_{(t)}$.
%\end{lemma*}
 \TODO{We use some techniques from [Lemma 17]\cite{koloskova_decentralized_2019-1} to prove Lemma \ref{lem_cvx_e1} and [Lemma 18]\cite{koloskova_decentralized_2019-1} to prove Lemma \ref{lem_cvx_e2}.}
%Note that \cite{koloskova_decentralized_2019-1} only analyze compression in decentralized SGD; whereas, in addition, we also incorporate local iterations and event-triggered communication, and analyze decentralized SGD with Nesterov momentum acceleration. These additional factors significantly complicate the proof of Lemma \ref{lem_cvx}. Observe that event-triggered communication inherently makes our algorithm asynchronous, because some workers may not send messages while others send. Note that \cite{koloskova_decentralized_2019-1} (see also \cite{koloskova_decentralized_2019}) incorporated momentum in their experiments, but left the theoretical analysis open. As far as we know, this is the first paper that not only incorporate momentum in their algorithm, but also incorporate local iterations and event-triggered communication to further save on communication, and theoretically analyze the final algorithm.

Now we give a proof sketch of Lemma \ref{lem_cvx}, which states that 
$e_{I_{(t)}}^{(1)}:=\sum_{j=1}^n \mathbb{E} \left\Vert \bar{\bx}^{I_{(t)}} - \bx^{I_{(t)}}_{j} \right\Vert^2$ 
-- the difference between the local and the average iterates at the synchronization indices -- 
decays asymptotically to zero for decaying learning rate $\eta_t$.
We show this by setting up a contracting recursion for $e_{I_{(t)}}^{(1)}$. First we prove that 
\begin{align}
e_{I_{(t+1)}}^{(1)} \leq (1-\alpha_1)e_{I_{(t)}}^{(1)} + (1-\alpha_1)e_{I_{(t)}}^{(2)} + c_1\eta_{I_{(t)}}^2, \label{eq:dec_avg_local-interim1}
\end{align}
where $e_{I_{(t)}}^{(2)}:=\sum_{j=1}^n \mathbb{E} \left\Vert \hat{\bx}^{I_{(t+1)}} - \bx^{I_{(t)}}_{j} \right\Vert^2$, $\alpha_1\in(0,1)$, and $c_1$ is a constant that depends on $n,\delta,\beta,H,G$. 
Note that \eqref{eq:dec_avg_local-interim1} gives a contracting recursion in $e_{I_{(t)}}^{(1)}$, but it also gives the other term $e_{I_{(t)}}^{(2)}$, which we have to bound. 
It turns out that we can prove a similar inequality for $e_{I_{(t)}}^{(2)}$ as well:
\begin{align}
e_{I_{(t+1)}}^{(2)} \leq (1-\alpha_2)e_{I_{(t)}}^{(1)} + (1-\alpha_2)e_{I_{(t)}}^{(2)} + c_2(t)\eta_{I_{(t)}}^2, \label{eq:dec_avg_local-interim2}
\end{align}
where $\alpha_2\in(0,1)$; furthermore, we can choose $\alpha_1,\alpha_2$ such that $\alpha_1+\alpha_2 > 1$.
In \eqref{eq:dec_avg_local-interim2}, $c_2(t)$, in addition to $n,\delta,\beta,H,G$, also depends on the compression factor $\omega$ and  $c_t$ which is the triggering threshold at timestep $t$.


Define $e_{I_{(t)}}:=e_{I_{(t)}}^{(1)} + e_{I_{(t)}}^{(2)}$. Adding \eqref{eq:dec_avg_local-interim1} and \eqref{eq:dec_avg_local-interim2} gives the following recursion with $\alpha\in(0,1)$:
\begin{align}
e_{I_{(t+1)}} \leq (1-\alpha)e_{I_{(t)}} + c_3(t)\eta_{I_{(t)}}^2. \label{eq:dec_avg_local-interim3}
\end{align}
From \eqref{eq:dec_avg_local-interim3}, we can show that $e_{I_{(t)}}\leq c(t)\eta_{I_{(t)}}^2$ for some $c(t)$ that depends on $n,\delta,\beta,H,G,\omega,c_t$. Lemma \ref{lem_cvx} follows from this because $\sum_{j=1}^n \mathbb{E} \left\Vert \bar{\bx}^{I_{(t)}} - \bx^{I_{(t)}}_{j} \right\Vert^2 = e_{I_{(t)}}^{(1)} \leq e_{I_{(t)}}$.

Now we establish the above-mentioned recursion on $e^{(1)}_{I_{(t+1)}}$ and $e^{(2)}_{I_{(t+1)}}$ in Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2}, respectively, and then using that we prove Lemma \ref{lem_cvx}.

\iffalse
Our proof of Lemma \ref{lem_cvx} involves analyzing the following expression:
\begin{align*}
e_{I_{(t+1)}} := \underbrace{\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2}_{e^{(1)}_{I_{(t+1)}}} + \underbrace{ \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}} \Vert_F^2}_{e^{(2)}_{I_{(t+1)}}}
\end{align*}
The first term $e^{(1)}_{I_{(t+1)}}$ in RHS above captures the deviation of local parameters of the nodes from the global average parameter. The second term $e^{(2)}_{I_{(t+1)}}$ captures the deviation of the node parameters from their estimates that other nodes have. In the section for Proof Outlines \ref{proof-outlines}, we proposed the idea of writing a bound for 
$e^{(1)}_{I_{(t+1)}}$ (and $e^{(2)}_{I_{(t+1)}}$) in terms of $e^{(1)}_{I_{(t)}}$ (and $e^{(2)}_{I_{(t)}}$), enabling us to write a recursive expression which could then be translated to a recursive expression for the sum $e_{I_{(t+1)}}$ in terms of $e_{I_{(t)}}$. 
\fi
\iffalse
We follow a different approach here, where we bound $e^{(1)}_{I_{(t+1)}}$ and $e^{(2)}_{I_{(t+1)}}$ individually in terms of parameters evaluated at the auxillary index $I_{(t+\frac{1}{2})}$. These bounds are provided in Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} below. These individual bounds are then added to yield a bound for the sum $e_{I_{(t+1)}}$ in terms of parameters evaluated at the auxillary index $I_{(t+\frac{1}{2})}$. 
Further simplification allows us to bound $e_{I_{(t+1)}}$ in terms of $e_{I_{(t)}}$, thus giving a recursive form.
%We first provide two lemmas which enable us to write recursive expressions for $e^{(1)}_{I_{(t+1)}}$ and $e^{(2)}_{I_{(t+1)}}$ (Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} respectively) and thus $e_{I_{(t+1)}}$.
This recursion enables us to bound $e_{I_{(t+1)}}$ as $e_{I_{(t+1)}} \leq \frac{20A_{I_{(t+1)}}}{p^2} \eta_{I_{(t+1)}}^2$ where $A_{I_{(t+1)}}$ is defined in the statement of Lemma \ref{lem_cvx}. Thus, the quantity of interest $e^{(1)}_{I_{(t+1)}} = \mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 $ is also bounded by $\frac{20A_{I_{(t+1)}}}{p^2} \eta_{I_{(t+1)}}^2$, proving Lemma \ref{lem_cvx}. \\
We first state and prove bounds on $e^{(1)}_{I_{(t+1)}}$ and $e^{(2)}_{I_{(t+1)}}$ in terms of parameters evaluated at the auxillary index $I_{(t+\frac{1}{2})}$ in Lemma \ref{lem_cvx_e1} and \ref{lem_cvx_e2} respectively. Using these bounds, we then proceed to prove Lemma \ref{lem_cvx}. \\
\fi
\TODO{\begin{lemma} \label{lem_cvx_e1}
Consider the sequence of updates in Algorithm \ref{alg_dec_sgd_li} in matrix form (refer \ref{mat_not_li} for the matrix form of Algorithm \ref{alg_dec_sgd_li}). The expected deviation between the local node parameters $\bX^{I_{(t+1)}}$ and the global average parameters $\Bar{\bX}^{I_{(t+1)}}$ evaluated at some $I_{(t+1)} \in \mathcal{I}_T$ satisfies:
\begin{align*}
	e^{(1)}_{I_{(t+1)}} := \mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq  (1+\alpha_5^{-1})R_1 \mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2  + (1+\alpha_5^{-1}) R_2 \mathbb{E} \Vert  {\bX}^{I_{(t)}}-\hat{\bX}^{I_{(t+1)}}\Vert_F^2 + Q_1\eta_{I_{(t+1)}}^2
\end{align*}
where $R_1=(1+\alpha_1)(1-\gamma \delta)^2 , R_2=(1+\alpha_1^{-1}) \gamma^2 \lambda^2 $ and $Q_1 = 8 H^2 n G^2 \left(1 + \frac{9\beta^2}{(1- \beta)^4} \right)(1+\alpha_5)(R_1+R_2) $. Here $\alpha_1, \alpha_5 >0$, $\delta$ is the spectral gap, $H$ is the synchronization gap, $\gamma$ is the consensus stepsize, and $\lambda := \verts{\mathbf{W}-\mathbf{I}}_2$ where $\mathbf{W}$ is a doubly stochastic mixing matrix. 
\end{lemma} }
\begin{proof}

	Using the definition of $\bX^{I_{(t+1)}}$ from Section \ref{mat_not_sec}, we have:
	\begin{align}
	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & = \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+1)}} + \gamma \hat{\bX}^{I_{(t+1)}} (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag 
	\intertext{Noting that $\Bar{\bX}^{I_{(t+1)}} = \Bar{\bX}^{I_{(t+\frac{1}{2})}} $ from (\ref{mean_seq_iter}) and $\Bar{\bX}^{I_{(t+\frac{1}{2})}} (\mathbf{W}-\mathbf{I})= 0$ from (\ref{mean_prop}), we get: }
	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & = 
	% 	\Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} + \gamma ( {\bX}^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} )  (\mathbf{W}-\mathbf{I})+ \gamma (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}}) (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag \\
	% 	& =
	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})+ \gamma (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}}) (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag
	\intertext{Using the fact $\Vert \mathbf{A} + \mathbf{B} \Vert_F^2 \leq (1+\alpha_1)\Vert \mathbf{A}\Vert_F^2 + (1+\alpha_1^{-1})\Vert \mathbf{B} \Vert_F^2$ for any $\alpha_1 >0$, }
	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq (1+\alpha_1)\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F^2 \notag \\
	& \qquad + (1+\alpha_1^{-1}) \Vert \gamma (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}}) (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag \\
	\intertext{Using $\Vert \mathbf{A} \mathbf{B} \Vert_F \leq \Vert \mathbf{A} \Vert_F \Vert \mathbf{B} \Vert_2 $ as per (\ref{bound_frob_mult}), we have: }
	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 &  \leq (1+\alpha_1)\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F^2 \notag \\
	& \qquad + (1+\alpha_1^{-1}) \gamma^2 \Vert  (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}})\Vert_F^2 .\Vert(\mathbf{W}-\mathbf{I})\Vert_2^2 \label{suppl_cvx_li_temp_eqn}
	\end{align}
	To bound the first term in (\ref{suppl_cvx_li_temp_eqn}), we use the triangle inequality for Frobenius norm, giving us:
	\begin{align*}
	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F & \leq (1-\gamma)\Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F+ \gamma \Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} )W\Vert_F
	\end{align*}
	{It follows from \eqref{mean_prop} that $\left(\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}}\right)\frac{\mathbbm{1}\mathbbm{1}^T}{n} = \bzero$. Adding this inside the last term above, we get: }
	\begin{align*}
	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F & \leq (1-\gamma)\Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F  + \gamma \left\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})\left (\mathbf{W} - \frac{\mathbbm{1}\mathbbm{1}^T}{n} \right) \right\Vert_F 
	\end{align*}
	{Using $\Vert \mathbf{A} \mathbf{B} \Vert_F \leq \Vert \mathbf{A} \Vert_F \Vert \mathbf{B} \Vert_2 $ as per (\ref{bound_frob_mult}) and then using (\ref{bound_W_mat}) with $k=1$, we can simplify the above to: }
	\begin{align*}
	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F \leq (1-\gamma \delta) \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F
	\end{align*}
	Substituting the above in (\ref{suppl_cvx_li_temp_eqn}) and using $\lambda = \text{max}_i \{ 1- \lambda_i(\mathbf{W}) \} \Rightarrow \Vert \mathbf{W}-\mathbf{I} \Vert_2^2 \leq \lambda^2 $, we get: 
	\begin{align*}
	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 \leq (1+\alpha_1)(1-\gamma \delta)^2  \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 + (1+\alpha_1^{-1}) \gamma^2 \lambda^2 \Vert  {\bX}^{I_{(t+\frac{1}{2})}}-\hat{\bX}^{I_{(t+1)}}\Vert_F^2
	\end{align*}
	Taking expectation w.r.t.\ the entire process, we have:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq (1+\alpha_1)(1-\gamma \delta)^2 \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 + (1+\alpha_1^{-1}) \gamma^2 \lambda^2 \mathbb{E} \Vert  {\bX}^{I_{(t+\frac{1}{2})}}-\hat{\bX}^{I_{(t+1)}}\Vert_F^2
	\end{align*}
	Define $R_1=(1+\alpha_1)(1-\gamma \delta)^2 , R_2=(1+\alpha_1^{-1}) \gamma^2 \lambda^2 $.
	Using the update algorithm, we have:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq R_1 \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} -  \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta_{t'} ( \beta \bV^{(t')} +  \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right) \right\Vert_F^2 \notag \\
	& \qquad + R_2 \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} + \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta_{t'} ( \beta \bV^{(t')} + \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2
	\end{align*} 	
	Thus, for any $\alpha_5 > 0 $, we have:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq R_1 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_2 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
	 & \qquad + R_1(1+\alpha_5)  \mathbb{E} \left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta_{t'} ( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{{\bf 1}{\bf 1}^T}{n} - I \right) \right\Vert_F^2 \notag \\
	 & \qquad + R_2 (1+\alpha_5) \mathbb{E} \left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta_{t'} ( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2
	\end{align*}
	Using $\verts{AB}_F \leq \verts{A}_F \verts{B}_2$ as per \eqref{bound_frob_mult} to split the third term, and then using the bound $\left\| \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right\|_2 =1$ (which is shown in Claim \ref{J-I_eigenvalue} below), and further using the bound in (\ref{bound_gap_grad}) for the third and fourth term, the above can be rewritten as:  
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq R_1 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_2 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
	& \qquad + 2\eta_{I_{(t)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\alpha_5)(R_1+R_2)
	\end{align*}
	Noting that $\eta_{I_{(t)}} \leq 2 \eta_{I_{(t+1)}}$\footnote{\label{ratio_eta}$\frac{\eta_{I_{(t)}}}{\eta_{I_{(t+1)}}} = \frac{I_{(t+1)} + a}{I_{(t)} + a} \leq \frac{I_{(t)} + H + a}{I_{(t)} + a} = 1 + \frac{H}{I_{(t)} + a} \leq 1 + \frac{H}{a} \leq 2$. The last inequality follows from that $a\geq \frac{5H}{p} \geq H$.} and defining $Q_1 = 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\alpha_5)(R_1+R_2) $ completes the proof of Lemma \ref{lem_cvx_e1}.
\end{proof}
%-----------------------------------------------------------------
\begin{claim}\label{J-I_eigenvalue}
For any $n\in\mathbb{N}$, we have $\left\| \frac{{\bf 1}{\bf 1}^T}{n} - I \right\|_2 = 1$ where ${\bf 1} = [ 1 \, 1 \hdots 1]^T_{1 \times n} $
\end{claim}
\begin{proof}
%\TODO{\bf FILL IN HERE...}
Note that $ \frac{{\bf 1}{\bf 1}^T}{n} $ is a symmetric doubly stochastic matrix with eigenvalues 1 and 0 (with algebraic multiplicity $n-1$). Thus, it has the eigen-decomposition $ \frac{{\bf 1}{\bf 1}^T}{n} = U D U^T  $ where columns of $U$ are orthogonal and D = $diag( [ 1 \, 0 \hdots 0]  )$, which gives us:
\begin{align*}
	\left\| \frac{{\bf 1}{\bf 1}^T}{n} - I \right\|_2 = \left\| UDU^T - UU^T  \right\|_2 = \left\| D-I \right\|_2=
	\left\|
	\begin{bmatrix}
		1 & 0 & \hdots  & 0 \\
		0 & 0 & \hdots & 0 \\
		\vdots & \vdots & \ddots & 0 \\
		0 & 0 & \hdots & 0 
	\end{bmatrix}
	 - 
	 \begin{bmatrix}
	 1 & 0 & \hdots  & 0 \\
	 0 & 1 & \hdots & 0 \\
	 \vdots & \vdots & \ddots & 0 \\
	 0 & 0 & \hdots & 1 
	 \end{bmatrix} \right\|_2 = 1
\end{align*}
\end{proof}
%-----------------------------------------------------------------
\begin{lemma}\label{lem_cvx_e2}
	Consider the sequence of updates in Algorithm \ref{alg_dec_sgd_li} in matrix form (refer \ref{mat_not_li}) with the threshold sequence $ \{  c_t \}_{t=0}^{T-1} $ such that $c_t =o(t)$, and decaying learning rate $\eta_t=\frac{b}{(a+t)}$, for some $b>0$. The expected deviation between the local node parameters $\bX^{I_{(t+1)}}$ and their estimates $\hat{\bX}^{I_{(t+2)}}$ at a synchronization time step $I_{(t+1)}$ satisfy:
	\begin{align*}
	e^{(2)}_{I_{(t+1)}} =	\mathbb{E} \Vert \bX^{I_{(t+1)}} -\hat{\bX}^{I_{(t+2)}}\Vert_F^2	 & \leq (1+\alpha_5^{-1}) R_3 \mathbb{E} \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}}\Vert_F^2 + (1+\alpha_5^{-1}) R_4 \mathbb{E} \Vert \bX^{I_{(t)}}- \Bar{\bX}^{I_{(t)}} \Vert_F^2  +  \eta_{I_{(t+1)}}^2Q_2,
	\end{align*}
	where $R_3 = (1+\gamma \lambda )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)$ , $R_4 = \gamma^2 \lambda^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) $ and $Q_2 = 8H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)((1+\alpha_5)(R_3+R_4)+( 1+\alpha_2^{-1}) + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega)) + (1+\alpha_2)\omega n c_{I_{(t+1)}}  $. Note that $Q_2$ depends on $t$ (as captured by $c_{I_{(t)}}$ in the expression) as we allow for our triggering threshold to change with time.  Here $\alpha_2, \alpha_3, \alpha_4 >0, \alpha_5 >0$  are the same as used in Lemma \ref{lem_cvx_e1}, $\delta$ is the spectral gap, $H$ is the synchronization gap, $\gamma$ is the consensus stepsize, and $\lambda = \verts{\mathbf{W}-\mathbf{I}}_2$ where $\mathbf{W}$ is a doubly stochastic mixing matrix.
\end{lemma} 
\begin{proof}
Note that $\hat{\bX}^{I_{(t+2)}} = \hat{\bX}^{I_{(t+1)}} + \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )$; see Section \ref{mat_not_sec}.
Substituting this in $\mathbb{E} \Vert \bX^{I_{(t+1)}} -\hat{\bX}^{I_{(t+2)}}\Vert_F^2$, we get:
	\begin{align*}
	& \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2  = \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 
	\intertext{Adding and subtracting $\bX^{I_{(t+\frac{3}{2})}}$ and rearranging terms, we get}
	&  \hspace{2.4cm} = \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}+ \bX^{I_{(t+1)}} - \bX^{I_{(t+\frac{3}{2})}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 
	\end{align*}
	Using $\Vert \mathbf{A} + \mathbf{B} \Vert_F^2 \leq (1+\alpha_2)\Vert \mathbf{A}\Vert_F^2 + (1+\alpha_2^{-1})\Vert \mathbf{B} \Vert_F^2$ for any $\alpha_2 >0$,
	\begin{align}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 & \leq (1+\alpha_2) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}}- \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 \notag \\
	&\hspace{1cm} + (1+\alpha_2^{-1})\mathbb{E}\Vert \bX^{I_{(t+1)}} - \bX^{I_{(t+\frac{3}{2})}} \Vert_F^2 \notag \\
	& = (1+\alpha_2) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 \notag \\
	& \hspace{1cm} + (1+\alpha_2^{-1})\mathbb{E}\left\Vert \sum_{t' = I_{(t+1)}}^{I_{(t+2)}-1} \eta_{t'} ( \beta \bV^{(t')} +  \partial F (\bX^{t'}, \xi^{t'})) \right\Vert_F^2 \label{cvx_lem1_interim1}
	\end{align}
	Bounding the last term in \eqref{cvx_lem1_interim1} using (\ref{bound_gap_grad}), we get:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 & \leq (1+\alpha_2) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 \\
	& \qquad + (1+\alpha_2^{-1}) 2\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)
	\end{align*}
Note that both $\mathbf{P}^{(I_{(t+2)}-1)} $ and $\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)} $ are diagonal matrices, with disjoint support on the diagonal entries, which implies that $\mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}\|_F^2 = \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})\mathbf{P}^{(I_{(t+2)}-1)}\|_F^2 + \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})({\bf I} - \mathbf{P}^{(I_{(t+2)}-1)})\|_F^2$. We get:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - & \hat{\bX}^{I_{(t+2)}}\Vert_F^2  \leq  (1+\alpha_2)  \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})\mathbf{P}^{(I_{(t+2)}-1)} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2  \\
	&   + (1+\alpha_2) \mathbb{E}\Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2  + 2 (1+\alpha_2^{-1}) \eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)
	\end{align*}
	Using the compression property of operator $\C$ as per (\ref{bound_comp}), we have:
	\begin{align*}
	& \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \leq (1+\alpha_2) (1-\omega) \mathbb{E}  \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})\mathbf{P}^{(I_{(t+2)}-1)} \Vert_F^2 \\
	& \hspace{1cm} +  (1+\alpha_2) \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2  + 2 (1+\alpha_2^{-1}) \eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)
	\end{align*}
	Adding and subtracting $ (1+\alpha_2)(1-\omega)  \mathbb{E}\Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2$, we get:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 & \leq (1+\alpha_2) (1-\omega)  \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2  + (1+\alpha_2^{-1})2\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)  \\
	& \qquad \qquad +(1+\alpha_2) \omega  \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2 
	\end{align*}
To bound the third term in the RHS above, note that $\hat{\bX}^{I_{(t+2)}-1} = \hat{\bX}^{I_{(t+1)}}$, because $\hat{\bX}$ does not change in between the synchronization indices,
which implies that $\mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2 = \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+2)}-1})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2$, which we can upper-bound using \eqref{bound_trig} by $nc_{I_{(t+2)}-1}\eta_{I_{(t+2)}-1}^2$. 
From Claim \ref{c_t-eta_bound} stated below, it follows that $c_{I_{(t+2)}-1}\eta_{I_{(t+2)}-1}^2 \leq H c_{I_{(t+1)}}\eta_{I_{(t+1)}}^2$. 
 Substituting this in the above gives:
	\begin{align} \label{cvx_lemm_interim2}
	\mathbb{E}& \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \notag \\
	& \leq (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 +(1+\alpha_2)\omega nH c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2 \notag \\
	& \qquad + (1+\alpha_2^{-1}) 2\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)\notag \\
	& = (1+\alpha_2) (1-\omega) \mathbb{E} \left\Vert \bX^{I_{(t+1)}}  - \sum_{t' = I_{(t+1)}}^{I_{(t+2)}-1}\eta_{t'} (\beta \bV^{(t')}+  \partial F (\bX^{t'}, \xi^{t'})) -  \hat{\bX}^{I_{(t+1)}} \right\Vert_F^2  \notag \\
	& \qquad + (1+\alpha_2^{-1}) 2\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) + (1+\alpha_2)\omega n H c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2 \notag \\
	& \leq (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+1)}}  -  \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + (1+\alpha_2^{-1}) 2\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \notag \\
	& \hspace{0.4cm} + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \mathbb{E} \left\Vert \sum_{t' = I_{(t+1)}}^{I_{(t+2)}-1}\eta_{t'} ( \beta V^{(t')} +  \partial F (\bX^{t'}, \xi^{t'})) \right\Vert_F^2 + (1+\alpha_2)\omega nH c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2
	\end{align}
	where in the last inequaility, we have used (\ref{bound_l2_sum}) and $\alpha_3 > 0$. Using (\ref{bound_gap_grad}) to bound the penultimate term in \eqref{cvx_lemm_interim2}, we get:
	\begin{align*}
	\mathbb{E} & \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \\
	& \leq (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+1)}}  -  \hat{\bX}^{I_{(t+1)}} \Vert_F^2 \\
	& \qquad +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) 2\eta_{I_{(t+1)}} ^2H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \\
	& \qquad + (1+\alpha_2)\omega n H c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2  + (1+\alpha_2^{-1}) 2\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \\
	& = (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} + \gamma \hat{\bX}^{I_{(t+1)}} (\mathbf{W}-\mathbf{I}) -  \hat{\bX}^{I_{(t+1)}} \Vert_F^2 \\
	& \qquad +  2(1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega)\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)\\
	& \qquad  + (1+\alpha_2)\omega n H c_{I_{(t+1)}}\eta_{I_{(t+1)}} ^2 + 2(1+\alpha_2^{-1}) \eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \\
	& \leq (1+\alpha_3) (1+\alpha_2) (1-\omega)\mathbb{E} \Vert (\bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}})((1+\gamma)\mathbf{I} - \gamma \mathbf{W})+ \gamma (\bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}})(\mathbf{W}-\mathbf{I})\Vert_F^2 \\
	& \qquad +  2(1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \\
	& \qquad + (1+\alpha_2)\omega nH c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2 + 2(1+\alpha_2^{-1}) \eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)
	\end{align*}
	where in the last inequality we've used $ \Bar{\bX}^{I_{(t+\frac{1}{2})}} (\mathbf{W}-\mathbf{I})= 0 $. For $\alpha_4 > 0 $, using (\ref{bound_l2_sum}) gives us:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert (\bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}})((1+\gamma)\mathbf{I} - \gamma \mathbf{W})\Vert_F^2 \\
	& \hspace{0.5cm} + (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \gamma (\bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}})(\mathbf{W}-\mathbf{I})\Vert_F^2 \\
	& \hspace{0.5cm} +  2(1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)  \\
	& \hspace{0.5cm} + 2(1+\alpha_2^{-1}) \eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)+ (1+\alpha_2)\omega n H c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2
	\end{align*}
	Using $\Vert (1+\gamma)\mathbf{I} - \gamma W \Vert_2 = \Vert I + \gamma (\mathbf{I} - \mathbf{W})\Vert_2 = 1 +  \gamma \Vert \mathbf{I} - \mathbf{W} \Vert_2  = 1 + \gamma \lambda $ (by definition of $\lambda = \text{max}_i \{ 1- \lambda_i(\mathbf{W}) \}$) and $\verts{\mathbf{I} - \mathbf{W}}_2 = \lambda$  along with $\verts{\mathbf{AB}}_F \leq \verts{\mathbf{A}}_F\verts{\mathbf{B}}_2$ from (\ref{bound_frob_mult}):
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq (1+\gamma \lambda )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)\mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}}\Vert_F^2 \notag \\
	& \qquad + \gamma^2 \lambda^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 \notag \\
	& \qquad +2\left(  ( 1+\alpha_2^{-1}) + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \right)\eta_{I_{(t+1)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \\
	& \qquad  + (1+\alpha_2)\omega nH c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2
	\end{align*}
	Define $R_3 = (1+\gamma \lambda )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)$ , $R_4 = \gamma^2 \lambda^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) $ and $R_5 = 2\left(  ( 1+\alpha_2^{-1}) + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \right) H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) + (1+\alpha_2)\omega n H c_{I_{(t+1)}}  $, then the above can be rewritten as :
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq R_3 \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}}\Vert_F^2  + R_4 \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 +  R_5\eta_{I_{(t+1)}} ^2
	\end{align*}
	Using the update rule, this can be expanded as :
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - & \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \leq R_3 \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} + \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta_{t'} ( \beta \bV^{(t')} +    \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2 \notag \\
	& + R_4 \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} -  \sum_{t' = I_{(t)}}^{I_{(t+1)}-1}\eta_{t'} ( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{{\bf 1}{\bf 1}^T}{n} - I \right) \right\Vert_F^2  +  R_5\eta_{I_{(t+1)}} ^2
	\end{align*}
For the same $\alpha_5>0$ as used in Lemma \ref{lem_cvx_e1}, we get:
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq R_3 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 + R_4 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
	& \qquad  + R_4 (1+\alpha_5) \mathbb{E}\left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta_{t'} ( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{{\bf 1}{\bf 1}^T}{n} - I \right) \right\Vert_F^2  \notag \\
	& \qquad + R_3 (1+\alpha_5)\mathbb{E} \left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1}\eta_{t'} ( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2  +  R_5\eta_{I_{(t+1)}} ^2
\end{align*}	
Using $\verts{AB}_F \leq \verts{A}_F \verts{B}_2$ as per \eqref{bound_frob_mult} to split the third term and then using $\left\| \frac{{\bf 1}{\bf 1}^T}{n} - I \right\| \leq 1$ (from Claim \ref{J-I_eigenvalue}), and further using the bound in (\ref{bound_gap_grad}) for the third and fourth term, the above can be rewritten as:  
	\begin{align*}
	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+2)}} \Vert_F^2 & \leq R_3 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 + R_4 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
	& \qquad + 2\eta_{I_{(t)}} ^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\alpha_5)(R_3+R_4) + R_5\eta_{I_{(t+1)}} ^2
	\end{align*}
	Noting that  $ \eta_{I_{(t)}} \leq 2 \eta_{I_{(t+1)}} $ (see Footnote \ref{ratio_eta}) and defining $Q_2 = 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\alpha_5)(R_3+R_4) + R_5 $ completes the proof of Lemma \ref{lem_cvx_e2}.	
\end{proof}


Having established the bounds on $e_{I_{(t+1)}}^{(1)}$ and $e_{I_{(t+1)}}^{(2)}$, we are now ready to prove Lemma \ref{lem_cvx}.
\begin{proof} [Proof of Lemma \ref{lem_cvx}]
	Consider the following expression:
	\begin{align} \label{suppl_et_eqn_li}
	e_{I_{(t+1)}} = \underbrace{\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2}_{e^{(1)}_{I_{(t+1)}}} + \underbrace{ \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}} \Vert_F^2}_{e^{(2)}_{I_{(t+1)}}}
	\end{align}
	We note that Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} provide bounds for the first and the second term in the RHS of (\ref{suppl_et_eqn_li}). Substituting them in (\ref{suppl_et_eqn_li}) gives:
	\begin{align} \label{suppl_et_eqn_total_li}
	&e_{I_{(t+1)}}  %&= \mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 + \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}} \Vert_F^2 \notag \\ 
	 \leq  R_1 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_2 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
	& \hspace{0.3cm}  + R_4 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_3 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 + (Q_1 + Q_2)\eta_{I_{(t+1)}} ^2
	\end{align}	
	Define the following:
	\begin{align}
	\pi_1 (\gamma) & := R_2 + R_3 = \gamma^2 \lambda^2 (1+\alpha_1^{-1}) + (1+\gamma \lambda )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \label{cvx_pi1}   \\
	\pi_2 (\gamma) & := R_1 + R_4 = (1-\delta \gamma)^2(1+\alpha_1) + \gamma^2 \lambda^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \label{cvx_pi2} \\
	\pi_{t} & := Q_1 + Q_2 \leq 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\alpha_5)(R_1 + R_2 +R_3+R_4) \notag \\
	& + 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)((1+\alpha_2^{-1}) + (1-\omega)(1+\alpha_3^{-1})(1+\alpha_2) ) + (1+\alpha_2)\omega n H c_{t} \label{cvx_pi3}
	\end{align}
	The bound on $e_{I_{(t+1)}}$ in (\ref{suppl_et_eqn_total_li}) can be rewritten as:
	\begin{align} \label{lemm_mom_cvx_interim}
	&e_{I_{(t+1)}} \leq (1+\alpha_5^{-1}) \left[\pi_1 (\gamma) \mathbb{E} \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \pi_2 (\gamma) \mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2\right] + \pi_{I_{(t+1)}} \eta_{I_{(t+1)}}^2 \notag \\
	&\quad \leq (1+\alpha_5^{-1}) max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \} \, \mathbb{E} \left[ \Vert {\bX}^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 \right] + \pi_{I_{(t+1)}}  \eta_{I_{(t+1)}} ^2
	\end{align}
	Calculation of $ max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \}$ and $\pi_{I_{(t)}}$ is given in Lemma \ref{suppl_lem_coeff_calc}, where we show that:\\
	$ max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \} \leq   \left(  1 - \frac{\gamma^* \delta}{8}  \right)   \leq \left( 1 - \frac{\delta^2 \omega}{644} \right)  $ and $\pi_t \leq \left(  8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega n H c_{t} \right) $ where $p:= \frac{\gamma^* \delta}{8} $. Here $\alpha_5 := \frac{2}{p}$. Here $\gamma^* = \frac{2 \delta \omega}{64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega}$ from Lemma \ref{suppl_lem_coeff_calc} is the consensus step-size. Substituting these bounds in \eqref{lemm_mom_cvx_interim} gives us:
	\begin{align*}
	e_{I_{(t+1)}} & \leq (1+\frac{p}{2}) \left( 1 - \frac{\delta \gamma^*}{8} \right)\mathbb{E}  \left[ \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2 \right] \\ 
	& \qquad + \left(  8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega n H c_{I_{(t+1)}} \right) \eta_{I_{(t+1)}} ^2
	\end{align*}
	where $p = \frac{\delta \gamma^*}{8}$. From definition of $e_{I_{(t)}} = \mathbb{E} \left[ \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2 + \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 \right] $ and we define $z_t :=\left(  8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega nH c_{t} \right) $. Since $c_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2 \leq H c_{I_{(t)}} \eta_{I_{(t)}}^2 $  (see Claim \ref{c_t-eta_bound}) and $\eta_{I_{(t+1)}} \leq \eta_{I_{(t)}}$, we have that $z_{I_{(t+1)}} \eta_{I_{(t+1)}} ^2 \leq H z_{I_{(t)}} \eta_{I_{(t)}}^2 $. Thus we have the following recurrence relation for $e_{I_{(t)}}$:
	\begin{align*}
	e_{I_{(t+1)}} \leq(1+\frac{p}{2}) (1-p) e_{I_{(t)}}  + H z_{I_{(t)}} \eta_{I_{(t)}}^2
	\end{align*}
	Define $A_t := \frac{p H z_t}{2n}$. Thus we have the following relation:
	\begin{align}  \label{suppl_lemm_rec_rel_li}
	e_{I_{(t+1)}} \leq \left( 1-\frac{p}{2} \right)e_{I_{(t)}} + \frac{2nA_{I_{(t)}}}{p}\eta_{I_{(t)}}^2.
	\end{align} 
We can now use Lemma \eqref{suppl_lem_e_seq_li} to bound the sequence $e_{I_{(t)}}$ for all $t$ as:
\begin{align*}
	e_{I_{(t)}} \leq \frac{20}{p^2}nA_{I_{(t)}}\eta_{I_{(t)}}^2
\end{align*}
	Note that we also have: $ \mathbb{E}\Vert\Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}}\Vert_F^2 \leq \mathbb{E} \left[ \Vert\Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}}\Vert_F^2  + \Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \Vert_F^2 \right] =: e_{I_{(t)}}$. Thus, we get the following result for any synchronization index $I_{(t)} \in \mathcal{I}_T$:
	\begin{align*}
	\mathbb{E}\Vert\Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}}\Vert_F^2 \leq \frac{20}{p^2}nA_{I_{(t)}}\eta_{I_{(t)}}^2
	\end{align*}
	where  $A_{I_{(t)}} =  \frac{pH}{2}\left(  8 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega H c_{I_{(t)}} \right) $, $p = \frac{\delta \gamma^*}{8} \leq 1$, $\delta\in(0,1]$, $\beta\in[0,1)$, $\omega\in(0,1]$, $\gamma^* =  \frac{2 \delta \omega}{64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega}$ is the chosen consensus step size, and $\{ c_t \}$ is the triggering threshold sequence.  This completes the proof for Lemma \ref{lem_cvx}.
\end{proof}
%--------------------------
\begin{claim} \label{c_t-eta_bound}
	Let $\mathcal{I}_T$ denote the set of synchronization indices in Algorithm \ref{alg_dec_sgd_li}. Then for any consecutive indices $I_{(t)}, I_{(t+1)} \in \mathcal{I}_T$ we have $c_{I_{(t+1)}-1}\eta_{I_{(t+1}-1}^2 \leq H c_{I_{(t)}}\eta_{I_{(t)}}^2$ where $c_t$ is the threshold sequence, $\eta_t$ is the learning rate sequence and $H$ is the number of local SGD steps between synchronization indices.
\end{claim}
\begin{proof}
	As we allow only for a fixed number of iterations $H$ between any consecutive synchronization indices, we have $I_{(t+1)} = I_{(t)}+H$. Now, for triggering threshold of the form $c_t = c_0 t^{1-\epsilon}$ for some $\epsilon \in (0,1)$ and $\eta_t = \frac{b}{t+a}$, we have:
	  \begin{align*}
	  \frac{c_{t} \eta_t^2}{c_{t-H}\eta_{t-H}^2} =  \left(  \frac{t}{t-H}  \right)^{1-\epsilon} \left(\frac{t-H+a}{t+a}\right)^2 \leq \frac{t}{t-H} 
	  \end{align*}
	  where the inequality follows from the fact that $\epsilon > 0$, $t-H+a < t+a$ and $t > t-H$. Thus, for $t \geq \frac{H^2}{H-1}$, we have:
	  \begin{align*}
	  	\frac{c_{t} \eta_t^2}{c_{t-H}\eta_{t-H}^2} \leq H
	  \end{align*}
\end{proof}
%------------Lemma-------
\begin{lemma}
\label{suppl_lem_coeff_calc}
	Consider the following variables:
	\begin{align*}
	\pi_1 (\gamma) & := \gamma^2 \lambda^2 (1+\alpha_1^{-1}) + (1+\gamma \lambda)^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
	\pi_2 (\gamma) & := (1-\delta \gamma)^2(1+\alpha_1) + \gamma^2 \lambda^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
	\pi_t & := 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\alpha_5)(\pi_1(\gamma) + \pi_2(\gamma) ) \\
	& + 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)((1+\alpha_2^{-1}) + (1-\omega)(1+\alpha_3^{-1})(1+\alpha_2) ) + (1+\alpha_2)\omega nH c_t
	\end{align*}
	and the following choice of variables:
	\begin{align*}
	\alpha_1 := \frac{\gamma \delta}{2}, \, 
	\alpha_2 := \frac{\omega}{4}, \,
	\alpha_3 := \frac{\omega}{4}, \,
	\alpha_4 := \frac{\omega}{4}, \,
	\alpha_5 := \frac{2}{p} \\
	p := \frac{\delta \gamma^*}{8}, \,
	\gamma^* := \frac{2 \delta \omega}{64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega} \\
	\end{align*}
	Then, it can be shown that:
	\begin{align*}
	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \}  \leq 1 - \frac{\delta^2 \omega}{644} \hspace{0.3cm}, \hspace{0.3cm}
	\pi_t \leq 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p}  \right) + 2 \omega nH c_t.
	\end{align*}
\end{lemma}
\begin{proof}
We adapt a part of the proof of [Theorem 2]\cite{koloskova_decentralized_2019-1} to prove Lemma \ref{suppl_lem_coeff_calc}. Note the in the proof of [Theorem 2]\cite{koloskova_decentralized_2019-1}, only two terms $\pi(\gamma)$ and $\pi(\gamma)$ arise (which have fewer variable than ours), and they do not even have the $\pi_t$ term, which arises because the use of local iterations, triggering threshold, and the momentum factor in our algorithm.

	Consider:
	\begin{align*}
	(1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) & = (1+\frac{\omega}{4})^3 (1-\omega) \\
	& = \left( 1 - \frac{\omega^4}{64} - \frac{11 \omega^3}{64} - \frac{9 \omega^2}{16} - \frac{\omega}{4} \right) \\
	& \leq \left( 1 - \frac{\omega}{4} \right)
	\end{align*}
	This gives us:
	\begin{align*}
	\pi_1(\gamma) \leq \gamma^2\lambda^2\left(1+\frac{2}{\gamma \delta} \right) + (1+\gamma\lambda)^2 \left( 1 - \frac{\omega}{4} \right)
	\end{align*}
	Noting that $\gamma^2 \leq \gamma $ (for $\gamma \leq 1 $ which is true for $\gamma^*$ ) and $\lambda \leq 2$, we have:
	\begin{align*}
	\pi_1(\gamma) \leq \lambda^2\left(\gamma +\frac{2\gamma}{\delta} \right) + (1+8\gamma) \left( 1 - \frac{\omega}{4} \right)
	\end{align*}
	Substituting value of $\gamma^*$ in above, it can be shown that:
	\begin{align*}
	\pi_1(\gamma^*) \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega)}
	\end{align*}
	Now we note that:
	\begin{align*}
	\pi_2 (\gamma) & =  (1-\delta \gamma)^2 \left(1+\frac{\delta \gamma}{2} \right) + \gamma^2 \lambda^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega}{4} \right)^2 (1-\omega) 
	\intertext{Noting the fact that for $x = \delta \gamma \leq 1 $, we have $(1 - x)^2 \left(1 + \frac{x}{2}\right) \leq (1-x)\left( 1 - \frac{x}{2}  \right) $,}
	\pi_2 (\gamma) & \leq \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \lambda^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega}{4} \right)^2 (1-\omega)\\
	%	& = \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega^2}{16} + \frac{\omega}{2} \right) (1-\omega) \\
	& = \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \lambda^2 \left(3+\frac{3\omega}{4}+\frac{\omega^2}{16} + \frac{4}{\omega} \right) (1-\omega) \\
	& \leq \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \lambda^2 \frac{4}{\omega} \, =: \zeta(\gamma)
	\end{align*}
	Note that $\zeta(\gamma)$ is convex and quadratic in $\gamma$, and attains minima at $\gamma' = \frac{2 \delta \omega}{16 \lambda^2 + \delta^2 \omega}$ with value $\zeta(\gamma') = \frac{16\lambda^2}{16\lambda^2 + \omega \delta^2}$.
	
	By the Jensen's inequality, we note that for any $s \in [0,1]$
	\begin{align*}
	\zeta(s \gamma') \leq (1-s) \zeta(0) + s \zeta(\gamma') = 1 - s \frac{\delta^2 \omega}{16 \lambda^2 + \delta^2 \omega}
	\end{align*}
	For the choice $s = \frac{16\lambda^2 + \omega \delta^2}{64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega}$, it can be seen that $s \gamma' = \gamma^*$. Thus we get:
	\begin{align*}
	\pi_2(\gamma^*) \leq  \zeta(s \gamma')  & \leq 1 - \frac{\delta^2\omega}{(64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega)} \\
	& \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega)}
	\end{align*}
	Thus we have:
	\begin{align*}
	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \} & \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega)}.
	\intertext{Using the value of $\gamma^*$ given in the lemma statement, we have $ \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega)} = \frac{\delta \gamma^*}{8}$. Define $p : = \frac{\gamma^* \delta}{8}$. 
	Using crude estimates $\delta \leq 1, \omega \geq 0, \lambda \leq2$, we can lower-bound $p$ as $p \geq \frac{\delta^2 \omega}{644}$. Thus we have }
	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \} & \leq 1 - \frac{\delta^2 \omega}{644}.
	\end{align*}
	Now we upper-bound the value of $\pi_t$:
	\begin{align*}
		\pi_t & := 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)(1+\alpha_5)(\pi_1(\gamma) + \pi_2(\gamma) )  + (1+\alpha_2)\omega n H c_t \\
		& \qquad + 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)((1+\alpha_2^{-1}) + (1-\omega)(1+\alpha_3^{-1})(1+\alpha_2) ) \\
		& \leq 16 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\frac{2}{p})(1-p) + (1+\frac{\omega}{4})\omega nH c_t \\
		& \qquad + 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)((1+\frac{4}{\omega}) + (1-\omega)(1+\frac{4}{\omega})(1+\frac{\omega}{4}) )  \\
		& \leq 16 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)\frac{2}{p} + (1+\frac{\omega}{4})\omega nH c_t + 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4}\right)(1+\frac{8}{\omega} )  \\
	\end{align*}
	Where in the first inequality we have used the fact that $\pi_1(\gamma) + \pi_2(\gamma) \leq 2(1-p) $. In the second inequality, we use the fact that $(1+\frac{2}{p})(1-p) \leq \frac{2}{p} $ and $(1-\omega)(1+\frac{4}{\omega})(1+\frac{\omega}{4}) \leq \frac{4}{\omega}$. Noting that for $\omega \leq 1$, we have $(1+\frac{\omega}{4}) \leq 2$ and $\left(1 + \frac{8}{\omega}\right) \leq \frac{16}{\omega}$. Using these, we have:
	\begin{align*}
		\pi_t & \leq 8 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left(\frac{4}{p} + \frac{16}{\omega} \right) + 2\omega nH c_t.
	\end{align*}
	This completes the proof of Lemma \ref{suppl_lem_coeff_calc}.
\end{proof}
%------------Lemma-------
\begin{lemma}  \label{suppl_lem_e_seq_li}
	Consider the sequence \{$e_{I_{(t)}}$\} given by
	\begin{align*}
	e_{I_{(t+1)}} \leq \left( 1-\frac{p}{2} \right)e_{I_{(t)}} + \frac{2}{p}\eta_{I_{(t)}}^2 n A_{I_{(t)}},
	\end{align*}
	where $ \mathcal{I}_T = \{ I_{(1)}, I_{(2)} , \hdots , I_{(t)}, \hdots  \} \in [T] $ denotes the set of synchronization indices. For a parameter $p >0$, an increasing positive sequence $\{A_t\}_{t=0}^{T-1}$, stepsize $\eta_t = \frac{b}{t+a}$ with parameter $a \geq \frac{5H}{p}$ and arbitrary $b >0$, we have:
	\begin{align*}
	e_{I_{(t)}} \leq \frac{20}{p^2}nA_{I_{(t)}}\eta_{I_{(t)}}^2.
	\end{align*}
\end{lemma}
\begin{proof}
The proof of Lemma \ref{suppl_lem_e_seq_li} is along the lines of the proof of [Lemma 22]\cite{koloskova_decentralized_2019-1}.

	We will proceed the proof by induction. Note that for $t=0$, $e_{I_{(0)}}:=0$ (we assume first synchronization index is 0), thus statement is true. Assume the statement holds for index $I_{(t)}$, then for index $I_{(t+1)}$:  
	\begin{align} \label{cvx_lemm_rec_interim1}
	e_{I_{(t+1)}} \leq \left( 1- \frac{p}{2} \right)e_{I_{(t)}} + \frac{2}{p}nA_{(t)}\eta_{I_{(t)}}^2 & \leq \left( 1- \frac{p}{2} \right)\frac{20}{p^2}nA_{I_{(t)}}\eta_{I_{(t)}}^2 + \frac{2}{p}nA_{I_{(t)}}\eta_{I_{(t)}}^2 \notag \\
	& = \frac{nA_{I_{(t)}}\eta_{I_{(t)}}^2}{p^2}(20-8p)  \stackrel{(p \geq \frac{5H}{a})}{\leq} \frac{20nA_{I_{(t)}}\eta_{I_{(t)}}^2}{p^2}\left( 1- \frac{2H}{a} \right)
	\end{align}
	Now we show that $\eta_{I_{(t)}}^2 \left( 1- \frac{2H}{a} \right) \leq \eta_{I_{(t+1)}}^2$.
	Since $\eta_{I_{(t+1)}} = \frac{b}{a + I_{(t+1)} }$, it suffices to prove that $(a+ I_{(t+1)})^2 \left( 1- \frac{2H}{a} \right) \leq (a+ I_{(t)})^2$, which we show below.
%	As the maximum sequence gap of $\mathcal{I}_T$ is $H$, we have:
	\begin{align*}
	(a+ I_{(t+1)})^2 \left( 1- \frac{2H}{a} \right) & \leq (a+ I_{(t)} + H )^2 \left( 1- \frac{2H}{a} \right) \tag{since $I_{(t+1)} \leq I_{(t)} + H$} \\
	& = (a+ I_{(t)})^2 + 2H(a+ I_{(t)}) + H^2 \\
	& \qquad - \left[ \frac{2H(a+ I_{(t)})^2}{a} + \frac{4H^2(a+ I_{(t)})}{a} + \frac{2H^3}{a} \right] \\
	& \leq (a+ I_{(t)})^2 + 2H(a+ I_{(t)}) + H^2 - \left[ 2H(a+ I_{(t)}) + 4H^2 \right] \\
	& \leq (a+ I_{(t)})^2
	\end{align*}
%	Thus, for $\eta_{I_{(t+1)}} = \frac{b}{a + I_{(t+1)} }$, we get:
%	\begin{align*}
%	\eta_{I_{(t)}}^2 \left( 1- \frac{2H}{a} \right) \leq \eta_{I_{(t+1)}}^2
%	\end{align*}
	Substituting the above bound in the bound for $e_{I_{(t+1)}}$ in \eqref{cvx_lemm_rec_interim1} and using the fact that $A_t$ is an increasing function:
	\begin{align*}
	e_{I_{(t+1)}} \leq \frac{20nA_{I_{(t)}}\eta_{I_{(t+1)}}^2}{p^2} \leq \frac{20nA_{I_{(t+1)}}\eta_{I_{(t+1)}}^2}{p^2}.
	\end{align*}
	Thus, by induction, $e_{I_{(t)}} \leq \frac{20nA_{I_{(t)}}\eta_{I_{(t)}}^2}{p^2}$ for all $I_{(t)} \in \mathcal{I}_T$.	
	This completes the proof of Lemma \ref{suppl_lem_e_seq_li}.
\end{proof}
}

==> lemma_noncvx_loc_global_err.tex <==
{\allowdisplaybreaks
	
%\section{Proof of Lemma \ref{lem_noncvx}}	
%
%\begin{lemma*} (Restating Lemma \ref{lem_noncvx})
%	Let $ \{ \bx_t ^{(i)}  \}_{t=0}^{T-1} $ be generated according to Algorithm \ref{alg_dec_sgd_li} under assumptions of Theorem \ref{thm_noncvx_fix_li} with constant stepsize $\eta$, an increasing threshold fucntion $c_t$ such that $c_t \leq \frac{1}{\eta^{(1-\epsilon)}}$ for all $t$ for some $\epsilon \in (0,1)$ and define $\bar{\bx}_t = \frac{1}{n} \sum_{i=1}^{n} \bx_t^{(i)} $.
%	Consider the set of synchronization indices $\mathcal{I}_T$ =  $\{ I_{(1)},I_{(2)}, \hdots, I_{(t)}, \hdots  \}$. Then for any $I_{(t)} \in \mathcal{I}_T$, we have:
%	\begin{align*}
%	\mathbb{E}\sum_{j=1}^n \left\Vert \bar{\bx}^{I_{(t)}} - \bx^{I_{(t)}}_{j} \right\Vert^2 = \mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2  \leq \frac{4nA  \eta^2}{p^2}
%	\end{align*}
%	for constant $A = \frac{p}{2}\left(  2 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + \frac{2\omega }{\eta^{(1-\epsilon)}} \right)$ where $p = \frac{\delta \gamma}{8} $, $\delta := 1 - | \lambda_2(\mathbf{W})|$, $\omega$ is compression parameter for operator $\C$, and $c_{I_{(t)}}$ and $\eta_{I_{(t)}}$ are respectively the triggering threshold and learning rate evaluated at timestep $I_{(t)}$.
%\end{lemma*}



%Our proof for Lemma \ref{lem_noncvx} involves analyzing the following expression:
%\begin{align*}
%e_{I_{(t+1)}} := \underbrace{\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2}_{e^{(1)}_{I_{(t+1)}}} + \underbrace{ \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}} \Vert_F^2}_{e^{(2)}_{I_{(t+1)}}}
%\end{align*}
%The first term $e^{(1)}_{I_{(t+1)}}$ in RHS above captures the deviation of local parameters of the nodes from the global average parameter. The second term $e^{(2)}_{I_{(t+1)}}$ captures the deviation of the node parameters from their copies. In the section for Proof Outlines \ref{proof-outlines}, we proposed the idea of writing a bound for 
%$e^{(1)}_{I_{(t+1)}}$ (and $e^{(2)}_{I_{(t+1)}}$) in terms of $e^{(1)}_{I_{(t)}}$ (and $e^{(2)}_{I_{(t)}}$), enabling us to write a recursive expression which could then be translated to a recursive expression for the sum $e_{I_{(t+1)}}$ in terms of $e_{I_{(t)}}$. \\
%We follow a different approach here, where we bound $e^{(1)}_{I_{(t+1)}}$ and $e^{(2)}_{I_{(t+1)}}$ individually in terms of parameters evaluated at the auxillary index $I_{(t+\frac{1}{2})}$. These bounds are provided in Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} below. These individual bounds are then added to yield a bound for the sum $e_{I_{(t+1)}}$ in terms of parameters evaluated at the auxillary index $I_{(t+\frac{1}{2})}$. 
%Further simplification allows us to bound $e_{I_{(t+1)}}$ in terms of $e_{I_{(t)}}$, thus giving a recursive form.
%%We first provide two lemmas which enable us to write recursive expressions for $e^{(1)}_{I_{(t+1)}}$ and $e^{(2)}_{I_{(t+1)}}$ (Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} respectively) and thus $e_{I_{(t+1)}}$.
%This recursion enables us to bound $e_{I_{(t+1)}}$ as $e_{I_{(t+1)}} \leq \frac{20A_{I_{(t+1)}}}{p^2} \eta_{I_{(t+1)}}^2$ where $A_{I_{(t+1)}}$ is defined in the statement of Lemma \ref{lem_cvx}. Thus, the quantity of interest $e^{(1)}_{I_{(t+1)}} = \mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 $ is also bounded by $\frac{20A_{I_{(t+1)}}}{p^2} \eta_{I_{(t+1)}}^2$, proving Lemma \ref{lem_cvx}. \\
%We first state and prove bounds on $e^{(1)}_{I_{(t+1)}}$ and $e^{(2)}_{I_{(t+1)}}$ in terms of parameters evaluated at the auxillary index $I_{(t+\frac{1}{2})}$ in Lemma \ref{lem_cvx_e1} and \ref{lem_cvx_e2} respectively. Using these bounds, we then proceed to prove Lemma \ref{lem_cvx}. \\
%
%\begin{lemma} \label{lem_cvx_e1}
%	Consider the sequence of updates in Algorithm \ref{alg_dec_sgd_li} in matrix form (refer \ref{mat_not_li}). The expected deviation between the local node parameter $\bX^{I_{(t+1)}}$ and the global average parameter $\Bar{\bX}^{I_{(t+1)}}$ evaluated at some $I_{(t+1)} \in \mathcal{I}_T$ satisfies:
%	\begin{align*}
%	e^{(1)}_{I_{(t+1)}} := \mathbb{E} \Vert \bX^{I_{(t+1)}} - & \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 \leq \\
%	& (1+\alpha_5^{-1})R_1 \mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2 + (1+\alpha_5^{-1}) R_2 \mathbb{E} \Vert  {\bX}^{I_{(t)}}-\hat{\bX}^{I_{(t+1)}}\Vert_F^2 + Q_1
%	\end{align*}
%	where $R_1=(1+\alpha_1)(1-\gamma \delta)^2 , R_2=(1+\alpha_1^{-1}) \gamma^2 \beta^2 $ and $Q_1 = 2\eta^2 H^2 n G^2 \left(1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\alpha_5)(R_1+R_2) $. Here $\alpha>0, \alpha_1, \alpha_5 >0$ are constants, $\delta$ is the spectral gap, $H$ is the synchronization gap, $\gamma$ is the consensus stepsize and $\beta = \verts{\mathbf{W}-\mathbf{I}}_2$ where $\mathbf{W}$ is a doubly stochastic mixing matrix. Constant $\alpha$ is chosen such that $\alpha > \frac{\beta^2}{(1-\beta^2)}$.
%\end{lemma} 
%\begin{proof}
%	% 	We first focus on bounding the first term in (\ref{suppl_et_eqn_li}). 
%	(The proof uses techniques similar to that of \cite[Lemma 17]{koloskova_decentralized_2019-1}).\\
%	Using the definition of $\bX^{I_{(t+1)}}$ from matrix notation in Section \ref{mat_not_sec}, we have:
%	\begin{align}
%	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & = \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+1)}} + \gamma \hat{\bX}^{I_{(t+1)}} (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag 
%	\intertext{Noting that $\Bar{\bX}^{I_{(t+1)}} = \Bar{\bX}^{I_{(t+\frac{1}{2})}} $ from (\ref{mean_seq_iter}) and $\Bar{\bX}^{I_{(t+\frac{1}{2})}} (\mathbf{W}-\mathbf{I})= 0$ from (\ref{mean_prop}), we get: }
%	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & = 
%	% 	\Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} + \gamma ( {\bX}^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} )  (\mathbf{W}-\mathbf{I})+ \gamma (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}}) (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag \\
%	% 	& =
%	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})+ \gamma (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}}) (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag
%	\intertext{Using the fact $\Vert \mathbf{A} + \mathbf{B} \Vert_F^2 \leq (1+\alpha_1)\Vert \mathbf{A}\Vert_F^2 + (1+\alpha_1^{-1})\Vert \mathbf{B} \Vert_F^2$ for any $\alpha_1 >0$, }
%	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq (1+\alpha_1)\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F^2 \notag \\
%	& \qquad + (1+\alpha_1^{-1}) \Vert \gamma (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}}) (\mathbf{W}-\mathbf{I}) \Vert_F^2 \notag \\
%	\intertext{Using $\Vert \mathbf{A} \mathbf{B} \Vert_F \leq \Vert \mathbf{A} \Vert_F \Vert \mathbf{B} \Vert_2 $ as per (\ref{bound_frob_mult}), we have: }
%	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 &  \leq (1+\alpha_1)\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F^2 \notag \\
%	& \qquad + (1+\alpha_1^{-1}) \gamma^2 \Vert  (\hat{\bX}^{I_{(t+1)}}-\bX^{I_{(t+\frac{1}{2})}})\Vert_F^2 .\Vert(\mathbf{W}-\mathbf{I})\Vert_2^2 \label{suppl_cvx_li_temp_eqn}
%	\end{align}
%	To bound the first term in (\ref{suppl_cvx_li_temp_eqn}), we use the triangle inequality for Frobenius norm, giving us:
%	\begin{align*}
%	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F & \leq (1-\gamma)\Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F \\
%	& \qquad + \gamma \Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} )W\Vert_F
%	\end{align*}
%	{From (\ref{mean_prop}), using $\Bar{\bX}^{I_{(t+\frac{1}{2})}} = \bX^{I_{(t+\frac{1}{2})}}\frac{\mathbbm{1}\mathbbm{1}^T}{n} $ and noting that $ \Bar{\bX}^{I_{(t+\frac{1}{2})}} \frac{\mathbbm{1}\mathbbm{1}^T}{n} = \Bar{\bX}^{I_{(t+\frac{1}{2})}} $, we get: }
%	\begin{align*}
%	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F & \leq (1-\gamma)\Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F \\
%	& \qquad + \gamma \left\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})\left (\mathbf{W} - \frac{\mathbbm{1}\mathbbm{1}^T}{n} \right) \right\Vert_F 
%	%	\intertext{Using remark 4,}
%	\end{align*}
%	{Using $\Vert \mathbf{A} \mathbf{B} \Vert_F \leq \Vert \mathbf{A} \Vert_F \Vert \mathbf{B} \Vert_2 $ as per (\ref{bound_frob_mult}) and using (\ref{bound_W_mat}) for $k=0$, we can simplify the above to: }
%	\begin{align*}
%	\Vert (\bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}})((1-\gamma)\mathbf{I} + \gamma \mathbf{W})\Vert_F \leq (1-\gamma \delta) \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F
%	\end{align*}
%	Substituting the above in (\ref{suppl_cvx_li_temp_eqn}) and using $\beta = \text{max}_i \{ 1- \lambda_i(\mathbf{W}) \} \Rightarrow \Vert \mathbf{W}-\mathbf{I} \Vert_2^2 \leq \beta^2 $, we get: 
%	\begin{align*}
%	\Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 \leq (1+\alpha_1)(1-\gamma \delta)^2  \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 + (1+\alpha_1^{-1}) \gamma^2 \beta^2 \Vert  {\bX}^{I_{(t+\frac{1}{2})}}-\hat{\bX}^{I_{(t+1)}}\Vert_F^2
%	\end{align*}
%	Taking expectation w.r.t the entire process, we have:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq (1+\alpha_1)(1-\gamma \delta)^2 \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 \notag \\
%	& \qquad + (1+\alpha_1^{-1}) \gamma^2 \beta^2 \mathbb{E} \Vert  {\bX}^{I_{(t+\frac{1}{2})}}-\hat{\bX}^{I_{(t+1)}}\Vert_F^2
%	\end{align*}
%	Define $R_1=(1+\alpha_1)(1-\gamma \delta)^2 , R_2=(1+\alpha_1^{-1}) \gamma^2 \beta^2 $
%	Using the update algorithm, we have:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq R_1 \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} -  \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta( \beta \bV^{(t')} +  \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right) \right\Vert_F^2 \notag \\
%	& \qquad + R_2 \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} + \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta ( \beta \bV^{(t')} + \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2
%	\end{align*} 	
%	Thus, for some constant $\alpha_5 > 0 $ we have:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq R_1 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_2 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
%	 & \qquad + R_1(1+\alpha_5)  \mathbb{E} \left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right) \right\Vert_F^2 \notag \\
%	 & \qquad + R_2 (1+\alpha_5) \mathbb{E} \left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2
%	\end{align*}
%	Using $\verts{AB}_F \leq \verts{A}_F \verts{B}_2$ as per \eqref{bound_frob_mult} to split the third term along with \eqref{bound_W_mat}, and further using the bound in (\ref{bound_gap_grad}) for some constant $\alpha > \frac{\beta^2}{1 - \beta^2}$ for the third and fourth term, the above can be rewritten as:  
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq R_1 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_2 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
%	& \qquad + 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\alpha_5)(R_1+R_2)
%	\end{align*}
%	Defining $Q_1 = 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\alpha_5)(R_1+R_2) $ 	completes the proof.
%\end{proof}
%%-----------------------------------------------------------------
%\begin{lemma}\label{lem_cvx_e2}
%	Consider the sequence of updates in Algorithm \ref{alg_dec_sgd_li} in matrix form (refer \ref{mat_not_li}) with the threshold sequence $ \{  c_t \}_{t=0}^{T-1} $ and constant learning rate $\eta$ such that $c_t < \frac{1}{\eta}$  for all t $\in [T]$ . The expected deviation between the local node parameters $\bX^{I_{(t+1)}}$ and their copies $\hat{\bX}^{I_{(t+2)}}$ evaluated at a synchronization timestep $I_{(t+1)}$ satisfy:
%	\begin{align*}
%	e^{(2)}_{I_{(t+1)}} =	\mathbb{E} \Vert \bX^{I_{(t+1)}} - & \hat{\bX}^{I_{(t+2)}}\Vert_F^2	 \leq \\
%	& (1+\alpha_5^{-1}) R_3 \mathbb{E} \Vert \bX^{I_{(t)}}- \Bar{\bX}^{I_{(t)}} \Vert_F^2 + (1+\alpha_5^{-1})R_4 \mathbb{E} \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}}\Vert_F^2  +  Q_2
%	\end{align*}
%	where $R_3 = (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)$ , $R_4 = \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) $ and $Q_2 = 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)((1+\alpha_5)(R_3+R_4)+( 1+\alpha_2^{-1}) + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega)) + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2 $. Note that $Q_2$ depends on $t$ (as captured by $c_{I_{(t)}}$ in the expression) as we allow for our triggering threshold to change with time.  Here $\alpha>0, \alpha_2, \alpha_3, \alpha_4 >0, \alpha_5 >0$ (same used in Lemma \ref{lem_cvx_e1}) are constants, $\delta$ is the spectral gap, $H$ is the synchronization gap, $\gamma$ is the consensus stepsize and $\beta = \verts{\mathbf{W}-\mathbf{I}}_2$ where $\mathbf{W}$ is a doubly stochastic mixing matrix. Constant $\alpha$ is chosen such that $\alpha > \frac{\beta^2}{(1-\beta^2)}$.
%\end{lemma} 
%\begin{proof}
%	Using definition of $\hat{\bX}^{I_{(t+2)}}$ from matrix notation in Section \ref{mat_not_sec} and considering expectation w.r.t entire process, we have:
%	\begin{align*}
%	& \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2  = \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 \\
%	&  \hspace{2.4cm} = \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}+ \bX^{I_{(t+1)}} - \bX^{I_{(t+\frac{3}{2})}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 
%	\end{align*}
%	Using $\Vert \mathbf{A} + \mathbf{B} \Vert_F^2 \leq (1+\alpha_2)\Vert \mathbf{A}\Vert_F^2 + (1+\alpha_2^{-1})\Vert \mathbf{B} \Vert_F^2$ for any $\alpha_2 >0$,
%	\begin{align}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 & \leq (1+\alpha_2) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}}- \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 \notag \\
%	&\hspace{2cm} + (1+\alpha_2^{-1})\mathbb{E}\Vert \bX^{I_{(t+1)}} - \bX^{I_{(t+\frac{3}{2})}} \Vert_F^2 \notag \\
%	& = (1+\alpha_2) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 \notag \\
%	& \hspace{2cm} + (1+\alpha_2^{-1})\mathbb{E}\left\Vert \sum_{t' = I_{(t+1)}}^{I_{(t+2)}-1} \eta( \beta \bV^{(t')} +  \partial F (\bX^{t'}, \xi^{t'})) \right\Vert_F^2 \label{cvx_lem1_interim1}
%	\end{align}
%	Bounding the last term in \eqref{cvx_lem1_interim1} using (\ref{bound_gap_grad}), we get:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 & \leq (1+\alpha_2) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2 \\
%	& \qquad + (1+\alpha_2^{-1}) 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)
%	\end{align*}
%	Noting that the entries of $\mathbf{P}^{(I_{(t+2)}-1)} $ and $\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)} $ are disjoint, we can separate them in the squared Frobenius norm:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - & \hat{\bX}^{I_{(t+2)}}\Vert_F^2  \leq  (1+\alpha_2)  \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})\mathbf{P}^{(I_{(t+2)}-1)} - \C ( (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}}) \mathbf{P}^{(I_{(t+2)}-1)} )\Vert_F^2  \\
%	&   + (1+\alpha_2) \mathbb{E}\Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2  + 2 (1+\alpha_2^{-1}) \eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)
%	\end{align*}
%	Using the compression property of operator $\C$ as per (\ref{bound_comp}), we have:
%	\begin{align*}
%	& \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \leq (1+\alpha_2) (1-\omega) \mathbb{E}  \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})\mathbf{P}^{(I_{(t+2)}-1)} \Vert_F^2 \\
%	& \hspace{2.5cm} +  (1+\alpha_2) \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2  + 2 (1+\alpha_2^{-1}) \eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)
%	\end{align*}
%	Adding and subtracting $ (1+\alpha_2)(1-\omega)  \mathbb{E}\Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2$, we get:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 & \leq (1+\alpha_2) (1-\omega)  \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + (1+\alpha_2^{-1})2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)  \\
%	& \qquad +(1+\alpha_2) \omega  \mathbb{E} \Vert (\bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}})(\mathbf{I} - \mathbf{P}^{(I_{(t+2)}-1)})\Vert_F^2 
%	\end{align*}
%	The third term in the RHS above denotes the norm of nodes which did not communicate and thus should be bounded by the triggering condition using (\ref{bound_trig}),
%	\begin{align} \label{cvx_lemm_interim2}
%	\mathbb{E}& \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \notag \\
%	& \leq (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+\frac{3}{2})}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 +(1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2 \notag \\
%	& \qquad + (1+\alpha_2^{-1}) 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \notag \\
%	& = (1+\alpha_2) (1-\omega) \mathbb{E} \left\Vert \bX^{I_{(t+1)}}  - \sum_{t' = I_{(t+1)}}^{I_{(t+2)}-1}\eta(\beta \bV^{(t')}+  \partial F (\bX^{t'}, \xi^{t'})) -  \hat{\bX}^{I_{(t+1)}} \right\Vert_F^2 + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2 \notag \\
%	& \qquad + (1+\alpha_2^{-1}) 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)  \notag \\
%	& \leq (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+1)}}  -  \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + (1+\alpha_2^{-1}) 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \notag \\
%	& \hspace{0.4cm} + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \mathbb{E} \left\Vert \sum_{t' = I_{(t+1)}}^{I_{(t+2)}-1}\eta( \beta V^{(t')} +  \partial F (\bX^{t'}, \xi^{t'})) \right\Vert_F^2 + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2 
%	\end{align}
%	where in the last inequaility, we have used (\ref{bound_l2_sum}) for some constant $\alpha_3 > 0$. Using (\ref{bound_gap_grad}) to bound the second last term in \eqref{cvx_lemm_interim2} , we have:
%	\begin{align*}
%	\mathbb{E} & \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \\
%	& \leq (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+1)}}  -  \hat{\bX}^{I_{(t+1)}} \Vert_F^2 \\
%	& \qquad +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \\
%	& \qquad + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2  + (1+\alpha_2^{-1}) 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \\
%	& = (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} + \gamma \hat{\bX}^{I_{(t+1)}} (\mathbf{W}-\mathbf{I}) -  \hat{\bX}^{I_{(t+1)}} \Vert_F^2 \\
%	& \qquad +  2(1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega)\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \\
%	& \qquad  + (1+\alpha_2)\omega n c_{I_{(t+1)}}\eta^2 + 2(1+\alpha_2^{-1}) \eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \\
%	& \leq (1+\alpha_3) (1+\alpha_2) (1-\omega)\mathbb{E} \Vert (\bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}})((1+\gamma)\mathbf{I} - \gamma \mathbf{W})+ \gamma (\bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}})(\mathbf{W}-\mathbf{I})\Vert_F^2 \\
%	& \qquad +  2(1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \\
%	& \qquad + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2 + 2(1+\alpha_2^{-1}) \eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)
%	\end{align*}
%	where in the last inequality we've used $ \Bar{\bX}^{I_{(t+\frac{1}{2})}} (\mathbf{W}-\mathbf{I})= 0 $. For $\alpha_4 > 0 $, using (\ref{bound_l2_sum}) gives us:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert (\bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}})((1+\gamma)\mathbf{I} - \gamma \mathbf{W})\Vert_F^2 \\
%	& \hspace{0.5cm} + (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \gamma (\bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}})(\mathbf{W}-\mathbf{I})\Vert_F^2 \\
%	& \hspace{1.0cm} +  2(1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)  \\
%	& \hspace{1.5cm} + 2(1+\alpha_2^{-1}) \eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2
%	\end{align*}
%	Using $\Vert (1+\gamma)\mathbf{I} - \gamma W \Vert_2 = \Vert I + \gamma (\mathbf{I} - \mathbf{W})\Vert_2 = 1 +  \gamma \Vert \mathbf{I} - \mathbf{W} \Vert_2  = 1 + \gamma \beta $ (by definition of $\beta = \text{max}_i \{ 1- \lambda_i(\mathbf{W}) \}$) and $\verts{\mathbf{I} - \mathbf{W}}_2 = \beta$  along with $\verts{\mathbf{AB}}_F \leq \verts{\mathbf{A}}_F\verts{\mathbf{B}}_2$ from (\ref{bound_frob_mult}):
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)\mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}}\Vert_F^2 \notag \\
%	& \qquad + \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 \notag \\
%	& \qquad +2\left(  ( 1+\alpha_2^{-1}) + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \right)\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \\
%	& \qquad  + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2
%	\end{align*}
%	Define $R_3 = (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)$ , $R_4 = \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) $ and $R_5 = 2\left(  ( 1+\alpha_2^{-1}) + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \right)\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) + (1+\alpha_2)\omega n c_{I_{(t+1)}} \eta^2 $, then the above can be rewritten as :
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq R_4 \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}}\Vert_F^2  + R_3 \mathbb{E} \Vert \bX^{I_{(t+\frac{1}{2})}}- \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 +  R_5
%	\end{align*}
%	Using the update rule, this can be expanded as :
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - & \hat{\bX}^{I_{(t+2)}}\Vert_F^2 \leq R_4 \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} + \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta ( \beta \bV^{(t')} +    \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2 \notag \\
%	& + R_3 \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} -  \sum_{t' = I_{(t)}}^{I_{(t+1)}-1}\eta ( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right) \right\Vert_F^2  +  R_5
%	\end{align*}
%	Thus for some constant $\alpha_5 > 0 $ (same as used in Lemma \ref{lem_cvx_e1}), we have:
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}}\Vert_F^2	& \leq R_4 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 + R_3 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
%	& \qquad  + R_3 (1+\alpha_5) \mathbb{E}\left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1} \eta( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} ))\left(   \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right) \right\Vert_F^2  \notag \\
%	& \qquad + R_4 (1+\alpha_5)\mathbb{E} \left\Vert \sum_{t' = I_{(t)}}^{I_{(t+1)}-1}\eta ( \beta \bV^{(t')} +   \partial F(\bX^{(t')}, \xi^{(t')} )) \right\Vert_F^2  +  R_5
%	\end{align*}	
%		Using $\verts{AB}_F \leq \verts{A}_F \verts{B}_2$ as per \eqref{bound_frob_mult} to split the third term along with \eqref{bound_W_mat}, and further using the bound in (\ref{bound_gap_grad}) for some constant $\alpha > \frac{\beta^2}{1 - \beta^2}$ for the third and fourth term, the above can be rewritten as:  
%	\begin{align*}
%	\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 & \leq R_3 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_4 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
%	& \qquad + 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\alpha_5)(R_3+R_4) + R_5
%	\end{align*}
%	Define $Q_2 = 2\eta^2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\alpha_5)(R_3+R_4) + R_5 $ completes the proof.	
%\end{proof}
%
%
%
%\TODO{END HERE}
%--------------------------------------------------------------------------------
\begin{proof} [Proof of Lemma \ref{lem_noncvx}] \label{proof_lemm_dec_li_sgd_fix}
	The proof follows similar steps to proof of Lemma \ref{lem_cvx}. 
	 Specifically, we note that Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} also hold for non-convex objectives although with variable step-size ($ \eta_t $) now replaced by a constant step-size ($\eta$). Note that in either Lemma \ref{lem_cvx_e1} or Lemma \ref{lem_cvx_e2}, we do not use any properties of the learning rate sequence $\eta_t$ apart from the fact that $\eta_{I_{(t)}} \leq 2 \eta_{I_{(t+1)}} $ for all $I_{(t)} \in \mathcal{I}_T$. Also, while deriving Lemmas \ref{lem_cvx_e1} and \ref{lem_cvx_e2}, we used the bound in \eqref{bound_gap_grad} which says $\mathbb{E}[ \Vert v_i^{(t)} \Vert] \leq \frac{9G^2}{(1-\beta)^4}$ for all $t$ and for all $i \in [n]$. In fact, for a constant stepsize $\eta_t = \eta$, it can be shown that this bound can be tightened to $\mathbb{E}[ \Vert v_i^{(t)} \Vert] \leq \frac{G^2}{(1-\beta)^2}$. In the course of proof of Theorem \ref{thm_noncvx_fix_li}, we will use the first bound which allows us to keep same proofs of Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} as before. Thus, the bounds derived in these lemmas also hold with constant step-size $\eta$ although with a slighlty different value of constants $Q_1$ and $Q_2$ on the account for not using the inequality $\eta_{I_{(t)}} \leq 2 \eta_{I_{(t+1)}} $ as now step-size $\eta$ is constant. It is easy to check that the values of $R_1, R_2, R_3$ and $R_4$ in these bounds are the same and the values of $Q_1$ and $Q_2$ now are:
	\begin{align*}
		Q_1 & = 2 H^2 n G^2 \left(1 + \frac{9\beta^2}{(1- \beta)^4} \right)(1+\alpha_5)(R_1+R_2) \\
		Q_2 & = 2H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)((1+\alpha_5)(R_3+R_4)+( 1+\alpha_2^{-1}) + (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega)) \\
		& \qquad + (1+\alpha_2)\omega nH c_{I_{(t+1)}} 
	\end{align*}
Thus, following along the same steps as in proof of Lemma \ref{lem_cvx}  with the updated constants as discussed above, we can rewrite \eqref{suppl_et_eqn_total_li} as:
	\begin{align*} 
&e_{I_{(t+1)}}  %&= \mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 + \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}} \Vert_F^2 \notag \\ 
\leq  R_1 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_2 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2  \\
& \hspace{0.3cm}  + R_3 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + R_4 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 + (Q_1 + Q_2)\eta ^2
\end{align*}		
	
%	We now proceed to the main proof of the lemma. Consider the following expression :
%	\begin{align} \label{suppl_et_eqn_li}
%	e_{I_{(t+1)}} := \underbrace{\mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2}_{e^{(1)}_{I_{(t+1)}}} + \underbrace{ \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}} \Vert_F^2}_{e^{(2)}_{I_{(t+1)}}}
%	\end{align}
%	We note that Lemma \ref{lem_cvx_e1} and Lemma \ref{lem_cvx_e2} provide bounds for the first and second term of in RHS of (\ref{suppl_et_eqn_li}). Substituting them in (\ref{suppl_et_eqn_li}) gives us:
%	\begin{align} \label{suppl_et_eqn_total_li}
%	e_{I_{(t+1)}} & = \mathbb{E} \Vert \bX^{I_{(t+1)}} - \Bar{\bX}^{I_{(t+1)}} \Vert_F^2 + \mathbb{E} \Vert \bX^{I_{(t+1)}} - \hat{\bX}^{I_{(t+2)}} \Vert_F^2 \notag \\ 
%	& \leq  R_2 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 + R_1 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 \notag \\
%	& \hspace{0.3cm}  + R_4 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert   \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \right\Vert^2 + R_3 (1+\alpha_5^{-1}) \mathbb{E} \left\Vert  \Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}} \right\Vert^2 + Q_1 + Q_2
%	\end{align}	
%	Define the following:
%	\begin{align*}
%	\pi_1 (\gamma) & := R_2 + R_4 = \gamma^2 \beta^2 (1+\alpha_1^{-1}) + (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
%	\pi_2 (\gamma) & := R_1 + R_3 = (1-\delta \gamma)^2(1+\alpha_1) + \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
%	\pi_{I_{(t)}} & := Q_1 + Q_2 = 2 H^2 n G^2 \left( 1 + \frac{\beta^2}{(1-\beta)^2} \right) (1+\alpha_5)(R_1 + R_2 +R_3+R_4) \\
%	& + 2 H^2 n G^2\left( 1 + \frac{\beta^2}{(1-\beta)^2} \right) ((1+\alpha_2^{-1}) + (1-\omega)(1+\alpha_3^{-1})(1+\alpha_2) ) + (1+\alpha_2)\omega n c_{I_{(t)}}
%	\end{align*}
%	The bound on $e_{I_{(t+1)}}$ in (\ref{suppl_et_eqn_total_li}) can be rewritten as:
%	\begin{align} \label{lemm_mom_cvx_interim}
%	e_{I_{(t+1)}} & \leq (1+\alpha_5^{-1}) (\pi_1 (\gamma) \mathbb{E} \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \pi_2 (\gamma) \mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2) + \pi_{I_{(t+1)}} \eta^2 \notag \\
%	& \leq (1+\alpha_5^{-1}) max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \} \, \mathbb{E} \left[ \Vert {\bX}^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 \right] + \pi_{I_{(t+1)}}  \eta^2
%	\end{align}

We can define same quantities as in \eqref{cvx_pi1}, \eqref{cvx_pi2} and a slightly different \eqref{cvx_pi3} due to changed values of $Q_1$ and $Q_2$:
\begin{align*}
\pi_1 (\gamma) & := R_2 + R_3 = \gamma^2 \lambda^2 (1+\alpha_1^{-1}) + (1+\gamma \lambda )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)   \\
\pi_2 (\gamma) & := R_1 + R_4 = (1-\delta \gamma)^2(1+\alpha_1) + \gamma^2 \lambda^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
\pi_{t} & := Q_1 + Q_2 \leq 2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)(1+\alpha_5)(R_1 + R_2 +R_3+R_4) \notag \\
& \qquad + 2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)((1+\alpha_2^{-1}) + (1-\omega)(1+\alpha_3^{-1})(1+\alpha_2) ) + (1+\alpha_2)\omega H n c_{t} 
\end{align*}
Thus, similar to \eqref{lemm_mom_cvx_interim}, we can show the total error $e_t$ follows a recursion:
	\begin{align} \label{lemm_mom_noncvx_interim}
e_{I_{(t+1)}} 
%\leq (1+\alpha_5^{-1}) \left[\pi_1 (\gamma) \mathbb{E} \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \pi_2 (\gamma) \mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2\right] + \pi_{I_{(t+1)}} \eta_{I_{(t+1)}}^2 \notag \\
%&\quad 
\leq (1+\alpha_5^{-1}) max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \} \, \mathbb{E} \left[ \Vert {\bX}^{I_{(t+\frac{1}{2})}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \Vert \bX^{I_{(t+\frac{1}{2})}} - \Bar{\bX}^{I_{(t+\frac{1}{2})}} \Vert_F^2 \right] + \pi_{I_{(t+1)}}  \eta^2
\end{align}

	Calculation of $ max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \}$ and $\pi_{I_{(t)}}$ is given in Lemma \ref{suppl_lem_coeff_calc}, where we show that:\\
	$ max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \} \leq   \left(  1 - \frac{\gamma^* \delta}{8}  \right)   \leq \left( 1 - \frac{\delta^2 \omega}{644} \right)  $ and $\pi_t \leq \left(  2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega n H c_{t} \right) $ where $p:= \frac{\gamma^* \delta}{8} $. Here $\gamma^* = \frac{2 \delta \omega}{64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega}$ from Lemma \ref{suppl_lem_coeff_calc} is the consensus step-size.
		Note that the value for bound on $\pi_t$ considered in Lemma \ref{suppl_lem_coeff_calc} is slightly different as it varies only by a constant on the first term, although it is easy to see that the above bound on $\pi_t$ holds now.
	For constant $\alpha_5 := \frac{2}{p}$, substituting these bounds in \eqref{lemm_mom_noncvx_interim} gives us:
	\begin{align*}
	e_{I_{(t+1)}} & \leq (1+\frac{2}{p}) \left( 1 - \frac{\delta \gamma^*}{8} \right)\mathbb{E}  \left[ \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 + \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2 \right] \\ 
	& \qquad + \left(  2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right)  \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega nH c_{I_{(t+1)}} \right) \eta^2
	\end{align*}
	where $p = \frac{\delta \gamma^*}{8}$. From definition of $e_{I_{(t)}} = \mathbb{E} \left[ \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2 + \Vert \bX^{I_{(t)}} - \hat{\bX}^{I_{(t+1)}} \Vert_F^2 \right] $ and by defining $z_t :=\left(  2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2H\omega n c_{{t}} \right) $, we have: 
	\begin{align*}
	e_{I_{(t+1)}} \leq(1+\frac{2}{p}) (1-p) e_{I_{(t)}}  + z_{I_{(t+1)}} \eta^2
	\end{align*}
	Define $A_t := \frac{p z_t}{2n}$ (where $z_t= \left(  2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{ (1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega nH c_{{t}} \right) $ as above), thus we have the following relation:
	\begin{align*} % \label{suppl_lemm_rec_rel_li}
	e_{I_{(t+1)}} \leq \left( 1-\frac{p}{2} \right)e_{I_{(t)}} + \frac{2nA_{I_{(t+1)}}}{p}\eta^2
	\end{align*}
	Note that as we restrict out triggering sequence $c_t < \frac{1}{\eta}$ for all $t \in T$, we have $ c_t \leq \frac{1}{\eta^{(1-\epsilon)}}$ $\forall \, t$, for some $\epsilon \in (0,1)$. Thus $A_{I_{(t+1)}}  \leq A := \frac{p}{2} \left(  2 H^2  G^2 \left( 1 + \frac{9\beta^2}{ (1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + \frac{2\omega H}{\eta^{(1-\epsilon)}} \right)$, giving us:
	\begin{align} \label{noncvx_lemm_interim1}
		e_{I_{(t+1)}} \leq \left( 1-\frac{p}{2} \right)e_{I_{(t)}} + \frac{2nA}{p}\eta^2
	\end{align}
	where constant $A =  \frac{p}{2}\left(  2 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + \frac{2H\omega }{\eta^{(1-\epsilon)}} \right)$.   By the  recursive definition of $e_{I_{(t)}}$ in \eqref{noncvx_lemm_interim1} , it is proved in Lemma \ref{lem_noncvx_seq_bound} that for all $I_{(t)} \in \mathcal{I}_T $, we have:   
	\begin{align*}
	e_{I_{(t)}} \leq \frac{4nA \eta^2}{p^2}
	\end{align*}
%	This can be seen by induction, note that the base case is satisfied as $e_0 = 0$, and assuming the bound holds for $e_{I_{(t)}}$, for $e_{I_{(t+1)}}$, we have: $e_{I_{(t+1)}} \leq (1-\frac{p}{2}) \frac{4A \eta^2}{p^2} + \frac{2A \eta^2}{p} = \frac{4A \eta^2}{p^2}  $.  
	Note that we also have: $ \mathbb{E}\Vert\Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}}\Vert_F^2 \leq \mathbb{E} \left[ \Vert\Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}}\Vert_F^2  + \Vert \hat{\bX}^{I_{(t+1)}} - \bX^{I_{(t)}} \Vert_F^2 \right] := e_{I_{(t)}}$. Thus, we get the following result for any synchronization index $I_{(t)} \in \mathcal{I}_T$:
	\begin{align*}
	\mathbb{E}\Vert\Bar{\bX}^{I_{(t)}} - \bX^{I_{(t)}}\Vert_F^2 \leq \frac{4nA\eta^2}{p^2}
	\end{align*}
	where $A =  \frac{p}{2}\left(  2 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + \frac{2H\omega }{\eta^{(1-\epsilon)}} \right)$ for $p = \frac{\delta \gamma^*}{8}$ , $\epsilon >0$ and 	$\gamma^* =  \frac{2 \delta \omega}{64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega} $ is the chosen consensus step size.  This completes the proof for Lemma \ref{lem_noncvx}
\end{proof}	
	\begin{lemma} \label{lem_noncvx_seq_bound}
		Consider the sequence \{$e_{I_{(t)}}$\} given by
		\begin{align*}
	e_{I_{(t+1)}} \leq \left( 1-\frac{p}{2} \right)e_{I_{(t)}} + \frac{2nA}{p}\eta^2,
		\end{align*}
		where $ \mathcal{I}_T = \{ I_{(1)}, I_{(2)} , \hdots , I_{(t)}, \hdots  \} \in [T] $ denotes the set of synchronization indices. For a parameter $p >0$, positive constants $A$ and $\eta$ , we have:
		\begin{align*}
		e_{I_{(t)}} \leq \frac{4nA}{p^2}\eta^2
		\end{align*}
			\end{lemma}
		\begin{proof}
	The proof uses an induction argument. Note that the base case is satisfied as $e_0 = 0$. Assuming the bound holds for $e_{I_{(t)}}$, for $e_{I_{(t+1)}}$, we have: 
	\begin{align*}
		e_{I_{(t+1)}} & \leq (1-\frac{p}{2}) \frac{4nA \eta^2}{p^2} + \frac{2nA \eta^2}{p} \\
		 & = \frac{4nA \eta^2}{p^2} 
	\end{align*}
	Thus $	e_{I_{(t)}} \leq \frac{4nA}{p^2}\eta^2$ for all $I_{(t)} \in \mathcal{I}_T$ from induction argument, which completes the proof.
		\end{proof}		

%--------------------------
%------------Lemma-------
%\begin{lemma} \label{suppl_lem_coeff_calc}
%	(Variant of \cite[Lemma 18]{koloskova_decentralized_2019-1})
%	Consider the following variables:
%	\begin{align*}
%	\pi_1 (\gamma) & := \gamma^2 \beta^2 (1+\alpha_1^{-1}) + (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
%	\pi_2 (\gamma) & := (1-\delta \gamma)^2(1+\alpha_1) + \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
%	\pi_t & := 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\alpha_5)(\pi_1(\gamma) + \pi_2(\gamma) ) \\
%	& + 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)((1+\alpha_2^{-1}) + (1-\omega)(1+\alpha_3^{-1})(1+\alpha_2) ) + (1+\alpha_2)\omega n c_t
%	\end{align*}
%	and the following choice of variables:
%	\begin{align*}
%	\alpha_1 := \frac{\gamma \delta}{2}, \, 
%	\alpha_2 := \frac{\omega}{4}, \,
%	\alpha_3 := \frac{\omega}{4}, \,
%	\alpha_4 := \frac{\omega}{4}, \,
%	\alpha_5 := \frac{2}{p} \\
%	p := \frac{\delta \gamma^*}{8}, \,
%	\gamma^* := \frac{2 \delta \omega}{64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega} \\
%	\end{align*}
%	Then, it can be shown that:
%	\begin{align*}
%	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \}  \leq 1 - \frac{\delta^2 \omega}{644} \hspace{0.3cm}, \hspace{0.3cm}
%	\pi_t \leq 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \left( \frac{16}{\omega} + \frac{4}{p}  \right) + 2 \omega n c_t
%	\end{align*}
%\end{lemma}
%\begin{proof}
%	Consider:
%	\begin{align*}
%	(1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) & = (1+\frac{\omega}{4})^3 (1-\omega) \\
%	& = \left( 1 - \frac{\omega^4}{64} - \frac{11 \omega^3}{64} - \frac{9 \omega^2}{16} - \frac{\omega}{4} \right) \\
%	& \leq \left( 1 - \frac{\omega}{4} \right)
%	\end{align*}
%	This gives us:
%	\begin{align*}
%	\pi_1(\gamma) \leq \gamma^2\beta^2\left(1+\frac{2}{\gamma \delta} \right) + (1+\gamma\beta)^2 \left( 1 - \frac{\omega}{4} \right)
%	\end{align*}
%	Noting that $\gamma^2 \leq \gamma $ (for $\gamma \leq 1 $ which is true for $\gamma^*$ ) and $\beta \leq 2$, we have:
%	\begin{align*}
%	\pi_1(\gamma) \leq \beta^2\left(\gamma +\frac{2\gamma}{\delta} \right) + (1+8\gamma) \left( 1 - \frac{\omega}{4} \right)
%	\end{align*}
%	Substituting value of $\gamma^*$ in above, it can be shown that:
%	\begin{align*}
%	\pi_1(\gamma^*) \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)}
%	\end{align*}
%	Now we note that:
%	\begin{align*}
%	\pi_2 (\gamma) & =  (1-\delta \gamma)^2 \left(1+\frac{\delta \gamma}{2} \right) + \gamma^2 \beta^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega}{4} \right)^2 (1-\omega) 
%	\intertext{Noting the fact that for $x = \delta \gamma \leq 1 $ : $\left( 1 - x  \right) \left(1 + \frac{x}{2}\right) \leq \left( 1 - \frac{x}{2}  \right) $ and $ \left( 1 -x \right) \left( 1 - \frac{x}{2} \right) \leq \left( 1 - \frac{x}{2}\right)^2 $, }
%	\pi_2 (\gamma) & \leq \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega}{4} \right)^2 (1-\omega)\\
%	%	& = \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega^2}{16} + \frac{\omega}{2} \right) (1-\omega) \\
%	& = \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \left(3+\frac{3\omega}{4}+\frac{\omega^2}{16} + \frac{4}{\omega} \right) (1-\omega) \\
%	& \leq \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \frac{4}{\omega} \, : = \zeta(\gamma)
%	\end{align*}
%	Note that $\zeta(\gamma)$ is convex and quadratic in $\gamma$, and attains minima at $\gamma' = \frac{2 \delta \omega}{16 \beta^2 + \delta^2 \omega}$ with value $\zeta(\gamma') = \frac{16\beta^2}{16\beta^2 + \omega \delta^2}$ \\
%	By Jensen's inequality, we note that for any $\lambda \in [0,1]$
%	\begin{align*}
%	\zeta(\lambda \gamma') \leq (1-\lambda) \zeta(0) + \lambda \zeta(\gamma') = 1 - \lambda \frac{\delta^2 \omega}{16 \beta^2 + \delta^2 \omega}
%	\end{align*}
%	For the choice $\lambda' = \frac{16\beta^2 + \omega \delta^2}{64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega}$, it can be seen that $\lambda' \gamma' = \gamma^*$. Thus we get:
%	\begin{align*}
%	\pi_2(\gamma^*) \leq  \zeta(\lambda' \gamma')  & \leq 1 - \frac{\delta^2\omega}{(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)} \\
%	& \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)}
%	\end{align*}
%	Thus we have:
%	\begin{align*}
%	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \} & \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)}
%	\intertext{from the value of $\gamma^*$ calculated above, we note that $ \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)} = \frac{\delta \gamma^*}{8}$. Define $p : = \frac{\gamma^* \delta}{8}$ Using crude estimates $\delta \leq 1, \omega \geq 0, \beta \leq2$, we thus have: }
%	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \} & \leq 1 - \frac{\gamma^* \delta}{8} = 1 - p  \leq 1 - \frac{\delta^2 \omega}{644}
%	\end{align*}
%	Now we note the value of $\pi_t$ (here $\omega \in (0,1)$):
%	\begin{align*}
%		\pi_t & := 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\alpha_5)(\pi_1(\gamma) + \pi_2(\gamma) )  + (1+\alpha_2)\omega n c_t \\
%		& \qquad + 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)((1+\alpha_2^{-1}) + (1-\omega)(1+\alpha_3^{-1})(1+\alpha_2) ) \\
%		& \leq 4 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\frac{2}{p})(1-p) + (1+\frac{\omega}{4})\omega n c_t \\
%		& \qquad + 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)((1+\frac{4}{\omega}) + (1-\omega)(1+\frac{4}{\omega})(1+\frac{\omega}{4}) )  \\
%		& \leq 4 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)\frac{2}{p} + (1+\frac{\omega}{4})\omega n c_t \\
%		& \qquad + 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)(1+\frac{8}{\omega} )  \\
%	\end{align*}
%	Where in the first inequality we have used the fact that $\pi_1(\gamma) + \pi_2(\gamma) \leq 2(1-p) $. In the second inequality, we use the fact that $(1+\frac{2}{p})(1-p) \leq \frac{2}{p} $ and $(1-\omega)(1+\frac{4}{\omega})(1+\frac{\omega}{4}) \leq \frac{4}{\omega}$. Noting that $\omega \leq 1$, we have $\frac{4}{\omega} \geq 1$ and $(1+\frac{\omega}{4}) \omega \leq 2\omega$. Using these, we have:
%	\begin{align*}
%		\pi_t & \leq 2 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \left(\frac{4}{p} + \frac{16}{\omega} \right) + 2\omega n c_t
%	\end{align*}
%\end{proof}
}
%------------Lemma-------
%\begin{lemma}  \label{suppl_lem_e_seq_li} (Variant of \cite[Lemma 22]{koloskova_decentralized_2019-1})
%	Consider the sequence \{$e_{I_{(t)}}$\} given by
%	\begin{align*}
%	e_{I_{(t+1)}} \leq \left( 1-\frac{p}{2} \right)e_{I_{(t)}} + \frac{2}{p}\eta^2A_{I_{(t)}}
%	\end{align*}
%	where $ \mathcal{I}_T = \{ I_{(1)}, I_{(2)} , \hdots , I_{(t)}, \hdots  \} \in [T] $ denotes the set of synchronization indices. For a parameter $p >0$, an increasing positive sequence $\{A_t\}_{t=0}^{T-1}$, constant stepsize $\eta$ with parameter $a \geq \frac{5H}{p}$ and arbitrary $b >0$, we have:
%	\begin{align*}
%	e_{I_{(t)}} \leq \frac{20}{p^2}A_{I_{(t)}}\eta_{I_{(t)}}^2
%	\end{align*}
%\end{lemma}
%\begin{proof}
%	f	
%\end{proof}

==> momentum_cvx.tex <==
%---------------------------------
%\section{Proof of Lemma}


%---------------------------------
{\allowdisplaybreaks
\section{Proof of Theorem \ref{thm_cvx_li} (Strongly-convex)} \label{proof_thm_cvx_li}

\begin{theorem*}[Restating Theorem \ref{thm_cvx_li} (Strongly-convex)]
	Suppose $f_i$, for all $i\in[n]$ be $L$-smooth and $\mu$-strongly convex. Let $\C$ be a compression operator with parameter equal to $\omega \in (0,1]$. Let $gap(\I_T)\leq H$. If we run SQuARM-SGD with consensus step-size $\gamma = \frac{2\delta \omega}{64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega}, (\text{where }\lambda = \text{max}_i \{ 1- \lambda_i(W) \})$, an increasing threshold function $c_t  \leq c_0t^{(1-\epsilon)} $ for all $t$ where constant $c_0 \geq 0$ and $\epsilon \in (0,1]$, momentum coefficient $\beta\in[0,1)$\footnote{Though we state and prove our main results for $c_t\leq c_0t^{(1-\epsilon)}$, they can be easily extended for an arbitrary threshold $c_t$, as long as $c_t=o(t)$, i.e., $c_t$ grows as a sub-linear function of $t$.}, and decaying learning rate $\eta_t = \frac{16(1-\beta)}{\mu(a+t)}$, where
	$a \geq \max \left\{  \frac{5H}{p}, \frac{128L}{\mu} , \frac{16(16L\beta^2)^2}{\mu (1-\beta)} \right\} $ for $p = \frac{\gamma\delta}{8}$, and let the algorithm generate $\{ \bx_i ^{(t)}  \}_{t=0}^{T-1}$ for $i\in[n]$, then the following holds:
	\begin{align*}
	\mathbb{E}f(\blx_{avg}^{(T)}) - f^* & \leq \frac{\mu a^3}{16S_T}\bbE\verts{{\blx}^{(0)} - \bx^*}^2 + \frac{Z_1 \bar{\sigma}^2T(T+2a)}{\mu nS_T} + \frac{Z_2 \beta^2G^2 (T+a)^{\nicefrac{3}{2}}}{(\mu^{\nicefrac{3}{2}}(1-\beta)^{\nicefrac{7}{2}}) S_T } \\
	& + \frac{Z_3(L+\mu)H\omega c_0}{\mu^2 p(2-\epsilon)} \frac{T^{(2-\epsilon)}}{S_T} + \frac{Z_4T}{\mu^2 S_T}\left[\frac{(L+ \mu)H^3 G^2}{p^2 (1-\beta)^2} + \frac{\mu\beta^4G^2}{2(1-\beta)^4}\right] 
	\end{align*}
	where $\blx^{(T)}_{avg} := \frac{1}{S_T} \sum_{t=0}^{T-1}w_t \bar{\bx}^{(t)}$, 
	where $\bar{\bx}^{(t)} = \frac{1}{n} \sum_{i=1}^{n} \bx^{(t)}_{i}$, weights $w_t = (a+t)^2$,  $S_T := \frac{T}{6} (2T^2+6aT-3T+6a^2-6a+1) \geq \frac{1}{3}T^3$ and $Z_1,Z_2,Z_3,Z_4$ are universal constants.
\end{theorem*}
\begin{proof}
In order to prove Theorem \ref{thm_cvx_li}, we define a virtual sequence ${\btx}_i^{(t)}$ for each node $i\in[n]$, as follows:
\begin{align} \label{virt_seq}
{\btx}_i^{(t)} = {\bx}_i^{(t)} - \frac{\eta_{t-1} \beta^2}{(1-\beta)} \bv_i^{(t-1)}.
\end{align}
%Proving convergence results by defining virtual sequences has been promising lately in stochastic optimization literature; see \cite{stich_sparsified_2018,alistarh_convergence_2018,stich-signsgd-19,basu_qsparse-local-sgd:_2019,distributed_momentum19} for instance. Our definition of virtual sequence \eqref{virt_seq} is inspired by \cite{distributed_momentum19}, which studies compressed {\em distributed SGD} with momentum for non-convex objectives only. However, our virtual sequence differs from theirs as they consider error compensated parameters to define this sequence, while we consider the true parameters at a node (${\bx}_i^{(t)}$) to define it. This is because we do not explicitly maintain an error vector to compensate the gradient updates and instead maintain copy of each node's parameters at its neighbors and communicate updates of these copies. Moreover, our proof is fundamentally different from \cite{distributed_momentum19}, as we are in a decentralized setup, and in addition to incorporating momentum, our algorithm also employs compression (both sparsification and quantization), local iterations, and event-triggered communication to save on communication bits.
%Also, in \cite{distributed_momentum19}, all the nodes have access to the same dataset, whereas, in our setup, all nodes have their own local datasets.
%
%%The proof of CHOCO-SGD in \cite{koloskova_decentralized_2019-1} is a bit related to this proof, as that paper also studies compressed decentralized optimization; however, though they incorporated momentum in their experiments, but left the theoretical analysis open; see also \cite{koloskova_decentralized_2019}. 
%
%Note that our proof is very different and significantly more involved than the proof of CHOCO-SGD in \cite{koloskova_decentralized_2019}.
%Some of the differences are as follows:
%{\sf (i)} Though CHOCO-SGD studied compression in a decentralized setting, they only incorporated momentum in their experiments and left the theoretical analysis open; see also \cite{koloskova_decentralized_2019}. 
%{\sf (ii)} Unlike CHOCO-SGD (which only employs either quantization {\em or} sparsification), we incorporate sparsification {\em and} quantization, local iterations, and event triggered communication to save on communication.
%{\sf (iii)} The proof of CHOCO-SGD did not have to use virtual sequences, whereas, to analyze our algorithm, we had to define virtual sequences (specifically, to handle the use of momentum) to prove the convergence result.
%
%All these factors make proving our convergence result with SGD like rate significantly more challenging than either of these papers, which is evident from the proof below as well as from the proof of Lemma \ref{lem_cvx}. As far as we know, this is the first paper that not only incorporates momentum in decentralized SGD, but also incorporate local iterations and event-triggered communication to further save on communication, and theoretically analyze the resulting algorithm.
%
%In order to be able to use the virtual sequence \eqref{virt_seq} (in particular, for establishing a recurrence relation), we crucially use the properties of the mixing matrix ${\bf W}$, as shown below.

In \eqref{virt_seq}, $\bx_i^{(t)}$ is the true local parameter at node $i$ at the $t$'th iteration, which is equal to (see line 16 of Algorithm \ref{alg_dec_sgd_li}):
\begin{align*}
\bx_i^{(t)} = \bx_i^{(t-\frac{1}{2})} + \mathbbm{1}_{(t) \in \mathcal{I}_T}\gamma \sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t)} - \hat{\bx}_i^{(t)}),
\end{align*}
where $\bx_i^{(t-\frac{1}{2})} = \bx_i ^{(t-1)} - \eta_{t-1} (\beta \bv_i^{(t-1)} + \nabla F_i(\bx_i^{(t-1)}, \xi_i^{(t-1)}))$ (line 5 in Algorithm \ref{alg_dec_sgd_li}).
Note that we changed the summation from $j\in\mathcal{N}_i$ to $j=1$ to $n$; this is because $w_{ij}=0$ whenever $j\notin\mathcal{N}_i$.

Let ${\blx}^{(t-1)} = \frac{1}{n} \sum_{i=1}^{n} \bx_{i}^{(t-1)}$ denote the average of the local iterates at time $t$.
Now we argue that ${\blx}^{(t)}={\blx}^{(t-\frac{1}{2})}$.
This trivially holds when $t\notin \I_T$. For the other case, i.e., $t\in \I_T$, this follows because
$\sum_{i=1}^n\sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t)} - \hat{\bx}_i^{(t)})=0$, which uses the fact that $W$ is a doubly stochastic matrix. 
Thus, we have 
\begin{equation}\label{eq:thm_cvx_interim0}
{\blx}^{(t)} =  {\blx}^{(t-1)} - \frac{\eta_{t-1}}{n}\sum_{i=1}^n \left(\beta \bv_i^{(t-1)} + \nabla F_i(\bx_i^{(t-1)}, \xi_i^{(t-1)})\right).
\end{equation}
Taking average over all the nodes in \eqref{virt_seq} and defining ${\btx}^{(t)} := \frac{1}{n}\sum_{i=1}^n{\btx}_i^{(t)}$, we get
\begin{align*}
{\btx}^{(t)} = {\blx}^{(t)} - \frac{\eta_{t-1} \beta^2}{(1-\beta)} \frac{1}{n} \sum_{i=1}^n \bv_i^{(t-1)}.
\end{align*}
%Note that the columns of ${\btX}^{(t+1)}$ are identical and equal to $\btx^{(t)}$. 
We now note a recurrence relation for the sequence ${\btx}^{(t+1)}$:
\begin{align} \label{virt_seq_rec}
{\btx}^{(t+1)} & = {\blx}^{(t+1)} - \frac{\eta_t \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n \bv_i^{(t)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta_t}{n}\sum_{i=1}^n \left(\beta \bv_i^{(t)} + \nabla F_i(\bx_i^{(t)}, \xi_i^{(t)})\right) - \frac{\eta_t \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n \bv_i^{(t)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta_t}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) -  \left( \eta_t \beta + \frac{\eta_t \beta^2}{(1-\beta)}\right)  \frac{1}{n}\sum_{i=1}^n \bv_i^{(t)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta_t}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) - \frac{\eta_t \beta}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n\left[ \frac{\eta_{t-1}}{\eta_t} \beta\bv_i^{(t-1)}  + \nabla F_i(\bx_i^{(t)},\xi_i^{(t)})\right] \notag \\
& =  {\blx}^{(t)} - \left(\eta_t + \frac{\eta_t\beta}{(1-\beta)} \right)\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) - \frac{\eta_{t-1} \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n\bv_i^{(t-1)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta_{t-1} \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n\bv_i^{(t-1)} - \frac{\eta_t}{(1-\beta)}\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) \notag \\
& =  {\btx}^{(t)} - \frac{\eta_t}{(1-\beta)}\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)})
\end{align}
%--------------------------------------------------------------------------------
%Consider expectation taken over sampling at time instant $t$: ${\boldsymbol{\xi}^{(t)}} = \{ \xi_1^{(t)}, \xi_2^{(t)}, \hdots, \xi_n^{(t)} \}$ and using $\Bar{\bX}^{(t)}  = \Bar{\bX}^{(t+\frac{1}{2})} $ (from (\ref{mean_seq_iter})) which gives: $ \Bar{\bx}^{(t+1)} =  \frac{1}{n}\sum_{j=1}^n \nabla F_j(\bx_j^{(t)},\xi_j^{(t)}) $ ,  we have:
Now, consider $\mathbb{E}_{\boldsymbol{\xi}^{(t)}}\|\btx^{(t+1)} - \bx^*\|^2$ (we shall form a recurrence relation), where expectation is taken over sampling across all the nodes at the $t$'th iteration:
\begin{align}
\mathbb{E}_{\boldsymbol{\xi}^{(t)}}& \Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^ 2 
=  \mathbb{E}_{\boldsymbol{\xi}^{(t)}} \left\Vert \tilde{\bx}^{(t)} - \frac{\eta_t}{(1-\beta)  n}\sum_{j=1}^n \nabla F_j(\bx_j^{(t)},\xi_j^{(t)}) - \bx^* \right\Vert^2  \notag\\
& = \mathbb{E}_{\boldsymbol{\xi}^{(t)}} \left\Vert \tilde{\bx}^{(t)} - \bx^* - \frac{\eta_t}{(1-\beta) n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) + \frac{\eta_t}{ (1-\beta) n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) - \frac{\eta_t}{n (1-\beta) }\sum_{j=1}^n \nabla F_j(\bx_j^{(t)},\xi_j^{(t)})  \right\Vert^2  \notag\\
& =  \left\Vert \tilde{\bx}^{(t)} - \bx^* - \frac{\eta_t}{ (1-\beta) n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) \right\Vert^2 + \frac{\eta_t^2}{(1-\beta)^2}  \mathbb{E}_{\boldsymbol{\xi}^{(t)}} \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla F_j(\bx_j^{(t)},\xi_j^{(t)}) \right\Vert^2 \notag\\
& \hspace{1cm} + \frac{2\eta_t}{ (1-\beta) n}\mathbb{E}_{\boldsymbol{\xi}^{(t)}} \left\langle \tilde{\bx}^{(t)} - \bx^* - \frac{\eta_t}{ (1-\beta) n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) , \sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) - \sum_{j=1}^n \nabla F_j(\bx_j^{(t)},\xi_j^{(t)}) \right\rangle \label{suppl_cvx_lemm_total0} \\
&\leq \left\Vert \tilde{\bx}^{(t)} - \bx^* - \frac{\eta_t}{ (1-\beta) n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) \right\Vert^2 + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n}
\label{suppl_cvx_lemm_total}
\end{align}
Note the last term of \eqref{suppl_cvx_lemm_total0} is zero as $\mathbb{E}_{\xi_i^{(t)}} \nabla F_i(\bx_i^{(t)}, \xi_i^{(t)}) = \nabla f_i(\bx_i^{(t)}) $ for all $i \in [n]$. 
The second term in \eqref{suppl_cvx_lemm_total0} can be bounded via the variance bound (\ref{bound_var}) by $ \frac{\eta_t^2 \bar{\sigma}^2}{n}$.
Now we thus consider the first term in the \eqref{suppl_cvx_lemm_total} :
\begin{align} \label{suppl_cvx_lemm_firstterm}
\left\Vert \tilde{\bx}^{(t)} - \bx^* - \frac{\eta_t}{(1-\beta)n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) \right\Vert^2 = \Vert \tilde{\bx}^{(t)} - \bx^* \Vert^2 + \frac{\eta_t^2}{(1-\beta)^2}  \underbrace{\left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) \right\Vert^2}_{T_1} \notag \\
- \frac{2\eta_t}{(1-\beta)} \underbrace{ \left\langle \tilde{\bx}^{(t)} - \bx^*,\frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)}) \right\rangle}_{T_2}
\end{align}
To bound $T_1$ in (\ref{suppl_cvx_lemm_firstterm}), note that:
\begin{align}
T_1 &= \left\Vert \frac{1}{n}\sum_{j=1}^n (\nabla f_j(\bx_j^{(t)}) - \nabla f_j(\Bar{\bx}^{(t)}) + \nabla f_j(\Bar{\bx}^{(t)}) - \nabla f_j(\bx^*) ) \right\Vert^2  \notag \\
& \leq \frac{2}{n}\sum_{j=1}^n \Vert \nabla f_j(\bx_j^{(t)}) - \nabla f_j(\Bar{\bx}^{(t)}) \Vert^2 + 2 \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\Bar{\bx}^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx^*) \right\Vert^2  \notag \\
%	\intertext{Using strong convexity of $f$, optimality of $\bx^*$ and $L-$smoothness property (\ref{l_smooth_prop}) of $f_j$ , and by noting that  :  $$ \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\Bar{\bx}^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx^*) \right\Vert^2 \leq \frac{1}{n} \sum_{j=1}^n \Vert \nabla f_j(\Bar{\bx}^{(t)}) -  \nabla f_j(\bx^*) \Vert^2  \leq \frac{1}{n} \sum_{j=1}^n 2L (f_j(\Bar{\bx}^{(t)}) - f_j(\bx^*)) $$ , }
%	& \stackrel{(a)}{\leq} \frac{2L^2}{n}\sum_{j=1}^n \Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2 + \frac{4L}{n} \sum_{j=1}^n (f_j(\Bar{\bx}^{(t)}) - f_j(\bx^*))  \notag \label{suppl_cvx_t1_bound} \\
& \leq \frac{2L^2}{n}\sum_{j=1}^n \Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2 + 4L  (f(\Bar{\bx}^{(t)}) - f^*)  \label{suppl_cvx_t1_bound}
\end{align}
where in the last inequality, we've used $L-$Lipschitz gradient property of $f_j's$ to bound the first term and optimality of $\bx^*$ for $f$ (i.e., $\nabla f(\bx^*) = 0$) and $L-$smoothness property (\ref{l_smooth_prop}) of $f$  to bound the second term as:
$ \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\Bar{\bx}^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx^*) \right\Vert^2 = \verts{ \nabla f (\Bar{\bx}^{(t)} ) - \nabla f (\bx^*)  }^2   \leq 2L \left( f(\Bar{\bx}^{(t)} ) -f^*  \right) $.\\
%	  \frac{1}{n} \sum_{j=1}^n \Vert \nabla f_j(\Bar{\bx}^{(t)}) -  \nabla f_j(\bx^*) \Vert^2  \leq \frac{1}{n} \sum_{j=1}^n 2L (f_j(\Bar{\bx}^{(t)}) - f_j(\bx^*)) $$
To bound $T_2$ in (\ref{suppl_cvx_lemm_firstterm}), note that: 
\begin{align}
-2T_2 & = - 2 \lragnle{\btx^{(t)}  -\blx^{(t)} , \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})    } - \frac{2}{n} \sum_{j=1}^n \lragnle{\blx^{(t)}  - \bx^* ,  \nabla f_j(\bx_j^{(t)})} \notag \\
%& = - 2 \lragnle{\tilde{x}^{(t)}  -\bar{x}^{(t)} , \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})    } - \frac{2}{n} \sum_{j=1}^n \lragnle{\bar{x}^{(t)}  - x^{(t)}_j ,  \nabla f_j(\bx_j^{(t)})    } \notag \\
& = 2\frac{\beta^2}{(1-\beta)} \lragnle{ \frac{\eta_{t-1}}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}   , \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})} - \frac{2}{n} \sum_{j=1}^n \lragnle{\blx^{(t)}  - \bx^*,  \nabla f_j(\bx_j^{(t)})    }  \label{eq:mom_cvx_interim2}
\end{align}
In \eqref{eq:mom_cvx_interim2}, we used the definition of $\btx^{(t)}$ from \eqref{virt_seq} to write $\btx^{(t)} - \blx^{(t)} = - \frac{\eta_{t-1}\beta^2}{(1-\beta)}\frac{1}{n}\sum_{i=1}^n\bv_i^{(t-1)}$. 
Now we note a simple trick for inner-products: 
\begin{align}
\lragnle{\frac{\eta_{t-1}}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}, \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})} = \lragnle{ \frac{(\eta_{t-1})^{\nicefrac{3}{4}}}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}, \frac{(\eta_{t-1})^{\nicefrac{1}{4}}}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})}. \label{eq:mom_cvx_interim_3}
\end{align}
This trick is crucial to getting a speedup of $n$ -- the number of worker nodes -- in our final convergence rate.
Using $2\langle {\bf a}, {\bf b} \rangle \leq \|{\bf a}\|^2 + \|{\bf b}\|^2$ for bounding \eqref{eq:mom_cvx_interim_3} and then substituting that in \eqref{eq:mom_cvx_interim2} gives
\begin{align}
-2T_2 &\leq 
%\frac{\beta^2}{(1-\beta)}\left[\left\|\frac{(\eta_{t-1})^{\nicefrac{3}{4}}}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}\right\|^2 + \left\|\frac{(\eta_{t-1})^{\nicefrac{1}{4}}}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})\right\|^2\right] \notag \\
%&\hspace{2cm} - \frac{2}{n} \sum_{j=1}^n \lragnle{\blx^{(t)}  - \bx^* ,  \nabla f_j(\bx_j^{(t)})}  \notag \\
%&= 
\frac{\beta^2}{(1-\beta)}\left[(\eta_{t-1})^{\nicefrac{3}{2}}\left\|\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}\right\|^2 + (\eta_{t-1})^{\nicefrac{1}{2}} \left\|\frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})\right\|^2\right]  - \frac{2}{n} \sum_{j=1}^n \lragnle{\blx^{(t)}  - \bx^* ,  \nabla f_j(\bx_j^{(t)})} \label{eq:mom_cvx_interim_4}
\end{align}
%Using Cauchy-Schwarz inequality to bound the first term, we have:
%\begin{align}
%-\frac{(1-\beta)}{\eta_t}T_2 & = \frac{2\eta_{t-1} \beta^2}{(1-\beta)} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)} }  \verts{ \frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})    } - \frac{2}{n} \sum_{j=1}^n \lragnle{\blx^{(t)}  - \bx^{(t)}_j ,  \nabla f_j(\bx_j^{(t)})    } 
%\end{align}
Note that the second term of \eqref{eq:mom_cvx_interim_4} is the same as $T_1$ from \eqref{suppl_cvx_lemm_firstterm} and we have already bounded that in \eqref{suppl_cvx_t1_bound}.
We now focus on bounding the last term of \eqref{eq:mom_cvx_interim_4}. Using expression for $\mu$-strong convexity (\ref{mu_strong_cvx}) and $L$-smoothness (\ref{l_smooth}) for $f_j , \, j \in [n] $ respectively, we can bound this as follows  : 
\begin{align} 
\frac{-2}{n} \sum_{j=1}^n \langle \blx^{(t)}  - & \bx^*,   \nabla f_j(\bx_j^{(t)})  \rangle  = -\frac{2}{n} \sum_{j=1}^n \left[ \left\langle \Bar{\bx}^{(t)} - \bx_j^{(t)}, \nabla f_j(\bx_j^{(t)}) \right\rangle + \left\langle \bx_j^{(t)} - \bx^*, \nabla f_j(\bx_j^{(t)}) \right\rangle \right] \notag  \\
& \leq -\frac{2}{n} \sum_{j=1}^n \left[  f_j(\Bar{\bx}^{(t)}) - f_j(\bx_j^{(t)}) - \frac{L}{2}\Vert \Bar{\bx}^{(t)} - \bx_j^{(t)}  \Vert^2  + f_j(\bx_j^{(t)}) - f_j(\bx^*) + \frac{\mu}{2}\Vert \bx_j^{(t)} - \bx^*  \Vert^2 \right] \notag \\
& = -2  (f(\Bar{\bx}^{(t)}) - f(\bx^*)) + \frac{L+ \mu}{n}\sum_{j=1}^n \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)}  \Vert^2   - \frac{\mu}{n} \sum_{j=1}^n \left[\Vert \Bar{\bx}^{(t)} - \bx_j^{(t)}  \Vert^2  +  \Vert \bx_j^{(t)} - \bx^*  \Vert^2 \right] \notag \\
& \leq  -2  (f(\Bar{\bx}^{(t)}) - f(\bx^*)) + \frac{L+ \mu}{n}\sum_{j=1}^n \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)}  \Vert^2   - \frac{\mu}{2n} \sum_{j=1}^n \left[\Vert \Bar{\bx}^{(t)} - \bx^*  \Vert^2 \right] \notag \\
& =  -2  (f(\Bar{\bx}^{(t)}) - f(\bx^*)) + \frac{L+ \mu}{n}\sum_{j=1}^n \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)}  \Vert^2   - \frac{\mu}{2} \Vert \Bar{\bx}^{(t)} - \bx^*  \Vert^2  \label{eq:mom_cov_interim_3} \\
& \leq -2  (f(\Bar{\bx}^{(t)}) - f(\bx^*)) + \frac{L+ \mu}{n}\sum_{j=1}^n \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)}  \Vert^2   - \frac{\mu}{2}\left( \frac{\|\btx^{(t)} - \bx^*\|^2}{2} - \|\btx^{(t)} - \blx^{(t)}\|^2 \right)\label{suppl_cvx_t2part_bound}
\end{align}
In \eqref{suppl_cvx_t2part_bound}, we used $\|\btx^{(t)} - \bx^*\|^2 \leq  2\|\btx^{(t)} - \blx^{(t)}\|^2 + 2\Vert \Bar{\bx}^{(t)} - \bx^*  \Vert^2$.
Substituting the bounds for the second and the last terms of \eqref{eq:mom_cvx_interim_4} from \eqref{suppl_cvx_t1_bound} and \eqref{suppl_cvx_t2part_bound}, respectively, we get
\begin{align*} 
-2T_2  & \leq \frac{(\eta_{t-1})^{\nicefrac{3}{2}}\beta^2}{(1-\beta)} \left\|\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}\right\|^2 + \frac{(\eta_{t-1})^{\nicefrac{1}{2}}\beta^2}{(1-\beta)}\left( \frac{2L^2}{n}\sum_{j=1}^n \Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2 + 4L  (f(\Bar{\bx}^{(t)}) - f^*)\right) \notag \\
& \hspace{1cm} - 2  (f(\Bar{\bx}^{(t)}) - f(\bx^*)) + \frac{L+ \mu}{n}\sum_{j=1}^n \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)}  \Vert^2   - \frac{\mu}{4}\|\btx^{(t)} - \bx^*\|^2 + \frac{\mu}{2}\|\btx^{(t)} - \blx^{(t)}\|^2
\end{align*}
%Note that by Jensen's inequality and the gradient bound \eqref{bound_grad}:
% $$\TODO{\verts{\frac{1}{n}\sum_{j=1}^n \nabla f_j(\bx_j^{(t)})}_2 = \verts{\mathbb{E} [\frac{1}{n}\sum_{j=1}^n \nabla F_j(\bx_j^{(t)}, \xi^{(t)}_j)]}_2 \leq \mathbb{E}\verts{\frac{1}{n}\sum_{j=1}^n \nabla F_j(\bx_j^{(t)}, \xi^{(t)}_j)}_2 \leq G }$$
By clubbing similar terms together and using $\eta_{t-1} \leq 2\eta_t$ (which implies $\eta_{t-1}^{\nicefrac{3}{2}} \leq 4\eta_{t}^{\nicefrac{3}{2}}$ and $\eta_{t-1}^{\nicefrac{1}{2}} \leq 2\eta_{t}^{\nicefrac{1}{2}}$), we have:
\begin{align}%\label{suppl_cvx_t2_bound}
& -\frac{2\eta_t}{(1-\beta)}T_2 \leq \notag \\
&  \frac{4\eta_{t}^{\nicefrac{5}{2}}\beta^2}{(1-\beta)^2} \left\|\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}\right\|^2 + \left(\frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^22L^2}{(1-\beta)^2} + \frac{\eta_t(L + \mu)}{(1-\beta)} \right)\frac{1}{n}\sum_{j=1}^n \Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2 \notag \\
& + \left(\frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2} - \frac{2\eta_t}{(1-\beta)}\right)\left(f(\blx^{(t)}) - f^*\right) - \frac{ \eta_t}{(1-\beta)} \frac{\mu}{4} \Vert \btx^{(t)} - \bx^*  \Vert^2 + \frac{ \eta_t}{(1-\beta)} \frac{\mu}{2} \Vert \btx^{(t)} - \blx^{(t)}  \Vert^2 \label{eq:mom_cvx_interim_5}
\end{align}
Substituting \eqref{suppl_cvx_t1_bound}, \eqref{eq:mom_cvx_interim_5} in \eqref{suppl_cvx_lemm_firstterm} and using the resulting bound back in \eqref{suppl_cvx_lemm_total}, and then taking expectation w.r.t.\ the entire process, we get:
\begin{align} 
\mathbb{E}\Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 + \frac{4\eta_{t}^{\nicefrac{5}{2}}\beta^2}{(1-\beta)^2} \bbE\left\|\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}\right\|^2 + \frac{\mu\eta_t}{2(1-\beta)}\bbE \Vert \btx^{(t)} - \blx^{(t)}  \Vert^2 \notag \\ 
& + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n}+ \left(\frac{2\eta_t^2L^2}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^22L^2}{(1-\beta)^2} + \frac{\eta_t(L + \mu)}{(1-\beta)} \right)\frac{1}{n}\sum_{j=1}^n \bbE\Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2 \notag \\
&\hspace{2cm} + \left(\frac{4\eta_t^2L}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2} - \frac{2\eta_t}{(1-\beta)}\right)\left(\bbE f(\blx^{(t)}) - f^*\right)  \label{eq:mom_cvx_interim1}
%&= \Vert \tilde{\bx}^{(t)} - \bx^* \Vert^2 - \left(\frac{\eta_t \mu}{2(1-\beta)} \right) \Vert \Bar{\bx}^{(t)} - \bx^* \Vert^2 + \frac{\eta_t^2 \Bar{\sigma}^2}{n} - 2\eta_t \left( \frac{1}{(1-\beta)} -\frac{2L\eta_t}{(1-\beta)^2}\right) (f(\Bar{\bx}^{(t)}) - f^*) \notag \\
%&\qquad + \eta_t \left(  \frac{2\eta_t L^2 }{n(1-\beta)^2} + \frac{ L + \mu}{(1-\beta)n }  \right) \sum_{j=1}^n \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)} \Vert^2 + \frac{2\eta_{t-1} \eta_t \beta^2G}{(1-\beta)^2} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)} }
\end{align}
%We now expand the second term in the RHS of above. For some constant $\alpha_1 > 0$, we have:
%\begin{align*}
%	\verts{\bar{x}^{(t)} - x^* }^2 \geq \frac{\verts{\tilde{x}^{(t)} - x^*}^2}{(1+\alpha_1)} - \frac{(1+\alpha^{-1}_1)}{(1+\alpha_1)} \verts{\tilde{x}^{(t)}  -\bar{x}^{(t)}      }     
%\end{align*}
%Using the above bound in \eqref{mom_cvx_interim1} we have:
%\begin{align*}
%\mathbb{E}_{\boldsymbol{\xi}^{(t)}} \Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq 
%\left( 1 - \frac{\mu \eta_t}{2 (1+\alpha_1)(1-\beta) }  \right)\Vert \tilde{\bx}^{(t)} - \bx^* \Vert^2 + \frac{\eta_t \mu}{2(1-\beta)}   \frac{(1+\alpha^{-1}_1)}{(1+\alpha_1)}    \Vert \tilde{\bx}^{(t)} - \bar{\bx}^{(t)} \Vert^2 \\
%& \qquad - 2\eta_t \left( \frac{1}{(1-\beta)} -\frac{2L\eta_t}{(1-\beta)^2}\right) (f(\Bar{\bx}^{(t)}) - f^*) + \frac{\eta_t^2 \Bar{\sigma}^2}{n}   \\
%&\qquad + \eta_t \left(  \frac{2\eta_t L^2 }{n(1-\beta)^2} + \frac{ L + \mu}{(1-\beta)n }  \right) \sum_{j=1}^n \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)} \Vert^2 + \frac{2\eta_{t-1} \eta_t \beta^2G}{(1-\beta)^2} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)} }
%\end{align*}
%This completes the proof of the lemma. 
\begin{lemma} \label{glob_virt_bound_cvx}
	Consider the deviation of the global average parameter $\bar{x}^{(t)}$  and the virtual sequence $\tilde{x}^{(t)}$ defined in \eqref{virt_seq}. Then at any time step $t$ of the Algorithm, the following holds:
	\begin{align}
	\mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv^{(t-1)}_i}^2 &\leq \frac{9G^2}{(1-\beta)^4} \label{glob_virt_bound_cvx1} \\
	 \mathbb{E}\verts{ \blx^{(t)} -  \btx^{(t)}}^2 &\leq \frac{9\beta^4 \eta_t^2 G^2}{(1-\beta)^6}  \label{glob_virt_bound_cvx2}
	\end{align}
\end{lemma}
\begin{proof}
Using the definition of $\btx^{(t)}$ as in \eqref{virt_seq}, we have:
\begin{align}\label{glob_virt_bound_cvx_interim1}
\mathbb{E} \verts{ \blx^{(t)} -  \btx^{(t)}}^2 &  =  \frac{ \beta^4 \eta_{t-1}^2}{(1-\beta)^2} \mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv^{(t-1)}_i}^2 
\end{align}
By the Jensen's inequality, we can write $\mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv^{(t-1)}_i}^2 \leq \frac{1}{n} \sum_{i=1}^{n}\mathbb{E} \verts{ \bv^{(t-1)}_i}^2$. We have already proved in \eqref{bound_v_it} that for every $i\in[n]$ and $t\geq 1$, we have $\mathbb{E} \verts{ \bv_i^{(t)}}^2 \leq \frac{9G^2}{(1-\beta)^4}$. Thus we have $\mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv^{(t-1)}_i}^2 \leq \frac{9G^2}{(1-\beta)^4}$, which proves \eqref{glob_virt_bound_cvx1}. 
Substituting this in \eqref{glob_virt_bound_cvx_interim1} proves \eqref{glob_virt_bound_cvx2}.
This completes the proof of Lemma \ref{glob_virt_bound_cvx}.
%\iffalse
%Now we bound $\mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv^{(t-1)}_i}^2$.
%Define $\theta_{t-1} = \sum_{k=0}^{t-1} \beta^{t-1-k} = \frac{1-\beta^t}{1-\beta}$.
%\begin{align*}
%\mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv^{(t-1)}_i}^2 & =\theta_{t-1}^2  \mathbb{E}\verts{  \sum_{k=0}^{t-1} \frac{\beta^{t-1-k}}{\theta_{t-1}}  \frac{1}{n} \sum_{i=1}^{n} \nabla F(x_i^{(k)}, \xi_i^{(k)})  }^2 \\
%	& \leq \theta_{t-1}^2   \sum_{k=0}^{t-1} \frac{\beta^{t-1-k}}{\theta_{t-1}}  \mathbb{E} \verts{ \frac{1}{n} \sum_{i=1}^{n} \nabla F(x_i^{(k)}, \xi_i^{(k)})  }^2 \\
%	& = \theta_{t-1}   \sum_{k=0}^{t-1} \beta^{t-1-k}  \mathbb{E} \verts{ \frac{1}{n} \sum_{i=1}^{n} \nabla F(x_i^{(k)}, \xi_i^{(k)})  }^2 \\
%	& \leq \frac{1}{(1-\beta)}  \sum_{\tau=0}^{t-1} \left[\beta^{t-\tau-1} \mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (x^{(\tau)}_i , \xi^{(\tau)}_i ) }^2\right] \\
%& \leq \frac{G^2}{(1-\beta)^2} 
%\end{align*}
%Where the first inequality follows from  Jensen's inequality, the second inequality follows from noting that $\theta_{t} \leq \frac{1}{1-\beta}$ and the last inequality follows from the bounded gradient assumption \eqref{bound_grad}. Substituting this in \eqref{glob_virt_bound_cvx_interim1} proves \eqref{glob_virt_bound_cvx2}.
%This completes the proof of Lemma \ref{glob_virt_bound_cvx}.
%\fi
\end{proof}

Using \eqref{glob_virt_bound_cvx1} and \eqref{glob_virt_bound_cvx2} in \eqref{eq:mom_cvx_interim1} gives 
\begin{align} 
\mathbb{E}\Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} + \frac{9\mu\beta^4\eta_t^3G^2}{2(1-\beta)^7} + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n}\notag \\ 
&\hspace{1cm} + \left(\frac{2\eta_t^2L^2}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^22L^2}{(1-\beta)^2} + \frac{\eta_t(L + \mu)}{(1-\beta)} \right)\frac{1}{n}\sum_{j=1}^n \bbE\Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2 \notag \\
&\hspace{2cm} + \left(\frac{4\eta_t^2L}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2} - \frac{2\eta_t}{(1-\beta)}\right)\left(\bbE f(\blx^{(t)}) - f^*\right)  \label{mom_cvx_interim_5}
\end{align}

%{\color{magenta}Note that for appropriate choice of $\eta_t$, the coefficients of $\frac{1}{n}\sum_{j=1}^n \bbE\Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2$ and $\bbE f(\blx^{(t)}) - f^*$ will be some constant times $\eta_t$. Also, note that there is only one term with $\eta_t^2$ that is $\frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n}$, with division by $n$.} \\ 
If we take $\eta_t \leq \min \left\{ \frac{(1-\beta)}{8L} , \frac{(1-\beta)^2}{(16L\beta^2)^2}   \right\}$, which can be achieved for $\eta_t = \frac{16(1-\beta)}{\mu(t+a)}$ by having $a \geq  \max \left\{  \frac{5H}{p}, \frac{128L}{\mu} , \frac{16(16L\beta^2)^2}{\mu (1-\beta)} \right\} $, then we have
\begin{align}
\left(\frac{2\eta_t^2 L^2}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^22L^2}{(1-\beta)^2} + \frac{\eta_t(L + \mu)}{(1-\beta)} \right) &\leq \frac{\eta_t(3L+ 2\mu)}{2(1-\beta)} \label{mom_cvx_bound1} \\
\left(\frac{4\eta_t^2L}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2} - \frac{2\eta_t}{(1-\beta)}\right) &\leq -\frac{\eta_t}{(1-\beta)} \label{mom_cvx_bound2}
\end{align}

\iffalse
We now consider the factor $\left(\frac{4\eta_t^2L}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2} - \frac{2\eta_t}{(1-\beta)}\right) $ multiplied with the last term. To have the value of this factor $\leq -\eta_t$, it suffices to show that:
\begin{align*}
	\left(  \frac{2\eta_t}{(1-\beta)} - \frac{4\eta_t^2L}{(1-\beta)^2} - \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2}  \right) \geq \frac{1}{(1-\beta)}
\end{align*}
where $\beta \leq 1$ implies that the LHS above is $\geq 1$. For the above equation to hold, a sufficient condition is:
\begin{align*}
	\frac{4\eta_t^2L}{(1-\beta)^2}  \leq \frac{1}{2(1-\beta)} \hspace{0.3cm} \text{and} \hspace{0.3cm} \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2} \leq \frac{1}{2(1-\beta)} 
\end{align*}
which is satisfied if   $\eta_t \leq \frac{(1-\beta)}{8L}$ and $\eta_t^{\nicefrac{1}{2}} \leq \frac{(1-\beta)}{16L\beta^2} $. Thus we want  $\eta_t \leq \min \left\{ \frac{(1-\beta)}{8L} , \frac{(1-\beta)^2}{256L^2\beta^4}   \right\} $ which can be achieved for $\eta_t := \frac{8}{\mu(t+a)}$ by having $a \geq  \max \left\{  \frac{5H}{p}, \frac{64L}{\mu (1-\beta)} , \frac{2048L^2 \beta^4 }{\mu (1-\beta)^2} \right\} $. Thus we have $\left(\frac{4\eta_t^2L}{(1-\beta)^2} + \frac{2\eta_{t}^{\nicefrac{3}{2}}\beta^24L}{(1-\beta)^2} - \frac{2\eta_t}{(1-\beta)}\right) \leq - \eta_t$  and using it in \eqref{mom_cvx_interim_5} gives us :
\fi

Substituting the bounds from \eqref{mom_cvx_bound1} and \eqref{mom_cvx_bound2} to \eqref{mom_cvx_interim_5} gives
\begin{align} 
\mathbb{E}\Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} + \frac{9\mu\beta^4\eta_t^3G^2}{2(1-\beta)^7} + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
&\hspace{1cm} + \frac{\eta_t(3L+ 2\mu)}{2(1-\beta)}\frac{1}{n}\sum_{j=1}^n \bbE\Vert \bx_j^{(t)} - \Bar{\bx}^{(t)} \Vert^2 - \frac{\eta_t}{(1-\beta)} \left(\bbE f(\blx^{(t)}) - f^*\right)  \label{mom_cvx_interim6}
\end{align}
%---------------------------------------------------
%Take expectation in \eqref{eq:mom_cvx_interim1} w.r.t.\ to the whole process, and noting that $\eta_{t-1} \leq 2 \eta_t $, we have:
%\begin{align} \label{mom_cvx_interim3}
%\mathbb{E} \Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq 
%\left( 1 - \frac{\mu \eta_t}{2 (1+\alpha_1)(1-\beta) }  \right) \mathbb{E} \Vert \tilde{\bx}^{(t)} - \bx^* \Vert^2 + \frac{\eta_t \mu}{2(1-\beta)}   \frac{(1+\alpha^{-1}_1)}{(1+\alpha_1)}    \mathbb{E} \Vert \tilde{\bx}^{(t)} - \bar{\bx}^{(t)} \Vert^2 \notag \\
%& \qquad - 2\eta_t \left( \frac{1}{(1-\beta)} -\frac{2L\eta_t}{(1-\beta)^2}\right) (\mathbb{E} f(\Bar{\bx}^{(t)}) - f^*) + \frac{\eta_t^2 \Bar{\sigma}^2}{n}   \notag \\
%&\qquad + \eta_t \left(  \frac{2\eta_t L^2 }{n(1-\beta)^2} + \frac{ L + \mu}{(1-\beta)n }  \right) \sum_{j=1}^n \mathbb{E} \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)} \Vert^2 + \frac{4 \eta_t^2 \beta^2G}{(1-\beta)^2} \mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)} }
%\end{align}
%We can use Lemma \ref{glob_virt_bound_cvx} and use the fact that $\eta_{t-1} \leq 2 \eta_t $ to bound the second term in RHS of \eqref{mom_cvx_interim3}. The last term can be bounded by induction argument and using the bounded gradient assumption. This gives us:
%\begin{align}
%\mathbb{E} \Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq 
%\left( 1 - \frac{\mu \eta_t}{2 (1+\alpha_1)(1-\beta) }  \right) \mathbb{E} \Vert \tilde{\bx}^{(t)} - \bx^* \Vert^2 + \frac{2 \eta_t \mu}{(1-\beta)}   \frac{(1+\alpha^{-1}_1)}{(1+\alpha_1)} \frac{G^2n \beta^4 \eta_t^2}{(1-\beta)^4} \notag \\
%& \qquad - 2\eta_t \left( \frac{1}{(1-\beta)} -\frac{2L\eta_t}{(1-\beta)^2}\right) (\mathbb{E} f(\Bar{\bx}^{(t)}) - f^*) + \frac{\eta_t^2 \Bar{\sigma}^2}{n}   \notag \\
%&\qquad + \eta_t \left(  \frac{2\eta_t L^2 }{n(1-\beta)^2} + \frac{ L + \mu}{(1-\beta)n }  \right) \sum_{j=1}^n \mathbb{E} \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)} \Vert^2 + \frac{4 \eta_t^2 \beta^2G^2}{(1-\beta)^3}  \notag
%\end{align}
%For $\eta_t = \frac{8}{\mu (a+t)}$ and $a \geq \max \{  \frac{32L}{\mu (1-\beta^2)} ,\frac{5H}{p} \}$, we have $\eta_t \leq \frac{(1-\beta^2)}{4L} \leq \frac{1}{4L} $. This implies that:  $\left( \frac{1}{(1-\beta)} -\frac{2L\eta_t}{(1-\beta)^2}\right)  \geq \frac{1}{2}  $ and $\left(  \frac{2\eta_t L^2 }{n(1-\beta)^2} + \frac{ L + \mu}{(1-\beta)n }  \right) \leq \frac{2L+\mu}{n(1-\beta)} $, Thus we have:
%\begin{align} \label{mom_cvx_interim4}
%	\mathbb{E} \Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq 
%	\left( 1 - \frac{\mu \eta_t}{2 (1+\alpha_1)(1-\beta) }  \right) \mathbb{E} \Vert \tilde{\bx}^{(t)} - \bx^* \Vert^2 + \frac{2 \eta_t \mu}{(1-\beta)}   \frac{(1+\alpha^{-1}_1)}{(1+\alpha_1)} \frac{G^2n \beta^4 \eta_t^2}{(1-\beta)^4} \notag \\
%	& \qquad - \eta_t  (\mathbb{E} f(\Bar{\bx}^{(t)}) - f^*) + \frac{\eta_t^2 \Bar{\sigma}^2}{n}   \notag \\
%	&\qquad + \eta_t \left(  \frac{2L+\mu}{n(1-\beta)}  \right) \sum_{j=1}^n \mathbb{E} \Vert \Bar{\bx}^{(t)} - \bx_j^{(t)} \Vert^2 + \frac{4 \eta_t^2 \beta^2G^2}{(1-\beta)^3}
%\end{align}
Note that in our matrix form, $ \mathbb{E}\verts{\bar{\bX}^{(t)} - \bX^{(t)} }_F^2 = \sum_{i=1}^{n} \mathbb{E}\verts{ \bx^{(t)}_i -  \bar{\bx}^{(t)}}^2$. Let $I_{(t+1)_0} \in \mathcal{I}_T$ denote the latest synchronization step before or equal to $(t+1)$. Then we have:
\begin{align*}
\bX^{(t+1)} & = \bX^{I_{(t+1)_0}} - \textstyle \sum_{t' = I_{(t+1)_0}}^{t}\eta_{t'} ( \beta \bV^{(t)} +\partial F(\bX^{(t')}, \boldsymbol{\xi}^{(t')} )) \\
\Bar{\bX}^{(t+1)} & = \bar{\bX}^{I_{(t+1)_0}} - \textstyle \sum_{t' = I_{(t+1)_0}}^{t}\eta_{t'} ( \beta \bV^{(t)} +\partial F(\bX^{(t')}, \boldsymbol{\xi}^{(t')} )) \frac{{\bf 1}{\bf 1}^T}{n} 
\end{align*} 
Thus the following holds:
\begin{align*}
\mathbb{E} & \Vert \bX^{(t+1)} -  \Bar{\bX}^{(t+1)} \Vert_F^2  = \mathbb{E} \left\Vert \bX^{I_{(t+1)_0}} - \Bar{\bX}^{I_{(t+1)_0}} -\sum_{t' = I_{(t+1)_0}}^{t} \eta_{t'} ( \beta \bV^{(t)} +\partial F(\bX^{(t')}, \boldsymbol{\xi}^{(t')} )) \left( \mathbf{I} - \frac{1}{n} {\bf 1}{\bf 1}^T  \right) \right\Vert_F^2 \\
& \hspace{2cm}  \leq 2 \mathbb{E}\Vert \bX^{I_{(t+1)_0}} - \Bar{\bX}^{I_{(t+1)}}  \Vert_F^2 + 2\mathbb{E} \left\Vert \sum_{t' = I_{(t+1)_0}}^{t} \eta_{t'} ( \beta \bV^{(t)} +\partial F(\bX^{(t')}, \boldsymbol{\xi}^{(t')} )) \left( \mathbf{I} - \frac{1}{n} {\bf 1}{\bf 1}^T  \right) \right\Vert_F^2 
\end{align*}
Using $\verts{AB}_F \leq \verts{A}_F \verts{B}_2$ as in (\ref{bound_frob_mult}) to split the second term above, and then using the bound in (\ref{bound_gap_grad}) and Claim \ref{J-I_eigenvalue}, we get: 
\begin{align} \label{mom_cvx_interim7}
\mathbb{E} \Vert \bX^{(t+1)} -  \Bar{\bX}^{(t+1)} \Vert_F^2 & \leq 2 \mathbb{E}\Vert \bX^{I_{(t+1)_0}} - \Bar{\bX}^{I_{(t+1)_0}}  \Vert_F^2 + 4\eta_{I_{(t+1)_0}}^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)
\end{align}
%For $A_{I_{(t)}}:= \frac{p}{2}\left(  8 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega n c_{I_{(t)}} \right)$, 
The first term in (\ref{mom_cvx_interim7}) can be bounded by Lemma \ref{lem_cvx} below for the synchronization index $I_{(t+1)_0}$ as:
\begin{align}\label{lem_cvx_bound}
\mathbb{E}\Vert \bX^{I_{(t+1)_0}} - \Bar{\bX}^{I_{(t+1)_0}}  \Vert_F^2  \leq \frac{20nA_{I_{(t+1)_0}}}{p^2}\eta_{I_{(t+1)_0}}^2,
\end{align}
where  $A_{I_{(t+1)_0}} = \frac{p}{2}\left(  8 H^2  G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega  c_{I_{(t+1)_0}} \right) $.

\begin{lemma}\label{lem_cvx}
	Let $ \{ \bx_t ^{(i)}  \}_{t=0}^{T-1} $ be generated according to Algorithm \ref{alg_dec_sgd_li} under assumptions of Theorem \ref{thm_cvx_li} with stepsize $\eta_t := \frac{b}{(a+t)}$ (where $a \geq \frac{5H}{p}, \, b > 0$), an increasing threshold fucntion $c_t \sim {o}(t)$ and define $\bar{\bx}_t = \frac{1}{n} \sum_{i=1}^{n} x_t^{(i)} $.
	Consider the set of synchronization indices $\mathcal{I}_T$ =  $\{ I_{(1)},I_{(2)}, \hdots, I_{(t)}, \hdots  \}$. Then for any $I_{(t)} \in \mathcal{I}_T$, we have:
	\begin{align*}
%	\mathbb{E}\sum_{j=1}^n \left\Vert \bar{\bx}^{I_{(t)}} - \bx^{I_{(t)}}_{j} \right\Vert^2 = 
\mathbb{E} \Vert \bX^{I_{(t)}} - \Bar{\bX}^{I_{(t)}} \Vert_F^2  \leq \frac{20nA_{I_{(t)}}  \eta_{I_{(t)}}^2}{p^2},
	\end{align*}
where $p = \frac{\delta \gamma}{8} $, $\delta = 1 - | \lambda_2(\mathbf{W})|$, $\omega$ is compression parameter for operator $\C$, and $A_{I_{(t)}}=\frac{pH}{2}\left(  8 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega Hc_{I_{(t)}} \right) $ where $c_{I_{(t)}}$ and $\eta_{I_{(t)}}$ are respectively the triggering threshold and learning rate at time step $I_{(t)}$.
\end{lemma}

%Substituting above bound in (\ref{suppl_cvx_li_gammat_temp}) and using the fact that $p \leq 1$, for the sequence at time $t$, we have:
%\begin{align*}
%\mathbb{E} \Vert \bX^{(t)} -  \Bar{\bX}^{(t)} \Vert_F^2 \leq  \frac{20\eta_{I_{(t)_0}}^2}{p} \left(  4 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \left( \frac{16}{\omega} + \frac{8}{p} \right) + \frac{2\omega n}{\eta^{(1-\epsilon)}} \right) 
%\end{align*}
%for some constant $\epsilon>0$ and $\alpha > \frac{\beta^2}{1-\beta^2}$. Note that the above bound holds for all values of $t$. Define $\Lambda := \frac{4}{p^2} \left(  4 H^2 n G^2 \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right) \left( \frac{16}{\omega} + \frac{8}{p} \right) + \frac{2\omega n}{\eta^{(1-\epsilon)}} \right) $. Substituting this bound in  \eqref{mom_noncvx_interim2} gives us:
Substituting the above bound from \eqref{lem_cvx_bound} back in (\ref{mom_cvx_interim7}) gives
\begin{align*}
\mathbb{E} \Vert \bX^{(t+1)} -  \Bar{\bX}^{(t+1)} \Vert_F^2 & \leq \frac{40nA_{I_{(t+1)_0}}}{p^2}\eta_{I_{(t+1)_0}}^2 + 4\eta_{I_{(t+1)_0}}^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)
\end{align*}
Using above bound for the second last term in \eqref{mom_cvx_interim6} we have $ \mathbb{E}\verts{\bar{\bX}^{(t)} - \bX^{(t)} }_F^2 = \sum_{i=1}^{n} \mathbb{E}\verts{ \bx^{(t)}_i -  \bar{\bx}^{(t)}}^2 \leq \frac{40nA_{I_{(t)_0}}}{p^2}\eta_{I_{(t)_0}}^2 + 4\eta_{I_{(t)_0}}^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) $ where $I_{(t)_0}$ denotes the last synchronization step before or equal to $t$. This gives us:
\begin{align} 
\mathbb{E}\Vert \tilde{\bx}^{(t+1)} - \bx^* & \Vert^2 \leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} + \frac{9\mu\beta^4\eta_t^3G^2}{2(1-\beta)^7} + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
& + \frac{\eta_t(3L+ 2\mu)}{2(1-\beta)}\frac{1}{n}\left[\frac{40nA_{I_{(t)_0}}}{p^2}\eta_{I_{(t)_0}}^2 {+} 4\eta_{I_{(t)_0}}^2 H^2 n G^2 \left( 1 {+} \frac{9\beta^2}{(1{-} \beta)^4} \right)\right]  - \frac{\eta_t}{(1-\beta)} \left(\bbE f(\blx^{(t)}) - f^*\right)  \label{mom_cvx_interim8}
\end{align}
Observe that $A_{I_{(t)_0}} \leq A_t $, as $I_{(t)_0}$ denotes the last synchronization index before $t$ and $ \{ A_t \}_{t=0}^T $ is an increasing sequence (as  $  \{ c_t \}_{t=0}^T $ is an increasing sequence), and also that $\eta_{I_{(t)_0}} \leq 2 \eta_t $. Using these relations in \eqref{mom_cvx_interim8}, we get
\begin{align} 
\mathbb{E}\Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} + \frac{9\mu\beta^4\eta_t^3G^2}{2(1-\beta)^7} + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
& + \frac{\eta_t(3L+ 2\mu)}{2(1-\beta)}\left[\frac{160A_t}{p^2}\eta_t^2 + 16\eta_t^2 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)\right]  - \frac{\eta_t}{(1-\beta)} \left(\bbE f(\blx^{(t)}) - f^*\right)  \label{mom_cvx_interim_8}
\end{align}
By rearranging terms, we get
\begin{align} 
	\mathbb{E}\Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 - \frac{\eta_t}{(1-\beta)} \left(\bbE f(\blx^{(t)}) - f^*\right) + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
&\hspace{1cm} + \eta_t^3\left[\frac{(3L+ 2\mu)}{2(1-\beta)}16H^2 G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^7}   \right]  \notag \\
&\hspace{2cm} + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} + \eta_t^3\frac{(3L+ 2\mu)}{2(1-\beta)}\frac{160A_t}{p^2} \label{mom_cvx_interim9} 
\end{align}
Substituting the value of $A_t = \frac{pH}{2}\left(  8 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega H c_t \right)$ and noting that $p \leq 1$, we have:
{\allowdisplaybreaks
\begin{align}
 \mathbb{E}\Vert \tilde{\bx}^{(t+1)} - \bx^* \Vert^2 &\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 - \frac{\eta_t}{(1-\beta)} \left(\bbE f(\blx^{(t)}) - f^*\right) + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
& + \eta_t^3\left[\frac{(3L+ 2\mu)}{2(1-\beta)}16H^2 G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^7}   \right]   + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} \notag \\
& \quad +  \eta_t^3\frac{(3L+ 2\mu)}{2(1-\beta)}\frac{160}{p^2}\frac{pH}{2}\left(  8 H^2 G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) \left( \frac{16}{\omega} + \frac{4}{p} \right) + 2\omega Hc_t \right) \notag \\
&= \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 - \frac{\eta_t}{(1-\beta)} \left(\bbE f(\blx^{(t)}) - f^*\right) + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
&+ \eta_t^3\left[\frac{(3L+ 2\mu)}{(1-\beta)}\frac{320H^3 G^2}{p} \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)\left(\frac{p}{40H} + \frac{16}{\omega} + \frac{4}{p} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^7}   \right]  \notag \\
& \qquad + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} +  \eta_t^3\frac{(3L+ 2\mu)}{(1-\beta)}\frac{80H\omega c_t}{p} \notag \\
&\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 - \frac{\eta_t}{(1-\beta)} \left(\bbE f(\blx^{(t)}) - f^*\right) + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
&\hspace{1cm} + \eta_t^3\left[\frac{(3L+ 2\mu)}{(1-\beta)}\frac{320H^3 G^2}{p} \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)\left(\frac{16}{\omega} + \frac{5}{p} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^7}   \right]  \notag \\
&\hspace{2cm} + \frac{36\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^6} +  \eta_t^3\frac{(3L+ 2\mu)}{(1-\beta)}\frac{80H\omega c_t}{p}\label{mom_cvx_interim9}
% &\leq \left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} - \bx^*\|^2 - \eta_t \left(\bbE f(\blx^{(t)}) - f^*\right) + \frac{4\eta_{t}^{\nicefrac{5}{2}}\beta^2G^2}{(1-\beta)^4} \\ 
%& \qquad + \eta_t^3 \left(\frac{\mu\beta^4G^2}{2(1-\beta)^5} +     \frac{640 \psi H^2G^2}{p} \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)  \left( \frac{16}{\omega} + \frac{8}{p}   \right)    \right)  + 
%\frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} \notag \\ 
%&\hspace{1cm} + \frac{160 \psi \omega c_t \eta_t^3 }{p}  \notag 
\end{align}
}
 We now use Lemma \ref{mom_cvx_suppl_lemm_stich} for the sequence above by defining:
 \begin{align*}
 	h_t & := \mathbb{E}\verts{\btx^{(t)}  - \bx^*}^2 \\
 	e_t & := \mathbb{E}f(\blx^{(t)}) - f^* \\
 	P &:= \frac{1}{(1-\beta)} \\
 	Q &:= \frac{\bar{\sigma}^2}{(1-\beta)^2n} \\
 	V&:=  \frac{36 \beta^2G^2}{(1-\beta)^6} \\
 	R&:= \frac{(3L+ 2\mu)}{(1-\beta)}\frac{320H^3 G^2}{p} \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)\left(\frac{16}{\omega} + \frac{5}{p} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^7} \\
 	U_t&:= Uc_t, \text{ where } U=\frac{(3L+ 2\mu)}{(1-\beta)}\frac{80H\omega}{p}
 \end{align*}
Let $c_t \leq c_0 t^{(1-\epsilon)}$, where $c_0 \geq 0$ is a constant and $\epsilon \in (0,1]$.
Note that $\btx^{(0)}=\blx^{(0)}$, so $h_0 = \bbE\verts{{\blx}^{(0)} - \bx^*}^2$.
For $w_t = (a+t)^2$, Lemma \ref{mom_cvx_suppl_lemm_stich} gives the following relation:
\begin{align*}
\frac{1}{S_T}\sum_{t=0}^{T-1} w_t e_t  &\leq  \frac{\mu a^3h_0}{16S_T}  + \frac{8(1-\beta)^2Q}{\mu}\frac{T(T+2a)}{S_T} + \frac{64(1-\beta)^{\nicefrac{5}{2}}}{\mu^{\nicefrac{3}{2}}}\frac{2V (T+a)^{\nicefrac{3}{2}} }{3S_T} \notag \\
&\hspace{2cm} + \frac{256(1-\beta)^3}{\mu^2}\frac{RT}{S_T} + \frac{256(1-\beta)^3}{\mu^2} \frac{U c_0}{(2-\epsilon)} \frac{T^{(2-\epsilon)}}{S_T}.
\end{align*}
% \begin{align*}
% \frac{1}{S_T} \sum_{t=0}^{T-1}w_t e_t & \leq \frac{\mu a^3}{8S_T}h_0^2 + \frac{4T(T+2a)}{\mu S_T} \frac{\bar{\sigma}^2}{(1-\beta)^2n} + \frac{128\sqrt{2} \beta^2 G^2 (T+a)^{\nicefrac{3}{2}} }{3 \mu^{\nicefrac{3}{2}}  S_T (1-\beta)^4 } \\
% & + \frac{64T}{\mu^2 S_T}\left(\frac{\mu\beta^4G^2}{2(1-\beta)^5} +     \frac{640 \psi H^2G^2}{p} \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)  \left( \frac{16}{\omega} + \frac{8}{p}   \right)    \right) \\
% & \qquad + \frac{64c_0T^{(2-\epsilon)}}{\mu^2 (2-\epsilon) S_T } \left( \frac{160 \psi \omega c_t }{p}\right)
% \end{align*}
Define $\bx^{(T)}_{avg} := \frac{1}{S_T} \sum_{t=0}^{T-1}w_t \bar{\bx}^{(t)}$.
From the convexity of $f$, we finally have:
 \begin{align*}
 \mathbb{E}f(\bx_{avg}^{(T)}) - f^* & \leq \frac{\mu a^3}{16S_T}\bbE\verts{{\blx}^{(0)} - \bx^*}^2 + \frac{8\bar{\sigma}^2}{\mu}\frac{T(T+2a)}{nS_T} + \frac{64}{(\mu^{\nicefrac{3}{2}} (1-\beta)^{\nicefrac{7}{2}})}\frac{72\beta^2G^2 (T+a)^{\nicefrac{3}{2}} }{3S_T} \notag \\
&\hspace{0.25cm} + \frac{256(1-\beta)^3}{\mu^2}\left[\frac{(3L+ 2\mu)}{(1-\beta)}\frac{320H^3 G^2}{p} \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)\left(\frac{16}{\omega} + \frac{5}{p} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^7}\right]\frac{T}{S_T} \\
&\hspace{0.5cm} + \frac{256(1-\beta)^2}{\mu^2} \frac{(3L+2\mu)80H\omega c_0}{p(2-\epsilon)} \frac{T^{(2-\epsilon)}}{S_T}.
%&= \frac{\mu a^3}{8S_T}a_0^2 + \frac{4T(T+2a)}{\mu S_T} \frac{\bar{\sigma}^2}{(1-\beta)^2n} + \frac{128\sqrt{2} \beta^2 G^2 (T+a)^{\nicefrac{3}{2}} }{3 \mu^{\nicefrac{3}{2}}  S_T (1-\beta)^4 } \\
% & + \frac{64T}{\mu^2 S_T}\left(\frac{\mu\beta^4G^2}{2(1-\beta)^5} +     \frac{640 \psi H^2G^2}{p} \left( 1 + \frac{(1+\alpha)}{1- (1+\alpha^{-1})\beta^2} \right)  \left( \frac{16}{\omega} + \frac{8}{p}   \right)    \right) \\
% & \qquad + \frac{64c_0T^{(2-\epsilon)}}{\mu^2 (2-\epsilon) S_T } \left( \frac{160 \psi \omega c_t }{p}\right)
 \end{align*}
% We finally use the fact that $p \leq \omega$ (as $\delta \leq 1$ and $p:= \frac{\gamma^* \delta}{8}$ with $\gamma^* \leq \omega $). This simplies the above expression as:
% \begin{align*}
% \mathbb{E}f(\bx_{avg}^{(T)}) - f^* & \leq \frac{\mu a^3}{8S_T}a_0^2 + \frac{4T(T+2a)}{\mu S_T}\frac{ \Bar{\sigma}^2}{n} + \frac{512T}{\mu^2 S_T} \left(  2L + \mu  \right) \left( \frac{160}{p^2}\right)G^2H^2 \\
% & \qquad +\frac{6400 c_0 \omega T ^{(2-\epsilon)}}{\mu^2 (2-\epsilon)S_T} \left(  \frac{2L + \mu}{p}  \right)
% \end{align*}
Using the inequality $ \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) \leq \frac{18}{(1-\beta)^4}$ and $(1-\beta) \leq 1$, we have:
 \begin{align*}
\mathbb{E}f(\bx_{avg}^{(T)}) - f^* & \leq \frac{\mu a^3}{16S_T}\bbE\verts{{\blx}^{(0)} - \bx^*}^2 + \frac{8\bar{\sigma}^2T(T+2a)}{\mu nS_T} + \frac{512\beta^23G^2 (T+a)^{\nicefrac{3}{2}}}{\mu^{\nicefrac{3}{2}} (1-\beta)^{\nicefrac{7}{2}} S_T } \notag \\
&\hspace{0.25cm} + \frac{256}{\mu^2}\left[\frac{(3L+ 2\mu)640H^3 G^29}{p(1-\beta)^2}\left(\frac{16}{\omega} + \frac{5}{p} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^4}\right]\frac{T}{S_T} \\
&\hspace{0.5cm} + \frac{256(3L+2\mu)80H\omega c_0}{\mu^2 p(2-\epsilon)} \frac{T^{(2-\epsilon)}}{S_T}.
\end{align*}

 We finally use the fact that $p \leq \omega$ (as $\delta \leq 1$ and $p:= \frac{\gamma^* \delta}{8}$ with $\gamma^* \leq \omega $). This completes proof of strongly convex part of Theorem \ref{thm_cvx_li}. We can further use the fact that $p \geq \frac{\delta^2 \omega}{644}$ and $\mathbb{E} \verts{\bar{\bx}^{(0)} - \bx^*}_2^2 \leq \frac{4G^2}{\mu^2}$ (from Lemma 2 in \cite{rakhlin2011making}) to get the expression given in the main paper.
 \end{proof}
 %------------Lemma-------
 \begin{lemma} \label{mom_cvx_suppl_lemm_stich}
 	Let $\{ h_t \}_{t \geq 0}, h_t \geq 0, \{e_t \}_{t \geq 0}, e_t \geq 0 $ be sequences satisfying :
\begin{align} \label{recursion}
h_{t+1} \leq \left(1- \frac{\mu \eta_t}{4(1-\beta)} \right) h_{t} - \eta_t e_t P + \eta_t^2Q + \eta_t^{\nicefrac{5}{2}}V  + \eta_t^3R + \eta_t^3U_t ,
\end{align}
where $\eta_t = \frac{16(1-\beta)}{\mu (a+t)} $ and $P,Q,R,V \geq 0$, $\mu>0, a>1$ are constants.
Let $U_t = U c_t$, where $U \geq 0$ is a constant and $c_t = o(t)$. 
In particular, if $c_t \leq c_0 t^{(1-\epsilon)}$ for some $c_0 \geq 0$ and $\epsilon \in (0,1]$, then it holds that
%\begin{align*}
%\frac{P}{S_T} \sum_{t=0}^{T-1}w_t e_t \leq \frac{\mu a^3}{8S_T}h_0 + \frac{4T(T+2a)}{\mu S_T}Q + \frac{32\sqrt{2} (T+a)^{\nicefrac{3}{2}} }{3 \mu^{\nicefrac{3}{2}}  S_T }V+ \frac{64T}{\mu^2 S_T}R + \frac{64c_0T^{(2-\epsilon)}}{\mu^2 (2-\epsilon) S_T }U ,
%\end{align*}
\begin{align*}
\frac{P}{S_T}\sum_{t=0}^{T-1} w_t e_t  &\leq  \frac{\mu a^3}{16(1-\beta)}\frac{h_{0}}{S_T} + \frac{8(1-\beta)Q}{\mu}\frac{T(T+2a)}{S_T} + \left(\frac{16(1-\beta)}{\mu}\right)^{\nicefrac{3}{2}}\frac{2V (T+a)^{\nicefrac{3}{2}} }{3S_T} \notag \\
&\hspace{2cm} + \left(\frac{16(1-\beta)}{\mu}\right)^2\frac{RT}{S_T} + \left(\frac{16(1-\beta)}{\mu}\right)^2 \frac{U c_0}{(2-\epsilon)} \frac{T^{(2-\epsilon)}}{S_T},
\end{align*}
where $w_t = (a+t)^2$ and $S_T := \sum_{t=0}^{T-1}w_t = \frac{T}{6} (2T^2+6aT-3T+6a^2-6a+1) \geq \frac{1}{3}T^3$.
For an arbitrary $c_t$ such that $c_t=o(t)$, the last term in the above bound would be $\left(\frac{16(1-\beta)}{\mu}\right)^2 U c_0 \frac{o(T^2)}{S_T}$.
\end{lemma}
\begin{proof}
We adapt the proof of [Lemma 3.3] \cite{stich_sparsified_2018} to prove Lemma \ref{mom_cvx_suppl_lemm_stich}, with appropriate modifications arising because we have a different recursion in \eqref{recursion} than the recursion in [Lemma 3.3] \cite{stich_sparsified_2018}.

First multiply both sides of \eqref{recursion} by $\frac{w_t}{\eta_t}$ which gives:
\begin{align}\label{recursion_interim1}
h_{t+1} \frac{w_t}{\eta_t} \leq \left(1- \frac{\mu\eta_t}{4(1-\beta)} \right) \frac{w_t}{\eta_t} h_{t} - w_t e_t P + w_t \eta_tQ + w_t \eta_t^{\nicefrac{3}{2}}  V  + w_t \eta_t^2R  + w_t \eta_t^2U_t. 
\end{align}
Now we show that $\left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\frac{w_t}{\eta_t} \leq \frac{w_{t-1}}{\eta_{t-1}}$:
\begin{align}
\left(1-\frac{\mu\eta_t}{4(1-\beta)}\right)\frac{w_t}{\eta_t} &= \left(\frac{a+t-4}{a+t}\right)\frac{\mu(a+t)^3}{16(1-\beta)} \notag \\
&= \frac{\mu(a+t-4)(a+t)^2}{16(1-\beta)} \notag \\
&\stackrel{\text{(a)}}{\leq} \frac{\mu(a+t-1)^3}{16(1-\beta)} \notag \\
&= \frac{w_{t-1}}{\eta_{t-1}}, \label{recursion_interim2}
\end{align}
where (a) follows from
\[(a+t-4)(a+t)^2 = (a+t-1)^3 + \underbrace{(1-3a-a^2-3t-2at-t^2)}_{\leq \ 0} \leq (a+t-1)^2.\]
Summing both sides of \eqref{recursion_interim1} from $t=0$ to $t=T-1$ and using \eqref{recursion_interim2} yields
\begin{align}\label{recursion_interim3}
h_{T} \frac{w_{T-1}}{\eta_{T-1}} \leq \left(1- \frac{\mu \eta_0}{4(1-\beta)} \right) \frac{w_0}{\eta_0} h_{0} -  \sum_{t=0}^{T-1} w_t e_t P + \sum_{t=0}^{T-1} w_t \eta_tQ+ \sum_{t=0}^{T-1} w_t \eta_t^{\nicefrac{3}{2}} V + \sum_{t=0}^{T-1} w_t \eta_t^2R  + \sum_{t=0}^{T-1} w_t \eta_t^2U_t. 
\end{align}
By ignoring $h_{T} \frac{w_{T-1}}{\eta_{T-1}} \geq 0$ and $\frac{\mu \eta_0}{4(1-\beta)}\frac{w_0}{\eta_0} h_{0} \geq 0$, and substituting $\frac{w_0}{\eta_0} = \frac{\mu a^3}{16(1-\beta)}$, we get:
\begin{align}\label{recursion_interim4}
P\sum_{t=0}^{T-1} w_t e_t  \leq \frac{\mu a^3}{16(1-\beta)} h_{0} + \sum_{t=0}^{T-1} w_t \eta_tQ+ \sum_{t=0}^{T-1} w_t \eta_t^{\nicefrac{3}{2}} V + \sum_{t=0}^{T-1} w_t \eta_t^2R  + \sum_{t=0}^{T-1} w_t \eta_t^2U_t. 
\end{align} 
%Rearranging the terms in above and noting that $\frac{w_0}{\eta_0} = \frac{\mu a^3}{8} $, we get:
% 	\begin{align} \label{cvx_stich_lemma_interim1}
% 	P \sum_{t=0}^{T-1} w_t e_t  \leq  \frac{\mu a^3}{8} + \sum_{t=0}^{T-1} w_t \eta_tQ + \sum_{t=0}^{T-1} w_t \eta_t^{\nicefrac{3}{2}} V +  \sum_{t=0}^{T-1} w_t \eta_t^2R + \sum_{t=0}^{T-1} w_t \eta_t^2U_t 
% 	\end{align}
We now bound the terms in the RHS of \eqref{recursion_interim4}. The bounds for the second and third term are given in [Lemma 3.3] \cite{stich_sparsified_2018}, which are:
\begin{align*}
 	\sum_{t=0}^{T-1} w_t \eta_tQ  & \leq \frac{8(1-\beta)Q}{\mu}T(T+2a) \\
 	\sum_{t=0}^{T-1} w_t \eta_t^{\nicefrac{3}{2}} V  & \leq \left(\frac{16(1-\beta)}{\mu}\right)^{\nicefrac{3}{2}}V \int_{0}^{T} \sqrt{t+a}\cdot dt \leq \left(\frac{16(1-\beta)}{\mu}\right)^{\nicefrac{3}{2}}\frac{2V (T+a)^{\nicefrac{3}{2}} }{3} \\
	\sum_{t=0}^{T-1} w_t \eta_t^2R & \leq \left(\frac{16(1-\beta)}{\mu}\right)^2RT
\end{align*}
To bound the last term in RHS of \eqref{recursion_interim4}, we note that $U_t = U c_t$ where $c_t = o(t)$ and $U \geq 0$ is a constant. 
For simplicity, we assume that $c_t \leq c_0 t^{1-\epsilon}$ for some $\epsilon \in (0,1]$, and proceed to bound the terms as:
\begin{align*}
\sum_{t=0}^{T-1} w_t \eta_t^2U_t &\leq U c_0\sum_{t=0}^{T-1} w_t \eta_t^2t^{(1-\epsilon)}
\\
&= \left(\frac{16(1-\beta)}{\mu}\right)^2 U c_0 \sum_{t=0}^{T-1}  t^{(1-\epsilon)} \\
&\leq \left(\frac{16(1-\beta)}{\mu}\right)^2 U c_0 \int_{0}^{T} t^{(1-\epsilon)} dt \\
&= \left(\frac{16(1-\beta)}{\mu}\right)^2 \frac{U c_0}{(2-\epsilon)} T^{(2-\epsilon)}
\end{align*}
Note that for $c_t = o(t)$, instead of $T^{(2-\epsilon)}$ we would have got $o(T^2)$ in the above bound. Substituting these bounds in \eqref{recursion_interim4} yields:
\begin{align*}
P \sum_{t=0}^{T-1} w_t e_t  &\leq  \frac{\mu a^3}{16(1-\beta)} h_{0} + \frac{8(1-\beta)Q}{\mu}T(T+2a) + \left(\frac{16(1-\beta)}{\mu}\right)^{\nicefrac{3}{2}}\frac{2V (T+a)^{\nicefrac{3}{2}} }{3} \notag \\
&\hspace{2cm} + \left(\frac{16(1-\beta)}{\mu}\right)^2RT + \left(\frac{16(1-\beta)}{\mu}\right)^2 \frac{U c_0}{(2-\epsilon)} T^{(2-\epsilon)}  
\end{align*}
Dividing both sides by $S_T := \sum_{t=0}^{T-1}w_t = \frac{T}{6} (2T^2+6aT-3T+6a^2-6a+1) \geq \frac{1}{3}T^3$, we get
\begin{align*}
\frac{P}{S_T}\sum_{t=0}^{T-1} w_t e_t  &\leq  \frac{\mu a^3}{16(1-\beta)}\frac{h_{0}}{S_T} + \frac{8(1-\beta)Q}{\mu}\frac{T(T+2a)}{S_T} + \left(\frac{16(1-\beta)}{\mu}\right)^{\nicefrac{3}{2}}\frac{2V (T+a)^{\nicefrac{3}{2}} }{3S_T} \notag \\
&\hspace{2cm} + \left(\frac{16(1-\beta)}{\mu}\right)^2\frac{RT}{S_T} + \left(\frac{16(1-\beta)}{\mu}\right)^2 \frac{U c_0}{(2-\epsilon)} \frac{T^{(2-\epsilon)}}{S_T}.
\end{align*}
This completes the proof of Lemma \ref{mom_cvx_suppl_lemm_stich}.
\end{proof}
}
 %--------------------------------------------------------------------

==> proof_outlines.tex <==
\allowdisplaybreaks{
	
Due to lack of space, below we only provide a proof-sketch of Theorem \ref{convergence_results}. We defer the interested reader to the complete proof in our full paper \cite{singh2020squarm}, where we also discuss technical challenges involved and a comparison to related works.	
	
	
%Before providing an outline for proof of our results, first we describe the technical challenges we faced.
%
%\noindent \textbf{Technical Challenges:}  Our convergence proofs require the use of virtual sequences as defined in \eqref{virt_seq_main} below.
%Proving convergence results using virtual sequences has been promising lately in stochastic optimization; see, for example, \cite{stich_sparsified_2018,alistarh_convergence_2018,stich-signsgd-19,basu_qsparse-local-sgd:_2019,Momentum_linear-speedup19,distributed_momentum19}. The most related works to ours are \cite{Momentum_linear-speedup19,distributed_momentum19}, 
%where \cite{Momentum_linear-speedup19} studies local SGD with momentum in a decentralized setup, but {\em without} any compressed or event-triggered communication, and \cite{distributed_momentum19} studies compressed {\em distributed} SGD with momentum for non-convex objectives, but without local iterations or event-triggered communication. %, and they also assume that all nodes have access to the same dataset.
%We would like to emphasize that even without momentum and local iterations, analyzing compression in decentralized optimization \cite{koloskova_decentralized_2019-1,koloskova_decentralized_2019} (whose analysis does not require virtual sequences) is significantly more involved and requires different technical tools than analyzing compression in distributed optimization \cite{alistarh_convergence_2018,stich-signsgd-19}. One of the main reasons for this is as follows: In a decentralized setup, we need to separately show that nodes eventually reach to the same parameters (i.e., consensus happens), which happens trivially in a distributed setup, because in each iteration all worker nodes have the same parameters sent by the master node. 
%On top of that, incorporating momentum updates (which has only been analyzed in distributed setups so far) in decentralized setting is non-trivial and gives similar challenges. We go even beyond that to save more on communication than just compression -- we also use local iterations and event-triggered communication in our algorithm. Note that the main challenge in handling local iterations is that performing local SGD steps causes drift in the local parameter vectors at different nodes, and bounding that drift even in a distributed setup (even without momentum and compression) is non-trivial; see, for example, \cite{MadhaviLocalSGD19,MadhaviLocalFL19,scaffold19,TighterTheoryLocalGD20,FedAvgNonIID20,TalwalkarFL20,alibaba_local}. In our event-triggered communication, nodes exchange their updates only when their local parameter vectors have changed significantly from the last time communication occurred. This inherently causes asynchrony, as after preforming $H$ local iterations, because of the drift in local parameters, not all nodes communicate at the same time, and handling this is another challenge.
%
%As a consequence, our proofs are fundamentally different and significantly more challenging from existing works, including \cite{distributed_momentum19, Momentum_linear-speedup19,koloskova_decentralized_2019-1,koloskova_decentralized_2019}, as we study decentralized setup with compressed exchanges, and in addition to incorporating momentum, our algorithm also employs local iterations and event-triggered communication with both sparisified and quantized compression to save on communication bits. 
%As opposed to \cite{distributed_momentum19}, we allow {\em heterogeneous} data setting, where different nodes may have different datasets. Moreover, with all these, we achieve vanilla SGD like convergence rates.
%
%Due to lack of space, below we only provide a proof-sketch of Theorem \ref{convergence_results} and defer the interest reader to the complete proof in our full paper \cite{singh2020squarm}.

%%--------------------------------------------------------------- 
%\textbf{Proof outline of Theorem \ref{convergence_results} (strongly-convex).} %\label{convex-convergence}
%Define virtual sequences ${\btx}_i^{(t)}$ for all $i\in[n]$ as:
%\begin{align} \label{virt_seq_main}
%{\btx}_i^{(t)} = {\bx}_i^{(t)} - \frac{\eta_{t-1} \beta^2}{(1-\beta)} \bv_i^{(t-1)}.
%\end{align}
%
%Consider the collection of iterates $\{\bx_i ^{(t)}\}_{t=0}^{T-1}$, $i \in [n]$ generated by Algorithm~\ref{alg_dec_sgd_li} at time $t$. 
%%For any time $t\geq0$, we have from line 15 of Algorithm~\ref{alg_dec_sgd_li} that:
%%\begin{align*}
%%\bx_i^{(t+1)} = \bx_i^{(t+\frac{1}{2})} + \mathbbm{1}_{(t+1) \in \mathcal{I}_T}\gamma \sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t+1)} - \hat{\bx}_i^{(t+1)}),
%%\end{align*}
%%where $\bx_i^{(t+\frac{1}{2})} = \bx_i ^{(t)} - \eta_t \nabla F_i(\bx_i^{(t)}, \xi_i^{(t)})$ (line 4).
%Let ${\blx}^{(t)} = \frac{1}{n} \sum_{i=1}^{n} \bx_{i}^{(t)}$.
%We first argue that ${\blx}^{(t+1)}={\blx}^{(t+\frac{1}{2})}$.
%This trivially holds when $(t+1)\notin \I_T$ (line 18). For the other case, i.e., $(t+1)\in \I_T$ (line 16), this follows because
%$\sum_{i=1}^n\sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t+1)} - \hat{\bx}_i^{(t+1)})=0$, as $W$ is doubly stochastic. 
%Thus, using the definition of $\bx_i^{(t+\frac{1}{2})}$ from line 5, we get
%\begin{equation}\label{eq:proof_out_interim0}
%{\blx}^{(t+1)} = \textstyle {\blx}^{(t)} - \frac{\eta_t}{n}\sum_{j=1}^n ( \beta \bv_j^{(t)} + \nabla F_j(\bx_j^{(t)},\xi_j^{(t)})).
%\end{equation}
%%We define a virtual sequence at each node $i \in [n]$ as: ${\btx}_i^{(t)} = {\bx}_i^{(t)} - \frac{\eta_t \beta^2}{(1-\beta)} \bv_i^{(t-1)}$. 
%%where we have used definition of $\bx_i^{(t+\frac{1}{2})}$ from line 5. 
%Define $\btx^{(t)} = \frac{1}{n}\sum_1^n \btx_i^{(t)}$. Taking an average of \eqref{virt_seq_main} gives
%%\begin{equation} \label{eq:proof_out_interim1}
%${\btx}^{(t)} = {\blx}^{(t)} - \frac{\eta_t \beta^2}{(1-\beta)} \frac{1}{n} \sum_{i=1}^n \bv_i^{(t-1)}$.
%%\end{equation}
%Together with \eqref{eq:proof_out_interim0}, we can show the following recurrence relation on $\btx^{(t)}$: % (the details are given in the appendix (in supplementary material)): %Appendix~\ref{proof_thm_cvx_li}):
%\begin{align}\label{eq:recurrence_virt-seq}
%{\btx}^{(t+1)} = \textstyle {\btx}^{(t)} - \frac{\eta_t}{(1-\beta)}\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}).
%\end{align}
%%Substituting value of ${\blx}^{(t)}$ from \eqref{eq:proof_out_interim0} in \eqref{eq:proof_out_interim1} and subtracting  $\bx^*$ (the minimizer of \eqref{eq:obj-fn}) from both sides gives
%%\begin{align*}
%%	{\btx}^{(t+1)} - \bx^* = {\btx}^{(t)} - \frac{\eta_t}{(1-\beta)}\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) -\bx^*
%%\end{align*}
%%Using  $\eta_t \leq \min \left\{ \frac{(1-\beta)}{8L} , \frac{(1-\beta)^2}{(16L\beta^2)^2}   \right\}$ (which follows from choice of $\eta_t$ stated in statement of Theorem \ref{thm_cvx_li}),  
%After a lot of algebraic manipulations provided in the supplementary material, where, other than using some properties of smoothness and strong-convexity (see footnote \ref{l-smooth-footnote},\ref{str-cvx-footnote}), we used an important trick on inner-products, which was crucial to getting the speed-up with the number of workers in our final convergence rate, we arrive at the following sequence relation for $\{\btx^{(t)}\}$:
%\begin{align}\label{eq:thm_cvx_interim3}
% \textstyle \mathbb{E}\Vert & {\btx}^{(t+1)}  {-} \bx^* \Vert^2 \leq  \left(1{-}\frac{\mu\eta_t}{4(1-\beta)}\right)\bbE\|\btx^{(t)} {-} \bx^*\|^2 \notag \\
% &  + \frac{\eta_t^2\bar{\sigma}^2}{(1-\beta)^2n} + \textstyle \frac{\eta_t(3L{+} 2\mu)}{2(1-\beta)}\frac{1}{n}\sum_{j=1}^n \bbE\Vert \bx_j^{(t)}  {-} {\blx}^{(t)} \Vert^2 \notag \\
%& - \frac{\eta_t(\bbE f(\blx^{(t)}) - f^*)}{(1-\beta)} \textstyle +\frac{4\eta_{t}^{\nicefrac{5}{2}}\beta^2}{(1-\beta)^2} \bbE\left\|\frac{1}{n} \sum_{i=1}^{n} \bv_i^{(t-1)}\right\|^2 \notag \\
% & + \frac{\mu\eta_t}{2(1-\beta)}\bbE \Vert \btx^{(t)} - \blx^{(t)}  \Vert^2
%\end{align}
%where expectation is w.r.t.~the entire process. 
%Let $I_{(t_0)} \in \mathcal{I}_T$ denote the last synchronization index before time $t$.
%The assumption that $gap(\I_T)\leq H$, implies $t-I_{(t_0)}\leq H$.  
%Using this and the bounded gradient assumption, we bound the term $\bbE\Vert \bx_j^{(t)}  - {\blx}^{(t)} \Vert^2$ as:
%\begin{align}\label{eq:thm_cvx_interim4}
% \textstyle \sum_{j=1}^n \mathbb{E} \Vert  {\blx}^{{(t)}} & -  \bx^{{(t)}}_{j} \Vert^2  \leq 2\mathbb{E} \textstyle\sum_{j=1}^n \Vert {\blx}^{I_{(t_0)}} - \bx^{I_{(t_0)}}_{j} \Vert^2 \notag \\
% & + 4\eta_{I_{(t+1)_0}}^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) 
%\end{align}
%We now note the following lemma (proved in the supplementary material) %Appendix \ref{proof_thm_cvx_li},\ref{proof_lem_dec_li_sgd}) 
%to bound the terms on RHS of \eqref{eq:thm_cvx_interim3} and \eqref{eq:thm_cvx_interim4}:
%\begin{lemma}\label{lem_dec_li_sgd}
%	 Consider assumptions of Theorem~\ref{convergence_results}, for $I_{(t)} \in \mathcal{I}_{T}$ and $c_{I_{(t)}}$ as threshold function evaluated at $I_{(t)}$. Define $A_{I_{(t)}}={pH}\left(  4 H^2 G^2 \left( 1 {+} \frac{9\beta^2}{(1{-}\beta)^4} \right) \left( \frac{16}{\omega} {+} \frac{4}{p} \right) {+} \omega Hc_{I_{(t)}} \right)$, then:
%	\begin{align*}
%	\mathbb{E}  \verts{\frac{1}{n} \textstyle \sum_{i=1}^{n} \bv^{(t-1)}_i} ^2 & \leq \frac{9G^2}{(1-\beta)^4}\\ %\hspace{0.1cm}
%	\mathbb{E}\Vert \blx^{(t)} -  \btx^{(t)} \Vert^2 & \leq \frac{9\beta^4 \eta_t^2 G^2}{(1-\beta)^6}\\ % \hspace{0.1cm}
%	\textstyle \sum_{j=1}^n \mathbb{E} \textstyle \left\Vert {\blx}^{I_{(t)}} - \bx^{I_{(t)}}_{j} \right\Vert^2 & \leq \frac{20nA_{I_{(t)}}\eta_{I_{(t)}}^2}{p^2}.
%	\end{align*}
%\end{lemma}
%The second and third bound in Lemma \ref{lem_dec_li_sgd} mean that the local sequences and the virtual sequence asymptotically approach the average sequence, respectively. We then substitute the bounds from \eqref{eq:thm_cvx_interim4}, Lemma \ref{lem_dec_li_sgd}  and the value of $A_t$ in \eqref{eq:thm_cvx_interim3} and also use $\eta_{I_{t_0}}\leq 2\eta_t$ (from assumption $a\geq H$).
%Then defining 
%$h_t = \mathbb{E} \Vert {\btx}^{(t)} - \bx^* \Vert^2 $, $ P= \frac{1}{(1-\beta)} $, $Q= \frac{ \Bar{\sigma}^2}{(1-\beta)^2 n} $, $R =   \frac{(3L+ 2\mu)}{(1-\beta)}\frac{320H^3 G^2}{p} \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right)\left(\frac{16}{\omega} + \frac{5}{p} \right) + \frac{9\mu\beta^4G^2}{2(1-\beta)^7}$, $V= \frac{36 \beta^2 G^2}{(1-\beta)^6} $, $U = \frac{(3L+2\mu)80H\omega}{(1-\beta)p}\omega $ and $U_t =U c_t $ in the resulting expression, we get:
%\begin{align*}
%	h_{t+1} \leq (1- \nicefrac{\mu \eta_t}{2} )h_{t} - \eta_t (\bbE f(\blx^{(t)}) - f^*) P \\
%	+ \eta_t^2Q + \eta_t^{\nicefrac{5}{2}}V+\eta_t^3R + \eta_t^3U_t,
%\end{align*}
%which is a contracting recurrence for $h_t$.
%Solving this and doing some algebraic manipulations provided in the supplementary material establishes the strongly-convex part of Theorem~\ref{convergence_results}.


\paragraph{Proof outline of Theorem \ref{convergence_results}.}
Define virtual sequences ${\btx}_i^{(t)}$ for all $i\in[n]$ as:
\begin{align} \label{virt_seq_main}
	{\btx}_i^{(t)} = {\bx}_i^{(t)} - \frac{\eta \beta^2}{(1-\beta)} \bv_i^{(t-1)}.
\end{align}

Consider the collection of iterates $\{\bx_i ^{(t)}\}_{t=0}^{T-1}$, $i \in [n]$ generated by Algorithm~\ref{alg_dec_sgd_li} at time $t$. 
%For any time $t\geq0$, we have from line 15 of Algorithm~\ref{alg_dec_sgd_li} that:
%\begin{align*}
%\bx_i^{(t+1)} = \bx_i^{(t+\frac{1}{2})} + \mathbbm{1}_{(t+1) \in \mathcal{I}_T}\gamma \sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t+1)} - \hat{\bx}_i^{(t+1)}),
%\end{align*}
%where $\bx_i^{(t+\frac{1}{2})} = \bx_i ^{(t)} - \eta_t \nabla F_i(\bx_i^{(t)}, \xi_i^{(t)})$ (line 4).
Let ${\blx}^{(t)} = \frac{1}{n} \sum_{i=1}^{n} \bx_{i}^{(t)}$.
We first argue that ${\blx}^{(t+1)}={\blx}^{(t+\frac{1}{2})}$.
This trivially holds when $(t+1)\notin \I_T$ (line 18). For the other case, i.e., $(t+1)\in \I_T$ (line 18), this follows because
$\sum_{i=1}^n\sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t+1)} - \hat{\bx}_i^{(t+1)})=0$, as $W$ is doubly stochastic. 
Thus, using the definition of $\bx_i^{(t+\frac{1}{2})}$ from line 5, we get
\begin{equation}\label{eq:proof_out_interim0}
	{\blx}^{(t+1)} =  {\blx}^{(t)} - \frac{\eta}{n}\sum_{j=1}^n ( \beta \bv_j^{(t)} + \nabla F_j(\bx_j^{(t)},\xi_j^{(t)})).
\end{equation}
%We define a virtual sequence at each node $i \in [n]$ as: ${\btx}_i^{(t)} = {\bx}_i^{(t)} - \frac{\eta_t \beta^2}{(1-\beta)} \bv_i^{(t-1)}$. 
%where we have used definition of $\bx_i^{(t+\frac{1}{2})}$ from line 5. 
Define $\btx^{(t)} = \frac{1}{n}\sum_1^n \btx_i^{(t)}$. Taking an average of \eqref{virt_seq_main} gives
%\begin{equation} \label{eq:proof_out_interim1}
${\btx}^{(t)} = {\blx}^{(t)} - \frac{\eta \beta^2}{(1-\beta)} \frac{1}{n} \sum_{i=1}^n \bv_i^{(t-1)}$.
%\end{equation}
Together with \eqref{eq:proof_out_interim0}, we can show the following recurrence relation on $\btx^{(t)}$: % (the details are given in the appendix (in supplementary material)): %Appendix~\ref{proof_thm_cvx_li}):
\begin{align}\label{eq:recurrence_virt-seq}
	{\btx}^{(t+1)} =  {\btx}^{(t)} - \frac{\eta}{(1-\beta)}\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}).
\end{align}
Evaluating the objective function $f$ at ${\btx}^{(t+1)}$ and using \eqref{eq:recurrence_virt-seq} along with some algebraic manipulations, we get: 
\begin{align} \label{eq:proof_out_interim5}
\textstyle	Z_1  \Vert \frac{1}{n} & \sum_{i=1}^{n} \nabla f_i(\bx^{(t)}_i) \Vert^2  \leq  f({\btx}^{(t)})  {-} f({\btx}^{(t+1)})\notag \\
 & + \frac{L\eta^2 \bar{\sigma}^2}{2n(1-\beta)^2}+ \frac{L^2 \eta}{ (1-\beta) n} \left(R_1(t) + R_2(t)\right)
%	& + \frac{L^2 \eta^3 \beta^4}{ (1-\beta)^4 } \sum_{\tau=0}^{t-1} \left[\beta^{t-\tau-1} \mathbb{E}_{\xi_{(t)}} \verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i ) }^2\right]
\end{align}
where $	Z_1 = \frac{\eta }{2(1-\beta) } - \frac{L\eta^2}{2(1-\beta)^2}$, $R_1(t)=\sum_{i=1}^{n} \Vert \bx^{(t)}_i -  {\blx}^{(t)} \Vert^2$, $R_2(t) =\sum_{i=1}^{n} \Vert {\blx}^{(t)} -  {\btx}^{(t)} \Vert^2 $.
Taking expectation and using Lemma \ref{lemm_dec_li_sgd_fix} (stated below and proved in our full paper \cite{singh2020squarm}) to bound $\bbE[R_2(t)]$ with $\eta \leq \frac{(1-\beta)^2}{2L}$, we get:
%Similar to \eqref{eq:thm_cvx_interim4}, we can show that 
%$R_1(t) = \sum_{j=1}^n \mathbb{E} \Vert \bar{\bx}^{{(t)}} -  \bx^{{(t)}}_{j} \Vert^2  \leq 2\mathbb{E} \sum_{j=1}^n \Vert \bar{\bx}^{I_{(t_0)}} - \bx^{I_{(t_0)}}_{j} \Vert^2  
%+ 4\eta_{I_{(t+1)_0}}^2 H^2 n G^2 \left( 1 + \frac{\beta^2}{(1- \beta)^2} \right)$.
%Now, in order to bound the RHS of \eqref{eq:proof_out_interim5}, we use Lemma \ref{lemm_dec_li_sgd_fix} stated below and $\eta \leq \frac{(1-\beta)^2}{2L}$ to get:
\begin{align} \label{eq:proof_out_interim4}
&  \Sigma:=\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \Vert \frac{1}{n} \sum_{i=1}^{n}  \nabla f_i(\bx^{(t)}_i) \Vert^2  \leq \notag \\ 
 &  \frac{4(1-\beta)}{\eta }\frac{(\mathbb{E}[f({\bx}^{(0)})] {-} f^*)}{T} 
 {+} \frac{4L^2 }{ n T} \sum_{t=0}^{T-1} \mathbb{E} [R_1(t)]  {+} Z_2
\end{align}
where $Z_2 = \frac{2L\eta \bar{\sigma}^2}{n   (1-\beta)}+ \frac{4L^2 \eta^2 \beta^4 \bar{\sigma}^2 }{n (1-\beta)^4 }$.
Note that \eqref{eq:proof_out_interim4} bounds $\Sigma=\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \Vert\frac{1}{n} \sum_{i=1}^{n} \nabla f_i(\bx^{(t)}_i) \Vert^2$, whereas, our goal is to bound $\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \Vert \nabla f({\blx}^{(t)})\Vert^2$. Using %, where $\nabla f({\blx}^{(t)}) = \frac{1}{n}\sum_{i=1}^n\nabla f_i({\blx}^{(t)})$.
$L$-Lipschitz gradient property of $f$ gives
%\begin{align} \label{eq:proof_out_interim2}
%\textstyle \frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \verts{ \nabla f({\blx}^{(t)})}^2  \leq \frac{2L^2}{nT} \sum_{t=0,}^{T-1}  \mathbb{E} [R_1(t)] \notag \\
% +  \frac{2}{T} \sum_{t=0}^{T-1} \mathbb{E}  \verts{ \frac{1}{n} \sum_{i=1}^{n} \nabla f_i(\bx^{(t)}_i)}^2
$\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \Vert \nabla f({\blx}^{(t)})\Vert^2  \leq \frac{2L^2}{nT} \sum_{t=0,}^{T-1}  \mathbb{E} [R_1(t)] +  2\Sigma$.
%\end{align}
Substituting the bound on $\Sigma$ from \eqref{eq:proof_out_interim4}, we get
\begin{align}\label{eq:proof_out_interim2}
\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \Vert \nabla f({\blx}^{(t)})\Vert^2  &\leq
\frac{8(1-\beta)}{\eta }\frac{(\mathbb{E}[f({\bx}^{(0)})] {-} f^*)}{T} \notag \\
&\quad + \frac{10L^2 }{ n T} \sum_{t=0}^{T-1} \mathbb{E} [R_1(t)]  + 2Z_2.
\end{align}
\begin{lemma}\label{lemm_dec_li_sgd_fix}
	Consider the assumptions of Theorem \ref{convergence_results} and let $I_{(t)} \in\I_T$ be a synchronization index. Let 	 $A = \frac{p}{2}\left(  2 H^2 G^2 \left( 1 {+} \frac{9\beta^2}{(1-\beta)^4} \right) \left( \frac{16}{\omega} {+} \frac{4}{p} \right) + \frac{2\omega c_0 }{\eta^{(1-\epsilon)}} \right)$. Then: 
	\begin{align*}
	\textstyle \sum_{j=1}^n \mathbb{E}\Vert {\blx}^{I_{(t)}} - \bx^{I_{(t)}}_{j} \Vert^2  & \leq \frac{4nA\eta^2}{p^2} \\ 
	\textstyle \mathbb{E}[R_2(t)] = \sum_{i=1}^{n} \mathbb{E} \Vert {\blx}^{(t)} -  {\btx}^{(t)} \Vert^2 & \leq \frac{n \beta^4 \eta^2}{(1-\beta)^3} \textstyle \sum_{\tau=0}^{t-1} \phi(t,\tau)
	\end{align*}
	 where $\phi(t,\tau) = \beta^{t-\tau-1}\mathbb{E}\verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i ) }^2 $.
\end{lemma}
Let $I_{(t_0)} \in \mathcal{I}_T$ denote the last synchronization index before time $t$.
The assumption $gap(\I_T)\leq H$ implies $t-I_{(t_0)}\leq H$.  
Using this and assumption {\sf (ii)}, we can bound: %write the bound for $\mathbb{E}[R_1(t)]=\sum_{i=1}^{n} \mathbb{E} \Vert {\blx}^{(t)} - \bx^{(t)}_i \Vert^2$ as:
\begin{align}\label{eq:thm_cvx_interim4}
\mathbb{E}[R_1(t)] =  \sum_{j=1}^n \mathbb{E} \Vert  {\blx}^{{(t)}} & -  \bx^{{(t)}}_{j} \Vert^2  \leq 2\mathbb{E} \sum_{j=1}^n \Vert {\blx}^{I_{(t_0)}} - \bx^{I_{(t_0)}}_{j} \Vert^2 \notag \\
 & + 4\eta^2 H^2 n G^2 \left( 1 + \frac{9\beta^2}{(1- \beta)^4} \right) 
\end{align}
Now use Lemma~\ref{lemm_dec_li_sgd_fix} to get a bound on $\bbE[R_1(t)]$ and  
then substitute the resulting bound into \eqref{eq:proof_out_interim2}. % and then substitute the bound for $\bbE[R_1(t)]$. 
%As we require a bound for the global objective $f$ evaluated at the global average $\bar{\bx}^{(t)}$, we substitute the resulting bound for $\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \verts{\frac{1}{n} \sum_{i=1}^{n} \nabla f_i(\bx^{(t)}_i) }^2 $ from \eqref{eq:proof_out_interim4} in \eqref{eq:proof_out_interim2} to obtain a bound for $\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} \verts{ \nabla f(\bar{\bx}^{(t)})}^2$.
%Note that for the case of fixed learning rate $\eta$, we have to fix the number of iterations $T$ before the algorithm begins.
We then expand on the value of $A$ from Lemma \ref{lemm_dec_li_sgd_fix} and set $\eta= (1-\beta) \sqrt{\frac{n}{T}}$ for $T \geq \frac{4L^2 n }{(1-\beta)^2}$. 
Using $p \geq \frac{\delta^2 \omega}{644}$ completes the proof of Theorem~\ref{convergence_results}. 
%\qed
%------------------------------------------------------------------


}


==> results_with_relaxed_assumptions.tex <==
%------------------------------------------------------------------
\allowdisplaybreaks{
\section{Results with Relaxed Assumptions: Proof of Theorem \ref{convergence_relaxed_assump}}\label{sec:relaxed-assump-results}


%{\sf (i)} {\textit{$L$-Smoothness}:} Each local function $f_i$ for $i \in [n]$ is $L$-smooth, i.e., $\forall \bx,\by \in \mathbb{R}^d$, we have $f_i(\by) \leq f_i(\bx) + \langle \nabla f_i(\bx), \by-\bx  \rangle + \frac{L}{2} \Vert \by-\bx \Vert^2$. \\
%{\sf (i)} {\textit{Bounded variance:}} For every $i\in[n]$, we have $\mathbb{E}_{\xi_i} \Vert \nabla F_i (\bx,\xi_i) - \nabla f_i(\bx) \Vert^2 \leq \sigma_i^2$, for some finite $\sigma_i$,
%where $\nabla F_i (\bx,\xi_i)$ denotes an unbiased stochastic gradient at worker $i$ with $\mathbb{E}_{\xi_i} [\nabla F_i (\bx ,\xi_{i})] = \nabla f_i (\bx)$. We define $\bar{\sigma}^2 := \frac{1}{n} \sum_{i=1}^{n}  \sigma_i ^2$.\\ 
%{\sf (ii)} {\textit{Bounded second moment:}} For every $i\in[n]$, we have $\mathbb{E}_{\xi_i} \Vert \nabla F_i (\bx,\xi_{i}) \Vert^2 \leq G^2$, for some finite $G$. 
%This is a standard assumption in stochastic optimization with compressed gradients \cite{stich_sparsified_2018,basu_qsparse-local-sgd:_2019,koloskova_decentralized_2019,distributed_momentum19}. \\
%{\sf (iii)} {\textit{Smoothness of objectives:}} We assume that each local objective $f_i$ is $L$-smooth\footnote{$f_i$ is $L$-smooth, if for every $\bx,\by\in\R^d$, we have $f_i(\by) \leq f_i(\bx) + \langle \nabla f_i(\bx), \by-\bx  \rangle + \frac{L}{2} \Vert \by-\bx \Vert^2$. \label{l-smooth-footnote}} for all $i \in [n].$

%------------------------------------------------------------------
%\begin{theorem}\label{convergence_results}
%	Let $\C$ be a compression operator with parameter $\omega \in (0,1]$ and  let $gap(\I_T)\leq H$. Consider running SQuARM-SGD under assumptions {\sf (i)-(iii)} above with consensus step-size $\gamma = \frac{2\delta \omega}{64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega}, (\text{where }\lambda = \text{max}_i \{ 1- \lambda_i(W) \})$,  momentum coefficient $\beta\in[0,1)$, learning rate $\eta = (1-\beta)\sqrt{\frac{n}{T}}$ and a threshold function $c_t \leq \frac{c_0}{\eta^{1-\epsilon}}$ for all $t$ where $\epsilon \in (0,1)$. 
%If $T \geq \frac{4L^2 n }{(1-\beta)^2}$, then the averaged iterates $\blx^{(t)} := \frac{1}{n} \sum_{i=0}^n \bx_i^{(t)}$ satisfy:
%		\begin{align*}
%			&\frac{\sum_{t=0}^{T-1}  \mathbb{E} \Vert \nabla f(\blx^{(t)}) \Vert_2^2}{T} =  \mathcal{O}  \left(  \frac{J^2 + \bar{\sigma}^2 }{\sqrt{nT}} + \frac{c_0 n^{\nicefrac{(1+\epsilon)}{2}}}{ \delta^2 T^{\nicefrac{(1+\epsilon)}{2}}  } +   \frac{nH^2G^2}{T \delta^4 \omega^2  } + \frac{  \beta^4 \bar{\sigma}^2 }{T (1-\beta)^2 }  \right), 
%		\end{align*}
%	where $J^2 < \infty$ is a constant such that $\mathbb{E}[f(\blx^{(0)})] - f^* \leq J^2 $.
%\end{theorem}


%\TODO{
%\begin{theorem}\label{convergence_relaxed_assump}
%	Let $\C$ be a compression operator with parameter $\omega \in (0,1]$ and  $gap(\I_T)= H$. Consider running SQuARM-SGD for $T$ iterations with consensus step-size $\gamma = \frac{2\delta \omega}{64 \delta + \delta^2 + 16 \lambda^2 + 8 \delta \lambda^2 - 16\delta \omega}$, $(\text{where }\lambda = \text{max}_i \{ 1- \lambda_i(\mathbf{W}) \})$, a threshold sequence $c_t \leq \frac{c_0}{\eta^{1-\epsilon}}$ for all $t$ where $\epsilon \in (0,1)$ and $c_0$ is a constant, momentum coefficient $\beta\in[0,1)$, and constant learning rate $\eta=(1-\beta)\sqrt{\frac{n}{T}}$. Let the algorithm generate $\{ \bx_i ^{(t)}  \}_{t=0}^{T-1}$ for $i\in[n]$. Then, we have the following guarantees:
%	\begin{itemize}%[ \bf 1]
%		\item{\bf[Non-convex:]} \label{thm_noncvx_fix_li} For $ T \geq \max \{ 16L^2n, \frac{8L^2 \beta^4 n}{(1-\beta)^2}  \} $, the averaged iterates $\blx^{(t)} := \frac{1}{n} \sum_{i=0}^n \bx_i^{(t)}$ satisfy:
%		\begin{align*}
%		&\frac{\sum_{t=0}^{T-1}  \mathbb{E} \Vert \nabla f(\blx^{(t)}) \Vert_2^2}{T} =  \mathcal{O}  \left(  \frac{J^2 + \bar{\sigma}^2 }{\sqrt{nT}} + \frac{c_0 n^{\nicefrac{(1+\epsilon)}{2}}}{ \delta^2 T^{\nicefrac{(1+\epsilon)}{2}}  } +   \frac{nH^2G^2}{T \delta^4 \omega^2  } + \frac{  \beta^4 \bar{\sigma}^2 }{T (1-\beta)^2 }  \right),
%		\end{align*}
%		where $J^2 < \infty$ is such that $\mathbb{E}[f(\blx^{(0)})] - f^* \leq J^2 $.
%		\item{\bf[Convex:]} \label{thm_cvx_li}  If $\{f_i\}_{i \in [n]}$ are convex, then for $T \geq \max\{ (8L)^2n,\frac{(8\beta^2L)^4n}{(1-\beta)^2}\}$, we have:
%		\begin{align*}
%		& \mathbb{E}[f(\blx^{(T)}_{avg})] - f^* =  \mathcal{O}\left( \frac{\|\blx^{(0)} - \bx^*\|^2 + \bar{\sigma}^2} {\sqrt{nT}}  + \frac{c_0  n^{\nicefrac{(1+\epsilon)}{2}}}{\delta^2 T^{\nicefrac{(1+\epsilon)}{2}}} + \frac{n^{\nicefrac{3}{4}} \beta^2 G^2}{(1-\beta)^{\nicefrac{3}{2}} T^{\nicefrac{3}{4}}}   + \frac{nH^2G^2}{\delta^4 \omega^2T}     \right),
%		\end{align*}
%		where $\blx^{(T)}_{avg} := \frac{1}{T} \sum_{t=0}^{T-1} \blx^{(t)}$ for $\blx^{(t)} = \frac{1}{n} \sum_{i=1}^{n} \bx^{(t)}_{i}$ and $\bx^{*}$ is an optimizer of $f$ with optimal value denoted by $f^{*}$.
%
%	\end{itemize}
%\end{theorem}
%\noindent We have used simplified convergence rate expressions in the above results, and provide precise rate expressions in the proofs provided in Section \ref{proof_thm_noncvx} and Section \ref{proof_thm_cvx} for non-convex and convex objectives, respectively. 
%}
%------------------------------------------------------------------

%\paragraph{Effects of parameters on convergence:} Observe that the factors $H, c_0,\omega,\delta$ to achieve communication efficiency -- $H,c_0$ for the event-triggered communication, $\omega$ for compression, and $\delta$ for the connectivity of the underlying graph -- do not affect the dominant terms in convergence rate for either non-convex and convex objectives in Theorem~\ref{convergence_results} and appear only in the higher order terms. 
%This implies that if we run SQuARM-SGD for sufficiently long, precisely, for at least $T_0:=C_0\times\max\left\{\left(\frac{c_0 n^{(2+\epsilon)}}{(J^2+\bar{\sigma}^2)^{2}  \delta^4 }\right)^{\nicefrac{1}{\epsilon}}{,}  \frac{n}{(J^2+\bar{\sigma}^2)^2} \left(\frac{nG^2H^2}{\omega^2\delta^4 (1-\beta)^2}  {+} \frac{\beta^4 \bar{\sigma}^2}{(1-\beta)^2}  \right)^2 \right\}$ iterations for a sufficiently large constant $C_0$, then SQuARM-SGD converges at a rate of $\mathcal{O}  \left(\nicefrac{1}{\sqrt{nT}} \right)$.	Note that this is the convergence rate of distributed {\em vanilla} SGD with the same speed-up w.r.t.\ the number of nodes $n$. Thus, we essentially converge at the same rate as vanilla SGD, while saving significantly in terms of total communication bits; this can be seen in our numerical results in Section \ref{experiments} as well.
\iffalse
\paragraph{Effects of parameters on convergence:} Observe that the factors $H, c_0,\omega,\delta$ to achieve communication efficiency -- $H,c_0$ for the event-triggered communication, $\omega$ for compression, and $\delta$ for the connectivity of the underlying graph -- do not affect the dominant terms in convergence rate for either non-convex or convex objectives in Theorem~\ref{convergence_results} and appear only in the higher order terms. 
This implies that if we run SQuARM-SGD for sufficiently long, precisely, for at least $T_0:=C_0\times\max\left\{\left(\frac{c_0^2 n^{(2+\epsilon)}}{(J^2+\bar{\sigma}^2)^{2}  \delta^4 }\right)^{\nicefrac{1}{\epsilon}}{,}  \frac{n}{(J^2+\bar{\sigma}^2)^2} \left(\frac{nG^2H^2}{\omega^2\delta^4 }  {+} \frac{\beta^4 \bar{\sigma}^2}{(1-\beta)^2}  \right)^2 \right\}$ iterations for non-convex objectives and for $T_1 := C_1 \times \max \left\{ \left(\frac{c_0^2 n^{2+\epsilon}}{\delta^4 ( \Vert \blx^{(0)} - \bx^{*} \Vert^2 + \bar{\sigma}^2 )^2}\right)^{\nicefrac{1}{\epsilon}} , \frac{n^3 H^4 G^2}{\delta^8 \omega^4 ( \Vert \blx^{(0)} - \bx^{*} \Vert^2 + \bar{\sigma}^2 )^2} , \frac{n^{5} G^8 \beta^8 }{(1-\beta)^6 ( \Vert \blx^{(0)} - \bx^{*} \Vert^2 + \bar{\sigma}^2 )^4 }    \right\}$ for convex objectives with sufficiently large constants $C_0$ and $C_1$, respectively, then SQuARM-SGD converges at a rate of $\mathcal{O}  \left(\nicefrac{1}{\sqrt{nT}} \right)$. Note that this is the convergence rate of distributed {\em vanilla} SGD with the same speed-up w.r.t.\ the number of nodes $n$ in both these settings. Thus, we essentially converge at the same rate as that of vanilla SGD, while saving significantly in terms of total communicated bits; this can be seen in our numerical results in Section \ref{experiments} as well.
\fi

In order to prove Theorem \ref{convergence_relaxed_assump}, we define a virtual sequence ${\btx}_i^{(t)}$ for each node $i\in[n]$, as follows:
\begin{align} \label{virt_seq}
{\btx}_i^{(t)} = {\bx}_i^{(t)} - \frac{\eta \beta^2}{(1-\beta)} \bv_i^{(t-1)}; \qquad \btx_i^{(0)}:=\bx_i^{(0)}.
\end{align}
%
This remaining section is divided into seven subsections. 
In Section~\ref{subsec:sgd-update-virtual}, we derive an SGD like update rule for the virtual sequence.
In Section~\ref{subsec:proof-outline-relaxed-thm}, we provide a proof-outline of Theorem~\ref{convergence_relaxed_assump}. The remaining subsections are dedicated to prove the lemmas stated in the proof outline given in Section~\ref{subsec:proof-outline-relaxed-thm}.
%
\subsection{Deriving an SGD-Like Update Rule for the Virtual Sequene}\label{subsec:sgd-update-virtual}
In \eqref{virt_seq}, $\bx_i^{(t)}$ is the true local parameter at node $i$ at the $t$'th iteration, which is equal to (see line 16 of Algorithm \ref{alg_dec_sgd_li}):
\begin{align*}
\bx_i^{(t)} = \bx_i^{(t-\frac{1}{2})} + \mathbbm{1}_{\{t \in \mathcal{I}_T\}}\gamma \sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t)} - \hat{\bx}_i^{(t)}),
\end{align*}
where $\bx_i^{(t-\frac{1}{2})} = \bx_i ^{(t-1)} - \eta (\beta \bv_i^{(t-1)} + \nabla F_i(\bx_i^{(t-1)}, \xi_i^{(t-1)}))$ (line 5 in Algorithm \ref{alg_dec_sgd_li}).
Note that we changed the summation from $j\in\mathcal{N}_i$ to $j=1$ to $n$; this is because $w_{ij}=0$ whenever $j\notin\mathcal{N}_i$.

Let ${\blx}^{(t)} = \frac{1}{n} \sum_{i=1}^{n} \bx_{i}^{(t)}$ denote the average of the local iterates at time $t$.
Now we argue that ${\blx}^{(t)}={\blx}^{(t-\frac{1}{2})}$.
This trivially holds when $t\notin \I_T$. For the other case, i.e., $t\in \I_T$, this follows because
$\sum_{i=1}^n\sum_{j=1}^n w_{ij} (\hat{\bx}_j^{(t)} - \hat{\bx}_i^{(t)})=0$, which uses the fact that $W$ is a doubly stochastic matrix. 
Thus, we have 
\begin{equation}\label{eq:thm_cvx_interim0}
{\blx}^{(t)} =  {\blx}^{(t-1)} - \frac{\eta}{n}\sum_{i=1}^n \left(\beta \bv_i^{(t-1)} + \nabla F_i(\bx_i^{(t-1)}, \xi_i^{(t-1)})\right).
\end{equation}
Taking average over all the nodes in \eqref{virt_seq} and defining ${\btx}^{(t)} := \frac{1}{n}\sum_{i=1}^n{\btx}_i^{(t)}$, we get
\begin{align*}
{\btx}^{(t)} = {\blx}^{(t)} - \frac{\eta \beta^2}{(1-\beta)} \frac{1}{n} \sum_{i=1}^n \bv_i^{(t-1)}.
\end{align*}
%Note that the columns of ${\btX}^{(t+1)}$ are identical and equal to $\btx^{(t)}$. 
We now note a recurrence relation for the sequence ${\btx}^{(t+1)}$:
\begin{align} \label{virt_seq_rec}
{\btx}^{(t+1)} & = {\blx}^{(t+1)} - \frac{\eta \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n \bv_i^{(t)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta}{n}\sum_{i=1}^n \left(\beta \bv_i^{(t)} + \nabla F_i(\bx_i^{(t)}, \xi_i^{(t)})\right) - \frac{\eta \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n \bv_i^{(t)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) -  \left( \eta \beta + \frac{\eta \beta^2}{(1-\beta)}\right)  \frac{1}{n}\sum_{i=1}^n \bv_i^{(t)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) - \frac{\eta \beta}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n\left[\beta\bv_i^{(t-1)}  + \nabla F_i(\bx_i^{(t)},\xi_i^{(t)})\right] \notag \\
& =  {\blx}^{(t)} - \left(\eta + \frac{\eta\beta}{(1-\beta)} \right)\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) - \frac{\eta \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n\bv_i^{(t-1)} \notag \\
& =  {\blx}^{(t)} - \frac{\eta \beta^2}{(1-\beta)} \frac{1}{n}\sum_{i=1}^n\bv_i^{(t-1)} - \frac{\eta}{(1-\beta)}\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)}) \notag \\
& =  {\btx}^{(t)} - \frac{\eta}{(1-\beta)}\frac{1}{n} \sum_{i=1}^n \nabla F_i(\bx_i^{(t)},\xi_i^{(t)})
\end{align}

\subsection{Proof Outline of Theorem~\ref{convergence_relaxed_assump}}\label{subsec:proof-outline-relaxed-thm}
The proof is divided into four lemmas. The first lemma (stated in Lemma~\ref{lem:similar-lem11}) derives the required convergence bound, however, the RHS depends on the deviation of local parameter vectors from the average parameter vector (i.e., $\Xi^{(t)}:=\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2$), which we have to bound. The remaining three lemmas are dedicated to bounding this quantity. 

Note that bounding this in the {\em distributed} setup is not difficult, as at synchronization indices all parameters are the same because it is coordinated by a central server. This means that at any time index $t\in[T]$, there is always a time index $t-H\leq t'\leq t$ when $\bx_i^{(t')}$ for all $i\in[n]$ are the same, and we have a reference point no too far in the past. However, in the decentralized setup, there is no central server for coordinating the updates, and hence there is no reference point in the past when the local parameters are the same. Moreover, our assumptions are arguably the weakest in literature, and we also are working with compression and momentum updates. Therefore, bounding $\Xi^{(t)}$ in our setup is highly non-trivial, and bounding this is one of the major technical contributions of our work.
\begin{lemma}\label{lem:similar-lem11}
When $\eta\leq\min\left\{\frac{2(1-\beta)^3}{9\beta^4},\frac{2(1-\beta)^2}{3\beta^2L}\sqrt{\frac{n}{M^2+n}},\frac{(1-\beta)^2}{6\beta^2LB}\sqrt{\frac{n}{2(M^2+n)}}\right\}$, we get
\begin{align*}
\frac{1}{T}\sum_{t=0}^{T-1}\bbE\verts{\nabla f(\blx^{(t)})}_2^2 &\leq \frac{16(1-\beta)(f(\blx^{(0)}) - f^*)}{\eta T} + \frac{16\eta L}{(1-\beta)}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\quad + \frac{64 L^2}{n}\frac{1}{T}\sum_{t=0}^{T-1}\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2.
\end{align*}
\end{lemma}
We prove Lemma~\ref{lem:similar-lem11} in Section~\ref{subsec:proof-similar-lem11}.

Fix an arbitrary $t\in[T]$.
We bound $\Xi^{(t)}=\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2$ via another quantity $S^{(t)}$ defined as
%
\[S^{(t)} := \Xi^{(t)} + \bbE\verts{\bX^{(t)} - \bhX^{((m+1)H)}}_F^2, \quad \text{ where } m=\lfloor\frac{t}{H}\rfloor - 1.\]
%
We derive two upper bounds on $S^{(t)}$ depending on the value of $t$. Note that in both the following lemmas, $m=\lfloor\frac{t}{H}\rfloor - 1$.
\begin{lemma}\label{lem:similar-eq16}
Consider any $t\in[T]$. Then for $m=\lfloor\frac{t}{H}\rfloor -1$, we have the following bound for $(m+1)H\leq t \leq (m+2)H-1$:
\begin{align*}
S^{(t)} &\leq \(1-\frac{\gamma\delta}{4}\)S^{(mH)} + 2c_1\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + c_1\eta^2H\beta^2\sum_{t'=mH}^{t-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\quad + 2c_1\eta^2H(M^2+1)L^2\sum_{t'=mH}^{t-1}S^{(t')} + 2c_1\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{t-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2,
\end{align*}
where $c_1 \leq 2(1+\frac{\gamma\delta}{4})\(\frac{3}{\gamma\delta} + \frac{9\lambda^2}{\delta^2} + \frac{45\gamma\lambda^2}{\delta\omega} + \frac{104\gamma^2\lambda^2}{\omega^2} + \frac{4}{\omega} - 2\) + 4(1+\frac{4}{\gamma\delta})$.
\end{lemma}
We prove Lemma~\ref{lem:similar-eq16} in Section~\ref{subsec:proof-similar-eq16}.
\begin{lemma}\label{lem:similar-eq17}
We have the following bound for $mH\leq \hatt < (m+1)H$:
\begin{align*}
S^{(\hatt)} &\leq \(1+\frac{\gamma\delta}{4}\)S^{(mH)} + 2c_1\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + c_1\eta^2H\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\quad + 2c_1\eta^2H(M^2+1)L^2\sum_{t'=mH}^{\hatt-1}S^{(t')} + 2c_1\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2,
\end{align*} 
where $c_1$ is exactly the same as in Lemma~\ref{lem:similar-eq16}.
\end{lemma}
We prove Lemma~\ref{lem:similar-eq17} in Section~\ref{subsec:proof-similar-eq17}.

%
Using both these lemmas, we will be able to bound $\Xi^{(t)}$. We state the result in the following lemma, which we prove in Section~\ref{subsec:proof-similar-lem14}.
\begin{lemma}\label{lem:similar-lem14}
When $\eta \leq \min\left\{\sqrt{\frac{\gamma\delta}{512c_1H^2(M^2+1)L^2}},\sqrt{ \frac{  \alpha (1-\beta) }{128 D H (M^2+1)L^2}}\right\}$, we have the following bound:
	\begin{align*}
	\frac{1}{T}\sum_{t=0}^{T-1}\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2 =	\frac{1}{T}\sum_{t=0}^{T-1} S^{(t)} & \leq 2\eta^2 J_1 + 2\eta^2 J_2 \frac{1}{T}\sum_{t=0}^{T-1}  \bbE \verts{ \nabla f (\blx^{(t)}) }^2,
	\end{align*}
	where $J_1= \left(\frac{32HA}{\alpha} + \left( \frac{32 D H}{\alpha} \right)  \left( \frac{2(M^2+1)nG^2 + n \sigma^2}{(1-\beta)}   \right)   \right)$ and $J_2=\left(\frac{32C  H}{\alpha}   + \left( \frac{32 D H }{\alpha} \right) \frac{2(M^2+1)nB^2}{(1-\beta)}\right)$, where $A=2c_1H^2n\(2(M^2+1)G^2 + \sigma^2\)$, $C=2c_1H(M^2+1)nB^2$, and $D=\frac{c_1H\beta^2}{(1-\beta)}$, and $c_1$ is exactly the same as in Lemma~\ref{lem:similar-eq16}.
\end{lemma}
%
Substituting the bounds from Lemma~\ref{lem:similar-lem14} into Lemma~\ref{lem:similar-lem11} and choosing $\eta=(1-\beta)\sqrt{\frac{n}{T}}$ (and running the algorithm for a sufficiently long time) completes the proof. Details with exact numbers are provided in Appendix~\ref{app:completing-proof}.

\subsection{Proof of Lemma~\ref{lem:similar-lem11}}\label{subsec:proof-similar-lem11}
Consider the quantity $\mathbb{E}_{\xi_{(t)}} [f(\btx^{(t+1)})] $ where expectation is taken w.r.t. the sampling at time $t$. From the recurrence relation of the virtual sequence \eqref{virt_seq_rec}, we have:
\begin{align}
&\mathbb{E}_{\xi_{(t)}} [f(\btx^{(t+1)})] = \mathbb{E}_{\xi_{(t)}} f \left(\btx^{(t)}  - \frac{\eta}{(1-\beta)} \frac{1}{n} \sum_{i=1}^{n} \nabla F_i(\bx^{(t)}_i, \xi^{(t)}_i) \right) \notag \\
&\stackrel{\text{(a)}}{\leq} f(\btx^{(t)}) \underbrace{- \lragnle{\nabla f(\btx^{(t)}) , \frac{\eta}{(1-\beta)} \frac{1}{n} \sum_{i=1}^{n}\nabla f_i(\bx^{(t)}_i)}}_{=:\ P_1} + \frac{L}{2} \frac{\eta^2}{(1-\beta)^2} \underbrace{\mathbb{E}_{\xi_{(t)}} \verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i(\bx^{(t)}_i, \xi^{(t)}_i)}^2}_{=:\ P_2},\label{mom_noncvx_relaxed-interim6}
\end{align}
where (a) follows from the $L$-smoothness of $f$.
We show the following bounds on $P_1$ and $P_2$ in Appendix~\ref{app:proof-similar-lem11}.
\begin{align}
P_1 &\leq - \frac{\eta}{2(1-\beta)} \verts{\nabla f(\btx^{(t)})}^2 + \frac{\eta L^2}{2n(1-\beta)}\sum_{i=1}^n\verts{\btx^{(t)} - \bx^{(t)}_i}^2, \label{bound_P1} \\
P_2 &\leq \frac{\sigma^2}{n} + \frac{2(M^2+n)L^2}{n^2}\sum_{i=1}^n\verts{\bx^{(t)}_i - \btx^{(t)}}_2^2 + \frac{2(M^2+n)}{n}\big(G^2+B^2\verts{\nabla f(\btx^{(t)})}_2^2\big) \label{bound_P2}
\end{align}

Substituting the bounds from \eqref{bound_P1} and \eqref{bound_P2} into \eqref{mom_noncvx_relaxed-interim6}, we get
\begin{align}
\mathbb{E}_{\xi_{(t)}} [f(\btx^{(t+1)})] &\leq f(\btx^{(t)}) + \frac{\eta^2L}{2(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\quad + \Big(\frac{\eta L^2}{2n(1-\beta)}+ \frac{\eta^2L^3(M^2+n)}{n^2(1-\beta)^2}\Big) \sum_{i=1}^n\verts{\bx^{(t)}_i - \btx^{(t)}}_2^2 \notag \\
&\qquad - \Big(\frac{\eta}{2(1-\beta)} - \frac{\eta^2L(M^2+n)B^2}{n(1-\beta)^2}\Big)\verts{\nabla f(\btx^{(t)})}_2^2. \label{mom_noncvx_interim7}
\end{align}
%
When $\eta\leq \frac{n(1-\beta)}{2L(M^2+n)}$, we get $\Big(\frac{\eta L^2}{2n(1-\beta)}+ \frac{\eta^2L^3(M^2+n)}{n^2(1-\beta)^2}\Big) \leq \frac{\eta L^2}{n(1-\beta)}$; and when $\eta \leq \frac{n(1-\beta)}{4LB^2(M^2+n)}$, we get $\Big(\frac{\eta}{2(1-\beta)} - \frac{\eta^2L(M^2+n)B^2}{n(1-\beta)^2}\Big)\geq\frac{\eta}{4(1-\beta)}$. Therefore, when $\eta\leq\min\{\frac{n(1-\beta)}{2L(M^2+n)},\frac{n(1-\beta)}{4LB^2(M^2+n)}\}$, we get
\begin{align}
\mathbb{E}_{\xi_{(t)}} [f(\btx^{(t+1)})] &\leq f(\btx^{(t)}) + \frac{\eta^2L}{2(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\qquad + \frac{\eta L^2}{n(1-\beta)}\sum_{i=1}^n\verts{\bx^{(t)}_i - \btx^{(t)}}_2^2 - \frac{\eta}{4(1-\beta)}\verts{\nabla f(\btx^{(t)})}_2^2. \label{mom_noncvx_interim8}
\end{align}
By Jensen's inequality and $L$-smoothness of $f$, we have $\verts{\nabla f(\blx^{(t)})}_2^2 \leq 2\verts{\nabla f(\blx^{(t)}) - \nabla f(\btx^{(t)})}_2^2 + 2\verts{\nabla f(\btx^{(t)})}_2^2 \leq 2L^2\verts{\blx^{(t)} - \btx^{(t)}}_2^2 + 2\verts{\nabla f(\btx^{(t)})}_2^2$. Rearranging this gives $\verts{\nabla f(\btx^{(t)})}_2^2 \geq \frac{1}{2}\verts{\nabla f(\blx^{(t)})}_2^2 - L^2\verts{\blx^{(t)} - \btx^{(t)}}_2^2$. Substituting this in \eqref{mom_noncvx_interim8} and rearranging yields
\begin{align}
\frac{\eta}{8(1-\beta)}\verts{\nabla f(\blx^{(t)})}_2^2 &\leq f(\btx^{(t)}) - \mathbb{E}_{\xi_{(t)}} [f(\btx^{(t+1)})] + \frac{\eta^2L}{2(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\quad + \frac{\eta L^2}{n(1-\beta)}\sum_{i=1}^n\verts{\bx^{(t)}_i - \btx^{(t)}}_2^2 + \frac{\eta L^2}{4(1-\beta)}\verts{\blx^{(t)} - \btx^{(t)}}_2^2 \notag \\
&\hspace{-2cm} \leq f(\btx^{(t)}) - \mathbb{E}_{\xi_{(t)}} [f(\btx^{(t+1)})] + \frac{\eta^2L}{2(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\hspace{-1.5cm} + \frac{2\eta L^2}{n(1-\beta)}\sum_{i=1}^n\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2 + \Big(\frac{2\eta L^2}{(1-\beta)} + \frac{\eta L^2}{4(1-\beta)}\Big)\verts{\blx^{(t)} - \btx^{(t)}}_2^2 \label{mom_noncvx_interim91}.
\end{align}
%
Now we bound $\verts{\blx^{(t)} - \btx^{(t)}}_2^2$ in the following lemma, which we prove in Appendix~\ref{app:proof-similar-lem11} in supplementary material: 
\begin{lemma}\label{glob_virt_bound}
Consider the deviation of the global average parameter $\blx^{(t)}$  and the virtual sequence $\btx^{(t)}$ defined in \eqref{virt_seq} for constant stepsize $\eta$. Then at any time step $t$, the following holds:
\begin{align}\label{eq:glob_virt_bound}
\verts{ \blx^{(t)} -  \btx^{(t)}}^2 & \leq \frac{\beta^4 \eta^2}{(1-\beta)^3}  \sum_{\tau=0}^{t-1} \left[\beta^{t-\tau-1}\verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i ) }^2\right]
\end{align}
\end{lemma}
%
Substituting the bound from \eqref{eq:glob_virt_bound} into \eqref{mom_noncvx_interim91} and then taking the expectation w.r.t.\ the entire past and average over $t=0$ to $t=T-1$ gives
\begin{align}
&\frac{\eta}{8(1-\beta)}\frac{1}{T}\sum_{t=0}^{T-1}\bbE\verts{\nabla f(\blx^{(t)})}_2^2 \leq \frac{1}{T}\bbE[f(\btx^{(0)}) - f(\btx^{(T)})] + \frac{\eta^2L}{2(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&+ \frac{1}{T}\sum_{t=0}^{T-1}\(\frac{2\eta L^2}{n(1-\beta)}\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2 + \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4}\sum_{\tau=0}^{t-1} \beta^{t-\tau-1}\bbE\verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i ) }^2\). \label{mom_noncvx_interim910}
\end{align}
%
In the following lemma (which we prove in Appendix~\ref{app:proof-similar-lem11}) we bound the last term of \eqref{mom_noncvx_interim910}.
%
\begin{lemma}\label{lem:bound-decaying-grads}
\begin{align}\label{eq:bound-decaying-grads}
&\frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \left[\beta^{t-\tau-1}\bbE\verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i ) }^2\right] \leq \frac{\sigma^2}{n(1-\beta)} + \frac{2(M^2+n)G^2}{n(1-\beta)} \notag \\
&\quad + \frac{2(M^2+n)L^2}{n^2(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^n\bbE\verts{\bx^{(\tau)}_i - \blx^{(\tau)}}_2^2  + \frac{2(M^2+n)B^2}{n(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\bbE\|\nabla f(\blx^{(\tau)})\|_2^2.
\end{align}
\end{lemma}
%\begin{proof}
%We have already bounded the expectation term in \eqref{bound_P2} -- the same bound holds when expectation is taken w.r.t.\ the entire past. Substituting that bound (i.e., $\bbE\verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i )}^2 \leq \frac{\sigma^2}{n} + \frac{(M^2+n)}{n^2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\bx^{(\tau)}_i)}_2^2$) from \eqref{bound_P2-interim} into \eqref{eq:bound-decaying-grads} gives
%\begin{align}
%&\frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \left[\beta^{t-\tau-1}\bbE\verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i ) }^2\right] \leq \frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \beta^{t-\tau-1}\frac{\sigma^2}{n} \notag \\
%&\hspace{3cm} + \frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \beta^{t-\tau-1}\frac{(M^2+n)}{n^2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\bx^{(\tau)}_i)}_2^2 \label{bound-decaying-grads-interim1}
%\end{align} 
%Now we bound both the terms of \eqref{bound-decaying-grads-interim1} separately.
%\begin{align}
%\frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \beta^{t-\tau-1}\frac{\sigma^2}{n} &= \frac{\sigma^2}{n}\frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \beta^{t-\tau-1}\leq\frac{\sigma^2}{n(1-\beta)}. \label{bound-decaying-grads-interim2} \\
%\frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \beta^{t-\tau-1}\frac{(M^2+n)}{n^2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\bx^{(\tau)}_i)}_2^2 &= \frac{1}{T}\sum_{\tau=0}^{T-2} \sum_{t=\tau+1}^{T-1} \beta^{t-\tau-1}\frac{(M^2+n)}{n^2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\bx^{(\tau)}_i)}_2^2 \notag \\
%&\hspace{-7cm}= \frac{(M^2+n)}{n^2}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\bx^{(\tau)}_i)}_2^2 \sum_{t=\tau+1}^{T-1} \beta^{t-\tau-1} \notag \\
%&\hspace{-7cm}\leq \frac{(M^2+n)}{n^2(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\bx^{(\tau)}_i)}_2^2 \notag \\
%&\hspace{-7cm}\leq \frac{2(M^2+n)}{n^2(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\bx^{(\tau)}_i) - \nabla f_i(\blx^{(\tau)})}_2^2 + \frac{2(M^2+n)}{n^2(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^n\bbE\verts{\nabla f_i(\blx^{(\tau)})}_2^2 \notag \\
%&\hspace{-7cm}\leq \frac{2(M^2+n)}{n^2(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^nL^2\bbE\verts{\bx^{(\tau)}_i - \blx^{(\tau)}}_2^2 + \frac{2(M^2+n)}{n(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\big(G^2 + B^2\bbE\|\nabla f(\blx^{(\tau)})\|_2^2\big) \notag \\
%&\hspace{-7cm}\leq \frac{2(M^2+n)L^2}{n^2(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^n\bbE\verts{\bx^{(\tau)}_i - \blx^{(\tau)}}_2^2 + \frac{2(M^2+n)G^2}{n(1-\beta)} + \frac{2(M^2+n)B^2}{n(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\bbE\|\nabla f(\blx^{(\tau)})\|_2^2 \label{bound-decaying-grads-interim3}
%\end{align}
%Substituting the bounds from \eqref{bound-decaying-grads-interim2}, \eqref{bound-decaying-grads-interim3} into \eqref{bound-decaying-grads-interim1} yields \eqref{eq:bound-decaying-grads}, which proves Lemma~\ref{lem:bound-decaying-grads}.
%%\begin{align}
%%\frac{1}{T}\sum_{t=0}^{T-1} \sum_{\tau=0}^{t-1} \left[\beta^{t-\tau-1}\bbE\verts{\frac{1}{n} \sum_{i=1}^{n} \nabla F_i (\bx^{(\tau)}_i , \xi^{(\tau)}_i ) }^2\right] &\leq \frac{\sigma^2}{n(1-\beta)} + \frac{2(M^2+n)L^2}{n^2(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\sum_{i=1}^n\bbE\verts{\bx^{(\tau)}_i - \blx^{(\tau)}}_2^2 \notag \\
%%&\hspace{-3cm}+ \frac{2(M^2+n)G^2}{n(1-\beta)} + \frac{2(M^2+n)B^2}{n(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-2}\bbE\|\nabla f(\blx^{(\tau)})\|_2^2 \label{bound-decaying-grads-interim4}
%%\end{align}
%\end{proof}
%
Substituting the bound from \eqref{eq:bound-decaying-grads} into \eqref{mom_noncvx_interim10} and noting that $\btx^{(0)}=\blx^{(0)}$ and $f(\btx^{(T)})\geq f^*$, where $f^*=f(\bx^*)$, we get
\begin{align}
&\frac{\eta}{8(1-\beta)}\frac{1}{T}\sum_{t=0}^{T-1}\bbE\verts{\nabla f(\blx^{(t)})}_2^2 \leq \frac{f(\blx^{(0)}) - f^*}{T} + \frac{\eta^2L}{2(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\quad + \left(\frac{2\eta L^2}{n(1-\beta)} + \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4}\frac{2(M^2+n)L^2}{n^2(1-\beta)} \right)\frac{1}{T}\sum_{t=0}^{T-1}\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2 \notag \\
&\quad+ \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4} \left(\frac{\sigma^2}{n(1-\beta)} + \frac{2(M^2+n)G^2}{n(1-\beta)} \right)  +  \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4}\frac{2(M^2+n)B^2}{n(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-1}\bbE\|\nabla f(\blx^{(\tau)})\|_2^2 \notag \\
&= \frac{f(\blx^{(0)}) - f^*}{T} + \frac{\eta^2L}{2(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big)\Big(1+\frac{9\eta\beta^4}{2(1-\beta)^3}\Big) \notag \\
&\quad + \left(\frac{2\eta L^2}{n(1-\beta)} + \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4}\frac{2(M^2+n)L^2}{n^2(1-\beta)} \right)\frac{1}{T}\sum_{t=0}^{T-1}\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2 \notag \\
%&\qquad+ \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4} \left(\frac{\sigma^2}{n(1-\beta)} + \frac{2(M^2+n)G^2}{n(1-\beta)} \right) \notag \\
&\qquad +  \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4}\frac{2(M^2+n)B^2}{n(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-1}\bbE\|\nabla f(\blx^{(\tau)})\|_2^2 \label{mom_noncvx_interim11}
\end{align}
Note that 
{\sf (i)} when $\eta\leq\frac{2(1-\beta)^3}{9\beta^4}$, we have $\Big(1+\frac{9\eta\beta^4}{2(1-\beta)^3}\Big)\leq2$; 
{\sf (ii)} when $\eta\leq\frac{2(1-\beta)^2}{3\beta^2L}\sqrt{\frac{n}{M^2+n}}$, we have $\left(\frac{2\eta L^2}{n(1-\beta)} + \frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4}\frac{2(M^2+n)L^2}{n^2(1-\beta)} \right) \leq \frac{4\eta L^2}{n(1-\beta)}$; and
{\sf (iii)} when $\eta\leq\frac{(1-\beta)^2}{6\beta^2LB}\sqrt{\frac{n}{2(M^2+n)}}$, we have $\frac{9\eta^3\beta^4 L^2}{4(1-\beta)^4}\frac{2(M^2+n)B^2}{n(1-\beta)}\leq \frac{\eta}{16(1-\beta)}$.
So, when $\eta\leq\min\{\frac{2(1-\beta)^3}{9\beta^4},\frac{2(1-\beta)^2}{3\beta^2L}\sqrt{\frac{n}{M^2+n}},\frac{(1-\beta)^2}{6\beta^2LB}\sqrt{\frac{n}{2(M^2+n)}}\}$, we get
\begin{align}
&\frac{\eta}{8(1-\beta)}\frac{1}{T}\sum_{t=0}^{T-1}\bbE\verts{\nabla f(\blx^{(t)})}_2^2 \leq \frac{f(\blx^{(0)}) - f^*}{T} + \frac{\eta^2L}{(1-\beta)^2}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\quad + \frac{4\eta L^2}{n(1-\beta)}\frac{1}{T}\sum_{t=0}^{T-1}\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2 + \frac{\eta}{16(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-1}\bbE\|\nabla f(\blx^{(\tau)})\|_2^2 \label{mom_noncvx_interim12}
\end{align}
Taking $\frac{\eta}{16(1-\beta)}\frac{1}{T}\sum_{\tau=0}^{T-1}\bbE\|\nabla f(\blx^{(\tau)})\|_2^2$ to the LHS and multiplying both sides by $\frac{16(1-\beta)}{\eta}$ gives
\begin{align}
\frac{1}{T}\sum_{t=0}^{T-1}\bbE\verts{\nabla f(\blx^{(t)})}_2^2 &\leq \frac{16(1-\beta)(f(\blx^{(0)}) - f^*)}{\eta T} + \frac{16\eta L}{(1-\beta)}\Big(\frac{\sigma^2+2(M^2+n)G^2}{n}\Big) \notag \\
&\quad + \frac{64 L^2}{n}\frac{1}{T}\sum_{t=0}^{T-1}\sum_{i=1}^n\bbE\verts{\bx^{(t)}_i - \blx^{(t)}}_2^2 \label{mom_noncvx_interim13}
\end{align}
%
\subsection{Useful Lemmas}\label{subsec:useful-lemmas}
%
The following two lemmas (which we prove in Appendix~\ref{app:useful-lemmas}) will be useful for proving Lemma~\ref{lem:similar-eq16} and Lemma~\ref{lem:similar-eq17}.

\begin{lemma}\label{lem:cvx_e1_relaxed}
Under the setting of Theorem \ref{convergence_relaxed_assump}, for any $m\in\bbN$, we have 
\begin{align}
\bbE\verts{\bX^{((m+1)H)} - \blX^{((m+1)H)}}_F^2 &\leq  a_1 \bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + a_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
&\qquad+ a_3\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1}\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2, \label{eq:cvx_e1_relaxed}
\end{align}
where $a_1=(1+\alpha_5^{-1})R_1,$ $a_2=(1+\alpha_5^{-1}) R_2 (1+\tau_1)(1-\omega)(1+\tau_2),$ and $$a_3=\((R_1+R_2)(1+\alpha_5)+(1+\alpha_5^{-1}) R_2\((1+\tau_1^{-1}) + (1+\tau_1)(1-\omega)(1+\tau_2^{-1})\)\).$$
Here, $\tau_1,\tau_2,\alpha_5>0$ are arbitrary numbers, $R_1=(1+\alpha_1)(1-\gamma \delta)^2, R_2=(1+\alpha_1^{-1}) \gamma^2 \lambda^2 $, $\alpha_1>0$, $\delta$ is the spectral gap, $H$ is the synchronization gap, $\gamma$ is the consensus step-size, and $\lambda := \verts{\mathbf{W}-\mathbf{I}}_2$ where $\mathbf{W}$ is a doubly stochastic mixing matrix. 
\end{lemma}
%\begin{proof}
%We show the following bound in Lemma~\ref{supp_lemma_consensus_part1} (provided in Appendix~\ref{app:useful-lemmas}):
%\begin{align}
%\bbE\verts{\bX^{((m+1)H)} - \blX^{((m+1)H)}}_F^2 &\leq \vartheta_1 \bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 +  \vartheta_2\bbE\verts{\bX^{(mH)} - \bhX^{((m+1)H)}}_F^2 \notag \\
%&\quad + \vartheta_3\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1}\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2, \label{lem_cvx_e1_relaxed-interim1}
%\end{align}
%where $\vartheta_1=(1+\alpha_5^{-1})R_1$, $\vartheta_2=(1+\alpha_5^{-1}) R_2$, and $\vartheta_3=(R_1+R_2)(1+\alpha_5)$.
%
%We want to write the second expectation term $\bbE\verts{\bX^{(mH)} - \bhX^{((m+1)H)}}_F^2$ on the RHS of \eqref{lem_cvx_e1_relaxed-interim1} in terms of $\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2$. 
%%
%For that, first we define 
%\begin{align}\label{eq:sum_momentum-updates}
%\bX^{((m+1/2)H)} := \bX^{(mH)} - \eta\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\).
%\end{align} 
%%
%\begin{align}
%&\bbE\verts{\bX^{(mH)} - \bhX^{((m+1)H)}}_F^2 = \bbE\verts{\bX^{(mH)} - \(\bhX^{(mH)} + \C\(\bX^{((m+1/2)H)} - \bhX^{(mH)}\)\)}_F^2 \notag \\
%&\quad= \bbE\verts{\bX^{((m+1/2)H)} - \bhX^{(mH)} - \C\(\bX^{((m+1/2)H)} - \bhX^{(mH)}\) + \bX^{(mH)} - \bX^{((m+1/2)H)}}_F^2 \notag \\
%&\quad\leq (1+\tau_1)(1-\omega)\bbE\verts{\bX^{((m+1/2)H)} - \bhX^{(mH)}}_F^2 + (1+\tau_1^{-1})\bbE\verts{\bX^{(mH)} - \bX^{((m+1/2)H)}}_F^2 \notag \\
%&\quad= (1+\tau_1)(1-\omega)\bbE\verts{\bX^{((m+1/2)H)} - \bX^{(mH)} + \bX^{(mH)}- \bhX^{(mH)}}_F^2 \notag \\
%&\hspace{3cm}+ (1+\tau_1^{-1})\bbE\verts{\bX^{(mH)} - \bX^{((m+1/2)H)}}_F^2 \notag \\
%&\quad\leq (1+\tau_1)(1-\omega)(1+\tau_2)\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
%&\hspace{3cm} + \((1+\tau_1^{-1}) + (1+\tau_1)(1-\omega)(1+\tau_2^{-1})\)\bbE\verts{\bX^{(mH)} - \bX^{((m+1/2)H)}}_F^2 \notag \\
%&\quad\leq \chi_1\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 + \chi_2\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2, \label{lem_cvx_e1_relaxed-interim3}
%\end{align}
%where $\chi_1=(1+\tau_1)(1-\omega)(1+\tau_2)$ and $\chi_2=\((1+\tau_1^{-1}) + (1+\tau_1)(1-\omega)(1+\tau_2^{-1})\)$. 
%
%Substituting this back in \eqref{lem_cvx_e1_relaxed-interim1} yields \eqref{eq:cvx_e1_relaxed}, which proves Lemma~\ref{lem:cvx_e1_relaxed}.
%\end{proof}
%
\begin{lemma}\label{lem:cvx_e2_relaxed}
Under the setting of Theorem \ref{convergence_relaxed_assump}, for any $m\in\bbN$, we have 
\begin{align}\label{eq:cvx_e2_relaxed}
\bbE\verts{\bX^{((m+1)H)} - \bhX^{((m+1)H)}}_F^2 &\leq b_1\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + b_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
&\quad + b_3\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2,
\end{align}
where $b_1 = (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6)$,
$b_2 = (1+\tau_3)(1-\omega)(1+\tau_4) + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6^{-1})(1+\tau_7)(1-\omega)(1+\tau_8)$,
$b_3 = (1+\tau_3)(1-\omega)(1+\tau_4^{-1}) + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6^{-1})\((1+\tau_7^{-1}) + (1+\tau_7)(1-\omega)(1+\tau_8^{-1})\) + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5^{-1})$. Here, $\tau_3,\tau_4,\tau_5,\tau_6,\tau_7,\tau_8>0$ are free parameters.
\end{lemma}
%\begin{proof}
%\begin{align}
%&\bbE\verts{\bX^{((m+1)H)} - \bhX^{((m+1)H)}}_F^2 = \bbE\verts{\bX^{((m+1)H)} - \(\bhX^{(mH)} + \C\(\bX^{((m+1/2)H)} - \bhX^{(mH)}\)\)}_F^2 \notag \\
%&\qquad= \bbE\verts{\bX^{((m+1/2)H)} - \bhX^{(mH)} - \C\(\bX^{((m+1/2)H)} - \bhX^{(mH)}\) + \bX^{((m+1)H)} - \bX^{((m+1/2)H)}}_F^2 \notag \\
%&\qquad\leq (1+\tau_3)(1-\omega)\underbrace{\bbE\verts{\bX^{((m+1/2)H)} - \bhX^{(mH)}}_F^2}_{=:\ T_1} + (1+\tau_3^{-1})\underbrace{\bbE\verts{\bX^{((m+1)H)} - \bX^{((m+1/2)H)}}_F^2}_{=:\ T_2} \label{cvx_e2_relaxed-interim2}
%\end{align}
%Now we bound $T_1$ and $T_2$.
%\begin{align}
%T_1 &= \bbE\verts{\bX^{((m+1/2)H)} - \bhX^{(mH)}}_F^2 \notag \\
%&= \bbE\verts{\bX^{(mH)} - \eta\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\) - \bhX^{(mH)}}_F^2 \notag \\
%&\leq (1+\tau_4)\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 + (1+\tau_4^{-1})\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \label{cvx_e2_relaxed-interim3}
%\end{align}
%\begin{align}
%T_2 &= \bbE\verts{\bX^{((m+1)H)} - \bX^{((m+1/2)H)}}_F^2 \notag \\
%&= \bbE\verts{\bX^{((m+1/2)H)} + \gamma\bhX^{((m+1)H)}(\bW-\bI) - \bX^{((m+1/2)H)}}_F^2 \notag \\
%&= \gamma^2\bbE\verts{\bhX^{((m+1)H)}(\bW-\bI)}_F^2 \notag \\
%&= \gamma^2\bbE\verts{\(\bhX^{((m+1)H)} - \blX^{((m+1/2)H)}\)(\bW-\bI)}_F^2 \tag{Since $\blX^{((m+1/2)H)}(\bW-\bI)={\bf 0}$} \\
%&\leq \gamma^2\lambda^2\bbE\verts{\bhX^{((m+1)H)} - \blX^{((m+1/2)H)}}_F^2 \tag{Since $\|\bW-\bI\|_2=\lambda$} \\
%&= \gamma^2\lambda^2\bbE\verts{\bhX^{((m+1)H)} - \(\blX^{(mH)} - \eta\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)\)}_F^2 \notag \\
%&\leq \phi_1\underbrace{\bbE\verts{\bhX^{((m+1)H)} - \blX^{(mH)}}_F^2}_{=:\ T_3} + \phi_2\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2, \label{cvx_e2_relaxed-interim4}
%\end{align}
%where $\phi_1=\gamma^2\lambda^2(1+\tau_5)$ and $\phi_2=\gamma^2\lambda^2(1+\tau_5^{-1})$.
%\begin{align}
%T_3 &= \bbE\verts{\bhX^{((m+1)H)} - \blX^{(mH)}}_F^2 \notag \\
%&= \bbE\verts{\bhX^{((m+1)H)} - \bX^{(mH)} + \bX^{(mH)} - \blX^{(mH)}}_F^2 \notag \\
%&\leq (1+\tau_6)\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + (1+\tau_6^{-1})\bbE\verts{\bhX^{((m+1)H)} - \bX^{(mH)}}_F^2 \notag \\
%&\stackrel{\text{(a)}}{\leq} (1+\tau_6)\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + (1+\tau_6^{-1})(1+\tau_7)(1-\omega)(1+\tau_8)\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
%&\hspace{1cm} + \phi\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2, \label{lem_cvx_e1_relaxed-interim5}
%\end{align}
%where $\phi_3=(1+\tau_6^{-1})\((1+\tau_7^{-1}) + (1+\tau_7)(1-\omega)(1+\tau_8^{-1})\)$, (a) follows from \eqref{lem_cvx_e1_relaxed-interim3} for bounding $\bbE\verts{\bhX^{((m+1)H)} - \bX^{(mH)}}_F^2$. Observe that since we are bounding this quantity separately for (a), we can use different coefficients here. In the above bound on $\bbE\verts{\bhX^{((m+1)H)} - \bX^{(mH)}}_F^2$ from \eqref{lem_cvx_e1_relaxed-interim3}, instead of using the same $\tau_1,\tau_2$, we used $\tau_7,\tau_8$, respectively.
%
%Substituting the above bound on $T_3$ into \eqref{cvx_e2_relaxed-interim4} and the substituting the resulting bound on $T_2$ from \eqref{cvx_e2_relaxed-interim4} and on $T_1$ from \eqref{cvx_e2_relaxed-interim3} into \eqref{cvx_e2_relaxed-interim2} gives
%%\begin{align}
%%&\bbE\verts{\bX^{((m+1)H)} - \bhX^{((m+1)H)}}_F^2 \leq (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6)\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 \notag \\
%%& + (1+\tau_3)(1-\omega)(1+\tau_4)\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
%%& + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6^{-1})(1+\tau_1)(1-\omega)(1+\tau_2)\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
%%&\qquad + (1+\tau_3)(1-\omega)(1+\tau_4^{-1})\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \notag \\
%%& + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6^{-1})\((1+\tau_1^{-1}) + (1+\tau_1)(1-\omega)(1+\tau_2^{-1})\)\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2  \notag \\
%%&\qquad + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5^{-1})\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2,
%%\end{align}
%\begin{align}
%\bbE\verts{\bX^{((m+1)H)} - \bhX^{((m+1)H)}}_F^2 &\leq b_1\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + b_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
%&\quad + b_3\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2,
%\end{align}
%where $b_1 = (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6)$,
%$b_2 = (1+\tau_3)(1-\omega)(1+\tau_4) + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6^{-1})(1+\tau_7)(1-\omega)(1+\tau_8)$,
%$b_3 = (1+\tau_3)(1-\omega)(1+\tau_4^{-1}) + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5)(1+\tau_6^{-1})\((1+\tau_7^{-1}) + (1+\tau_7)(1-\omega)(1+\tau_8^{-1})\) + (1+\tau_3^{-1})\gamma^2\lambda^2(1+\tau_5^{-1})$.
%\end{proof}
%

%
%\begin{proposition}\label{prop:sum_momentum-updates}
%For any $m\in\bbN$, we have
%\begin{align}\label{eq:sum_momentum-updates}
%\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 &\leq \frac{2 H\beta^2}{1-\beta}\sum_{t'=mH}^{(m+1)H-1}\Lambda^{(t')}  + 2 H \sum_{t'=mH}^{(m+1)H-1} \bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2. 
%\end{align}
%\end{proposition}
%\begin{proof}
%\begin{align}
%\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 &\leq H \sum_{t'=mH}^{(m+1)H-1} \bbE\verts{\beta V^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2 \notag \\
%&\hspace{-3cm}\leq 2H\beta^2 \sum_{t'=mH}^{(m+1)H-1} \bbE\verts{\bV^{(t')}}_F^2 + 2 H \sum_{t'=mH}^{(m+1)H-1} \bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2 \notag \\
%%&\hspace{-3cm}\leq 2\eta^2 H\beta^2 \sum_{t'=mH}^{(m+1)H-1} \bbE\verts{\sum_{k=0}^{t'} \beta^{t'-k}\nabla \bF(\bX^{(k)}, \bxi^{(k)})}_F^2 + 2\eta^2 H \sum_{t'=mH}^{(m+1)H-1} \bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2 \notag \\
%&\hspace{-3cm}\leq \frac{2 H\beta^2}{1-\beta}\sum_{t'=mH}^{(m+1)H-1}\Lambda^{(t')}  + 2 H \sum_{t'=mH}^{(m+1)H-1} \bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2. 
%\end{align}
%\end{proof}



\subsection{Proof of Lemma~\ref{lem:similar-eq16}}\label{subsec:proof-similar-eq16}
For $t\in[T]$, define $m\in\lfloor\frac{t}{H}\rfloor-1$. This implies that $(m+1)H\leq t < (m+2)H$.
\begin{align}
&\Xi^{(t)} := \bbE\verts{\bX^{(t)} - \blX^{(t)}}_F^2 = \bbE\verts{\bX^{(t)} - \blX^{((m+1)H)} - \(\blX^{(t)} - \blX^{((m+1)H)}\)}_F^2 \notag \\
&\stackrel{\text{(a)}}{\leq} \bbE\verts{\bX^{(t)} - \blX^{((m+1)H)}}_F^2 \label{equi16-interim0} \\
&= \bbE\verts{\bX^{((m+1)H)} - \eta\sum_{t'=(m+1)H}^{t-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\) - \blX^{((m+1)H)}}_F^2 \notag \\
&\leq (1+\nu_1)\bbE\verts{\bX^{((m+1)H)} - \blX^{((m+1)H)}}_F^2 + (1+\nu_1^{-1})\eta^2\bbE\verts{\sum_{t'=(m+1)H}^{t-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \notag \\
&\stackrel{\text{(b)}}{\leq} (1+\nu_1)a_1 \bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + (1+\nu_1)a_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
&\hspace{2cm} + (1+\nu_1)a_3\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1}\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2 \notag \\
&\hspace{4cm} + (1+\nu_1^{-1})\eta^2\bbE\verts{\sum_{t'=(m+1)H}^{t-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \notag \\
&\leq (1+\nu_1)a_1 \bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + (1+\nu_1)a_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
&\quad + \((1+\nu_1)a_3 + (1+\nu_1^{-1})\)\eta^2H\sum_{t'=mH}^{t-1}\bbE\verts{\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2 \notag \\
&\leq (1+\nu_1)a_1 \Xi^{(mH)} + (1+\nu_1)a_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
&\quad + \((1+\nu_1)a_3 + (1+\nu_1^{-1})\)\eta^2H\sum_{t'=mH}^{t-1}2\(\beta^2\bbE\verts{\bV^{(t')}}_F^2 + \bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2\). \label{equi-16-interim1}
\end{align}
Here, (a) follows from the inequality: $\frac{1}{n}\sum_{i=1}^n\verts{\ba_i-\frac{1}{n}\sum_{i=1}^n\ba_i}_2^2 \leq \frac{1}{n}\sum_{i=1}^n\verts{\ba_i}_2^2$ and (b) follows from \eqref{eq:cvx_e1_relaxed} (in Lemma~\ref{lem:cvx_e1_relaxed}). The coefficients $a_1,a_2,a_3$ in the RHS of (b) are defined in Lemma~\ref{lem:cvx_e1_relaxed}.
%
\begin{proposition}\label{prop:mom-update-norm}
For any $t'$, we have
\begin{align}\label{eq:mom-update-norm}
\bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2 &\leq 2(M^2+1)\(L^2\Xi^{(t')} + nG^2+nB^2\bbE\verts{\nabla f(\blx^{(t')})}_2^2\) + n\sigma^2.
\end{align}
\end{proposition}
%
Substituting from \eqref{eq:mom-update-norm} into \eqref{equi-16-interim1}, we get for $(m+1)H\leq t < (m+2)H$:
\begin{align}
&\Xi^{(t)} \leq (1+\nu_1)\(a_1 \Xi^{(mH)} + a_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2\)  + 2c_2\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\)\notag \\
&\hspace{2cm} + c_2\eta^2H\beta^2\sum_{t'=mH}^{t-1}\bbE\verts{\bV^{(t')}}_F^2 + 2c_2\eta^2H(M^2+1)L^2\sum_{t'=mH}^{t-1}\Xi^{(t')} \notag \\
&\hspace{4cm} + 2c_2\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{t-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2, \label{equi-16-interim2}
\end{align}
where %$c_1=\max\{(1+\nu_1)a_1,(1+\nu_1)a_2\}$ and 
$c_2=2\((1+\nu_1)a_3 + (1+\nu_1^{-1})\)$.

For any $j\in[T]$ and $m'=\lfloor\frac{j}{H}\rfloor - 1$, define 
\begin{align}\label{Sj-defn}
S^{(j)} := \Xi^{(j)} + \bbE\verts{\bX^{(j)} - \bhX^{((m'+1)H)}}_F^2.
\end{align}
By definition, we have $S^{(mH)} = \Xi^{(mH)} + \bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2$ and also that $\Xi^{(t')}\leq S^{(t')}$ for any $t'$. Using these in \eqref{equi-16-interim2}, we get
\begin{align}
&\Xi^{(t)} \leq (1+\nu_1)\(a_1 \Xi^{(mH)} + a_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2\) \notag \\
&\quad + 2c_2\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + c_2\eta^2H\beta^2\sum_{t'=mH}^{t-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\hspace{1cm} + 2c_2\eta^2H(M^2+1)L^2\sum_{t'=mH}^{t-1}S^{(t')} + 2c_2\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{t-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2, \label{equi-16-interim3}
\end{align}
Our aim is to get an upper-bound on $S^{(t)}$, which is defined in \eqref{Sj-defn} as $S^{(t)} = \Xi^{(t)} + \bbE\verts{\bX^{(t)} - \bhX^{(\lfloor t/H\rfloor H)}}_F^2$. However, in \eqref{equi-16-interim3}, we have only derived  an upper-bound on $\Xi^{(t)}$ in terms of $S^{(t')}$ for $t'<t$. So,, we need to derive a similar upper-bound on the other term $\bbE\verts{\bX^{(t)} - \bhX^{(\lfloor t/H\rfloor H)}}_F^2$, and then we will add both the upper-bounds to get an upper-bound on $S^{(t)}$. In the following, we derive an upper bound on $\bbE\verts{\bX^{(t)} - \bhX^{(\lfloor t/H\rfloor H)}}_F^2$. 

Let $m=\lfloor\frac{t}{H}\rfloor - 1$.
\begin{align}
&\bbE\verts{\bX^{(t)} - \bhX^{((m+1)H)}}_F^2 = \bbE\verts{\bX^{((m+1)H)} - \eta\sum_{t'=(m+1)H}^{t-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\) - \bhX^{((m+1)H)}}_F^2 \notag \\
&\leq (1+\nu_1)\bbE\verts{\bX^{((m+1)H)} - \bhX^{((m+1)H)}}_F^2 + (1+\nu_1^{-1})\eta^2\bbE\verts{\sum_{t'=(m+1)H}^{t-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \notag \\
&\stackrel{\text{(a)}}{\leq} (1+\nu_1)b_1\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + (1+\nu_1)b_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
&\hspace{1cm} + (1+\nu_1)b_3\eta^2\bbE\verts{\sum_{t'=mH}^{(m+1)H-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \notag \\
&\hspace{2cm} + (1+\nu_1^{-1})\eta^2\bbE\verts{\sum_{t'=(m+1)H}^{t-1} \(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \notag \\
&\leq (1+\nu_1)b_1\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + (1+\nu_1)b_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 \notag \\
&\hspace{1cm} + \((1+\nu_1)b_3 + (1+\nu_1^{-1})\)\eta^2H\sum_{t'=mH}^{t-1} \bbE\verts{\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2 \notag \\
&\leq (1+\nu_1)\(b_1\Xi^{(mH)} + b_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2\) \notag \\
&\hspace{1cm} + \((1+\nu_1)b_3 + (1+\nu_1^{-1})\)\eta^2H\sum_{t'=mH}^{t-1}2\(\beta^2\bbE\verts{\bV^{(t')}}_F^2 + \bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2\) \notag \\
&\stackrel{\text{(b)}}{\leq} (1+\nu_1)\(b_1\Xi^{(mH)} + b_2\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2\) \notag \\
&\quad + 2c_4\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + c_4\eta^2H\beta^2\sum_{t'=mH}^{t-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\hspace{1cm} + 2c_4\eta^2H(M^2+1)L^2\sum_{t'=mH}^{t-1}\Xi^{(t')} + 2c_4\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{t-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2, \label{equi-16-interim4}
\end{align}
where (a) follows from \eqref{eq:cvx_e2_relaxed} in Lemma~\ref{lem:cvx_e2_relaxed} and the coefficients $b_1,b_2,b_3$ in the RHS of (a) are defined in Lemma~\ref{lem:cvx_e2_relaxed}, and (b) follows from substituting the bound from \eqref{eq:mom-update-norm} (in Proposition~\ref{prop:mom-update-norm}). In the RHS of (b), %$c_3=\max\{(1+\nu_1)b_1,(1+\nu_1)b_2\}$ and 
$c_4=2\((1+\nu_1)b_3 + (1+\nu_1^{-1})\)$.

Adding \eqref{equi-16-interim3} and \eqref{equi-16-interim4} and substituting $S^{(t)}=\Xi^{(t)}+\bbE\verts{\bX^{(t)} - \bhX^{((m+1)H)}}_F^2$, we get
\begin{align}
S^{(t)} &\leq (1+\nu_1)\max\{a_1+b_1,a_2+b_2\}S^{(mH)} + 2c_1\eta^2H^2\varGamma + c_1\eta^2H\beta^2\sum_{t'=mH}^{t-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\quad + 2c_1\eta^2H(M^2+1)L^2\sum_{t'=mH}^{t-1}S^{(t')} + 2c_1\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{t-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2, \label{equi-16-interim5}
\end{align}
where $\varGamma=n\(2(M^2+1)G^2 + \sigma^2\)$ and $c_1=c_2+c_4$ with %$c_1=\max\{(1+\nu_1)a_1,(1+\nu_1)a_2\}$, 
$c_2=2\((1+\nu_1)a_3 + (1+\nu_1^{-1})\)$ %, $c_3=\max\{(1+\nu_1)b_1,(1+\nu_1)b_2\}$ 
and $c_4=2\((1+\nu_1)b_3 + (1+\nu_1^{-1})\)$. Here, $\nu_1>0$ is a free coefficient, and $a_1,a_2,a_3$ and $b_1,b_2,b_3$ are defined in Lemma~\ref{lem:cvx_e1_relaxed} and Lemma~\ref{lem:cvx_e2_relaxed}, respectively. We will set the free variables such that the coefficients of $S^{(t')}$ for any $t'=mH,...,t-1$ on the RHS become strictly less than one.

In Appendix~\ref{app:setting-params}, we show that if we set the free parameters to be the following:
\begin{align*}
&\tau_i = \frac{\omega}{4}, \text{ for } i=1,2,3,4,5,7,8; \quad \tau_6 = \frac{4}{\omega};  \quad \nu_1=\frac{\gamma^*\delta}{4}; \\
&\alpha_1 = \frac{\gamma\delta}{2}; \quad \alpha_5^{-1} = \frac{\gamma\delta}{2}; \quad \gamma = \frac{2\delta\omega^3}{(128\lambda^2 + 24\lambda^2\omega^2 + 4\delta^2\omega^2)};
\end{align*}
Then we get 
\begin{align}
(1+\nu_1)\max\{a_1+b_1,a_2+b_2\} \leq 1-\frac{\gamma^*\delta}{4} \leq 1- \frac{\delta^2\omega^3}{1224}, \label{final-bound_coeff_St} \\
c_1 \leq 2(1+\frac{\gamma\delta}{4})\(\frac{3}{\gamma\delta} + \frac{9\lambda^2}{\delta^2} + \frac{45\gamma\lambda^2}{\delta\omega} + \frac{104\gamma^2\lambda^2}{\omega^2} + \frac{4}{\omega} - 2\) + 4(1+\frac{4}{\gamma\delta}). \label{final-bound-c2+c4}
\end{align}
%
Putting these bounds back into \eqref{equi-16-interim5}, we get the following upper bound for $(m+1)H\leq t \leq (m+2)H-1$:
\begin{align}
S^{(t)} &\leq \(1-\frac{\gamma\delta}{4}\)S^{(mH)} + 2c_1\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + c_1\eta^2H\beta^2\sum_{t'=mH}^{t-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\quad + 2c_1\eta^2H(M^2+1)L^2\sum_{t'=mH}^{t-1}S^{(t')} + 2c_1\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{t-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2. \label{equi-16-final-bound}
\end{align} 




\subsection{Proof of Lemma~\ref{lem:similar-eq17}}\label{subsec:proof-similar-eq17}
For any fixed $t\in[T]$ and the corresponding $m\in\lfloor\frac{t}{H}\rfloor-1$, in Section~\ref{subsec:proof-similar-eq16}, we derived an upper-bound on $S^{(\hatt)}$ all $\hatt\in[T]$ such that $(m+1)H\leq \hatt < (m+2)H$ (note that $t$ and $\hatt$ will give exactly the same terms in Section~\ref{subsec:proof-similar-eq16}, so we just kept $t$ everywhere). In this section, we consider the case when $mH\leq \hatt < (m+1)H$.
%
\begin{align}
\Xi^{(\hatt)} &\leq \bbE\verts{\bX^{(\hatt)}-\blX^{(\hatt)}}_F^2 = \bbE\verts{\bX^{(\hatt)} - \blX^{(mH)} - \(\blX^{(\hatt)} - \blX^{(mH)}\)}_F^2 \notag \\
&\stackrel{\text{(a)}}{\leq} \bbE\verts{\bX^{(\hatt)} - \blX^{(mH)}}_F^2 \label{equi-17-interim0} \\
&= \bbE\verts{\bX^{(mH)} - \eta\sum_{t'=mH}^{\hatt-1} \(\beta \bV^{(\hatt)}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\) - \blX^{(mH)}}_F^2 \notag \\
&\leq (1+\nu_3)\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2 + (1+\nu_3^{-1})\eta^2\bbE\verts{\sum_{t'=mH}^{\hatt-1}\(\beta \bV^{(t')}+\nabla \bF(\bX^{(t')},\bxi^{(t')})\)}_F^2 \notag \\
&\stackrel{\text{(b)}}{\leq} (1+\nu_3)\Xi^{(mH)} + 2(1+\nu_3^{-1})\eta^2H\(\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 + \sum_{t'=mH}^{\hatt-1}\bbE\verts{\nabla \bF(\bX^{(t')},\bxi^{(t')})}_F^2\) \notag \\
&\stackrel{\text{(c)}}{\leq} (1+\nu_3)\Xi^{(mH)} + 2(1+\nu_3^{-1})\eta^2H\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\quad + 2(1+\nu_3^{-1})\eta^2H\sum_{t'=mH}^{\hatt-1}\(2(M^2+1)\(L^2\Xi^{(t')} + nG^2+nB^2\bbE\verts{\nabla f(\blx^{(t')})}_2^2\) + n\sigma^2\) \notag \\
&\leq (1+\nu_3)\Xi^{(mH)} + 2(1+\nu_3^{-1})\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + 2(1+\nu_3^{-1})\eta^2H\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\quad + 4(1+\nu_3^{-1})\eta^2H(M^2+1)L^2\sum_{t'=mH}^{\hatt-1}\Xi^{(t')} + 4(1+\nu_3^{-1})\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2 \label{equi-17-interim1}
\end{align}
where (a) follows from the same reasoning using which we obtained \eqref{equi16-interim0}, (b) uses $\Xi^{(mH)}=\bbE\verts{\bX^{(mH)} - \blX^{(mH)}}_F^2$, and (c) follows from \eqref{eq:mom-update-norm} (in Proposition~\ref{prop:mom-update-norm}).

As mentioned in Section~\ref{subsec:proof-similar-eq16}, our aim is to get an upper-bound on $S^{(\hatt)}$, which is defined in \eqref{Sj-defn} as $S^{(\hatt)} = \Xi^{(\hatt)} + \bbE\verts{\bX^{(\hatt)} - \bhX^{(\lfloor \hatt/H\rfloor H)}}_F^2$. However, in \eqref{equi-17-interim1}, we have only derived an upper-bound on $\Xi^{(\hatt)}$. So, we need to derive a similar upper-bound on the other term $\bbE\verts{\bX^{(\hatt)} - \bhX^{(\lfloor \hatt/H\rfloor H)}}_F^2$, and then we will add both the upper-bounds to get an upper-bound on $S^{(\hatt)}$. 

Note that since $mH\leq \hatt < (m+1)H$, we have that $\lfloor\frac{\hatt}{H}\rfloor = m$. In order to upper-bound $\bbE\verts{\bX^{(\hatt)} - \bhX^{(mH)}}_F^2$, we can follow the same steps that we used for going from \eqref{equi-17-interim0} to \eqref{equi-17-interim1} (just replace $\blX^{(mH)}$ with $\bhX^{(mH)}$). This would give the following bound:
\begin{align}
&\bbE\verts{\bX^{(\hatt)} - \bhX^{(mH)}}_F^2 \leq (1+\nu_3)\bbE\verts{\bX^{(mH)} - \bhX^{(mH)}}_F^2 + 2(1+\nu_3^{-1})\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) \notag \\
&\quad + 2(1+\nu_3^{-1})\eta^2H\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 + 4(1+\nu_3^{-1})\eta^2H(M^2+1)L^2\sum_{t'=mH}^{\hatt-1}\Xi^{(t')} \notag \\
&\qquad + 4(1+\nu_3^{-1})\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2. \label{equi-17-interim2}
\end{align}
Adding \eqref{equi-17-interim1} and \eqref{equi-17-interim2}, and using the definition that $S^{(\hatt)} = \Xi^{(\hatt)} + \bbE\verts{\bX^{(\hatt)} - \bhX^{(\lfloor \hatt/H\rfloor H)}}_F^2$ together with that $\Xi^{(t')}\leq S^{(t')}$, and taking $\nu_3=\frac{\gamma\delta}{4}$, we get
\begin{align}
S^{(\hatt)} &\leq (1+\frac{\gamma\delta}{4})S^{(mH)} + 4(1+\frac{4}{\gamma\delta})\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) \notag \\
&\quad + 4(1+\frac{4}{\gamma\delta})\eta^2H\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 + 8(1+\frac{4}{\gamma\delta})\eta^2H(M^2+1)L^2\sum_{t'=mH}^{\hatt-1}S^{(t')} \notag \\
&\qquad + 8(1+\frac{4}{\gamma\delta})\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2. \label{equi-17-interim3}
\end{align}
In order to make our calculations less cluttered later, we would like to write all terms (except the first one) in the RHS above in the same form as given in \eqref{equi-16-final-bound}. Indeed, it can be verified easily that $4(1+\frac{4}{\gamma\delta})\leq c_1$, where $c_1$ is exactly the same as in \eqref{equi-16-final-bound}. Substituting this in \eqref{equi-17-interim3} above yields the bound below for $mH\leq \hatt < (m+1)H$, where $m\in\lfloor\frac{t}{H}\rfloor-1$:
\begin{align}
S^{(\hatt)} &\leq \(1+\frac{\gamma\delta}{4}\)S^{(mH)} + 2c_1\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + c_1\eta^2H\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
&\quad + 2c_1\eta^2H(M^2+1)L^2\sum_{t'=mH}^{\hatt-1}S^{(t')} + 2c_1\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2, \label{equi-17-interim4}
\end{align} 
where $c_1$ is exactly the same as in \eqref{equi-16-final-bound}.



\subsection{Proof of Lemma~\ref{lem:similar-lem14}}\label{subsec:proof-similar-lem14}
Let $A=2c_1H^2n\(2(M^2+1)G^2 + \sigma^2\)$, $C=2c_1H(M^2+1)nB^2$, $D=\frac{c_1H\beta^2}{(1-\beta)}$, and $\Lambda^{(t')}=(1-\beta)\bbE\verts{\bV^{(t)}}_F^2$, where $c_1$ is the same as in \eqref{equi-16-final-bound}.
Since $\eta\leq\sqrt{\frac{\gamma\delta}{512c_1H^2(M^2+1)L^2}}$, we have $2c_1\eta^2H(M^2+1)L^2\leq \frac{\gamma\delta}{4}\frac{1}{64H}$.


Take any $t\in[T]$. Let $m=\lfloor\frac{t}{H}\rfloor-1$. 

With these substitutions and letting $\alpha=\frac{\gamma\delta}{4}$, the bound from \eqref{equi-16-final-bound} for any $t$ such that $(m+1)H\leq t\leq(m+2)H-1$ becomes:
	\begin{align}\label{bound1-on-St}
		S^{(t)} \leq \left(1 - \frac{\alpha}{2} \right) S^{(mH)} + A \eta^2 + \frac{\alpha}{64H} \sum_{t' = mH}^{t-1} S^{(t')} + C \eta^2 \sum_{t' = mH}^{t-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + D \eta^2 \sum_{t' = mH}^{t-1} \Lambda^{(t')}.
	\end{align}
	%
	And for any $\hatt$ such that $mH \leq \hatt < (m+1)H$, the bound from \eqref{equi-17-interim4} becomes:
	\begin{align}\label{bound2-on-St}
		S^{(\hatt)} \leq \left(1 - \frac{\alpha}{2} \right) S^{(mH)} + A \eta^2 + \frac{\alpha}{64H} \sum_{t' = mH}^{\hatt-1} S^{(t')} + C \eta^2 \sum_{t' = mH}^{\hatt-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + D \eta^2 \sum_{t' = mH}^{\hatt-1} \Lambda^{(t')}.
	\end{align}	
%With these substitutions and letting $\alpha=\frac{\gamma\delta}{4}$, the bound from \eqref{equi-16-final-bound} and \eqref{equi-17-interim4} are as follows:
%\begin{align}
%\end{align}
%
%The bound from \eqref{equi-16-final-bound} is the following:
%\begin{align*}
%S^{(t)} &\leq \(1-\frac{\gamma\delta}{4}\)S^{(mH)} + 2c_1\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) + c_1\eta^2H\beta^2\sum_{t'=mH}^{t-1}\bbE\verts{\bV^{(t')}}_F^2 \notag \\
%&\quad + 2c_1\eta^2H(M^2+1)L^2\sum_{t'=mH}^{t-1}S^{(t')} + 2c_1\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{t-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2,
%\end{align*} 
%where $c_1=c_2+c_4$ and the bound on $c_2+c_4$ is given in \eqref{final-bound-c2+c4}, and $\gamma=\gamma^*$ is defined in \eqref{params-setting-alphas-gamma}.
%
%The bound from \eqref{equi-17-interim4} is the following:
%\begin{align*}
%S^{(\hatt)} &\leq (1+\frac{\gamma\delta}{4})S^{(mH)} + 4(1+\frac{4}{\gamma\delta})\eta^2H^2n\(2(M^2+1)G^2 + \sigma^2\) \notag \\
%&\quad + 4(1+\frac{4}{\gamma\delta})\eta^2H\beta^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\bV^{(t')}}_F^2 + 8(1+\frac{4}{\gamma\delta})\eta^2H(M^2+1)L^2\sum_{t'=mH}^{\hatt-1}S^{(t')} \notag \\
%&\qquad + 8(1+\frac{4}{\gamma\delta})\eta^2H(M^2+1)nB^2\sum_{t'=mH}^{\hatt-1}\bbE\verts{\nabla f(\blx^{(t')})}_2^2. 
%\end{align*}
%
%Note that the equation below is different from the one above. The eq above has a better upper bound (but how?) -- the coefficient of $S^{(t')}$ has $\eta^2$ in the above bound, but not in the bound below. Check it out.}
%
%From eq ??, we note that for $(m+1)H \leq t < (m+2)H$, for $\eta \leq ??$ we have:	
%	\begin{align*}
%		S^{(t)} \leq \left(1 - \frac{\alpha}{2} \right) S^{(mH)} + A \eta^2 + \frac{\alpha}{64H} \sum_{t' = mH}^{t-1} S^{(t')} + C \eta^2 \sum_{t' = mH}^{t-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + D \eta^2 \sum_{t' = mH}^{t-1} \Lambda^{(t')}
%	\end{align*}
%	where $\alpha = ??$. 
	Consider \eqref{bound1-on-St}. Substituting the value of $S^{(t-1)}$ recursively in the RHS of \eqref{bound1-on-St}, we get:
	\begin{align*}
		&S^{(t)} \leq \left(1 - \frac{\alpha}{2} \right) S^{(mH)} + A \eta^2 + \frac{\alpha}{64H} \sum_{t' = mH}^{t-2} S^{(t')} + C \eta^2 \sum_{t' = mH}^{t-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + D \eta^2 \sum_{t' = mH}^{t-1} \Lambda^{(t')} \\
		& \ + \frac{\alpha}{64H} \left(  \left(1 - \frac{\alpha}{2} \right) S^{(mH)} + A \eta^2 + \frac{\alpha}{64H} \sum_{t' = mH}^{t-2} S^{(t')} + C \eta^2 \sum_{t' = mH}^{t-2} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + D \eta^2 \sum_{t' = mH}^{t-2} \Lambda^{(t')}   \right) \\
		& = \left(1 - \frac{\alpha}{2} \right) \left( 1 + \frac{\alpha}{64H} \right) S^{(mH)} + A \left( 1 + \frac{\alpha}{64H} \right)  \eta^2 + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{64H} \right) \sum_{t' = mH}^{t-2} S^{(t')} \\
		& \qquad + \left( 1 + \frac{\alpha}{64H} \right) C\eta^2 \sum_{t' = mH}^{t-2} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{64H} \right) D \eta^2 \sum_{t' = mH}^{t-2 } \Lambda^{(t')} \\
		& \qquad + C\eta^2 \bbE \verts{ \nabla f (\blx^{(t-1)}) }^2 + D \eta^2 \Lambda_{t-1}
	\end{align*}
	Substituting the values in the RHS till $(m+1)H$, we get:
	\begin{align*}
		&S^{(t)} \leq \left(1 - \frac{\alpha}{2} \right) \left( 1 + \frac{\alpha}{64H} \right)^{H} S^{(mH)} + A \left( 1 + \frac{\alpha}{64H} \right)^H  \eta^2 + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{64H} \right)^H \sum_{t' = mH}^{(m+1)H-1} S^{(t')} \\
		& \quad + \left( 1 + \frac{\alpha}{64H} \right)^H C\eta^2 \sum_{t' = mH}^{(m+1)H-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{64H} \right)^H D \eta^2 \sum_{t' = mH}^{(m+1)H-1 } \Lambda^{(t')} \\
		& \quad + C\eta^2  \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \bbE \verts{ \nabla f (\blx^{(t')}) }^2  + D \eta^2 \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \Lambda^{(t')}
	\end{align*}
	Now consider $t'$ such that $mH \leq t' < (m+1)H$. Substituting the value of $S^{((m+1)H -1)}$ from \eqref{bound2-on-St} into the RHS above gives us: 
	\begin{align*}
		&S^{(t)}  \leq \left(1 - \frac{\alpha}{2} \right) \left( 1 + \frac{\alpha}{64H} \right)^{H} S^{(mH)} + A \left( 1 + \frac{\alpha}{64H} \right)^H  \eta^2 + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{64H} \right)^H \sum_{t' = mH}^{(m+1)H-2} S^{(t')} \\
		& \quad + \left( 1 + \frac{\alpha}{64H} \right)^H C\eta^2 \sum_{t' = mH}^{(m+1)H-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{64H} \right)^H D \eta^2 \sum_{t' = mH}^{(m+1)H-1 } \Lambda^{(t')} \\
		& \quad + C\eta^2  \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \bbE \verts{ \nabla f (\blx^{(t')}) }^2  + D \eta^2 \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \Lambda^{(t')} \\
		& \quad + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{64H} \right)^H \left[ (1+\frac{\alpha}{2}) S^{(mH)}  + A \eta^2 + \frac{\alpha}{64H} \sum_{j = mH}^{(m+1)H-2} S^{(j)}  \right. \\
		& \quad \qquad \left.	 + C\eta^2 \sum_{j = mH}^{(m+1)H-2}  \bbE \verts{\nabla f(\blx^{(j)})} + D \eta^2 \sum_{j=mH}^{(m+1)H-2} \Lambda^{(j)} \right] \\
		& \leq \left(\left(1 - \frac{\alpha}{2} \right) +  \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{2} \right) \right) \left( 1 + \frac{\alpha}{64H} \right)^{H} S^{(mH)}  \\
		& \quad + A \left( 1 + \frac{\alpha}{64H} \right)^{H+1}  \eta^2 + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{64H} \right)^{H+1} \sum_{t' = mH}^{(m+1)H-2} S^{(t')} \\
		& \quad + \left( 1 + \frac{\alpha}{64H} \right)^{H+1} C\eta^2 \sum_{t' = mH}^{(m+1)H-2} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{64H} \right)^{H+1} D \eta^2 \sum_{t' = mH}^{(m+1)H-2 } \Lambda^{(t')} \\
		& \quad + C\eta^2  \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \bbE \verts{ \nabla f (\blx^{(t')}) }^2  + D \eta^2 \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \Lambda^{(t')} \\
		& \quad + C\eta^2  \left( 1 + \frac{\alpha}{64H} \right)^{H} \bbE \verts{ \nabla f (\blx^{((m+1)H-1)}) }^2  + D \eta^2  \left( 1 + \frac{\alpha}{64H} \right)^{H} \Lambda^{((m+1)H-1)}		
	\end{align*} 
	Now we note that for $0 < \alpha \leq 1$, $  \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{2} \right)  \leq \left( 1 - \frac{\alpha}{2} \right) \frac{\alpha}{16H}$. Using this fact in the first term and $(1 + \frac{\alpha}{64H}) \leq (1+ \frac{\alpha}{16H})$ everywhere else, and also substituting $\left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \leq ( 1+ \frac{\alpha}{16H})^{H}$ for all $t' \in \{(m+1)H,\hdots,t-1\}$ in the RHS above gives:
%	\begin{align*}
%		S^{(t)} & \leq  \left(1 - \frac{\alpha}{2} \right)  \left( 1 + \frac{\alpha}{16H} \right)^{H+1} S^{(mH)}  \\
%		& \qquad + A \left( 1 + \frac{\alpha}{16H} \right)^{H+1}  \eta^2 + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{16H} \right)^{H+1} \sum_{t' = mH}^{(m+1)H-2} S^{(t')} \\
%		& \qquad + \left( 1 + \frac{\alpha}{16H} \right)^{H+1} C\eta^2 \sum_{t' = mH}^{(m+1)H-2} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{16H} \right)^{H+1} D \eta^2 \sum_{t' = mH}^{(m+1)H-2 } \Lambda^{(t')} \\
%		& \qquad + C\eta^2  \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{16H} \right)^{t-1-t'} \bbE \verts{ \nabla f (\blx^{(t')}) }^2  + D \eta^2 \sum_{t' = (m+1)H}^{t-1} \left( 1 + \frac{\alpha}{16H} \right)^{t-1-t'} \Lambda^{(t')} \\
%		& \qquad + C\eta^2  \left( 1 + \frac{\alpha}{16H} \right)^{H} \bbE \verts{ \nabla f (\blx^{((m+1)H-1)}) }^2  + D \eta^2  \left( 1 + \frac{\alpha}{16H} \right)^{H} \Lambda_{(m+1)H-1}		
%	\end{align*}
		\begin{align*}
		S^{(t)} & \leq  \left(1 - \frac{\alpha}{2} \right)  \left( 1 + \frac{\alpha}{16H} \right)^{H+1} S^{(mH)}  + A \left( 1 + \frac{\alpha}{16H} \right)^{H+1}  \eta^2 + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{16H} \right)^{H+1} \sum_{t' = mH}^{(m+1)H-2} S^{(t')} \\
		& \qquad + \left( 1 + \frac{\alpha}{16H} \right)^{H+1} C\eta^2 \sum_{t' = mH}^{(m+1)H-2} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{16H} \right)^{H+1} D \eta^2 \sum_{t' = mH}^{(m+1)H-2 } \Lambda^{(t')} \\
		& \qquad + C\eta^2  \left( 1 + \frac{\alpha}{16H} \right)^{H}\sum_{t' = (m+1)H}^{t-1}  \bbE \verts{ \nabla f (\blx^{(t')}) }^2  + D \eta^2\left( 1 + \frac{\alpha}{16H} \right)^{H} \sum_{t' = (m+1)H}^{t-1}  \Lambda^{(t')} \\
		& \qquad + C\eta^2  \left( 1 + \frac{\alpha}{16H} \right)^{H} \bbE \verts{ \nabla f (\blx^{((m+1)H-1)}) }^2  + D \eta^2  \left( 1 + \frac{\alpha}{16H} \right)^{H} \Lambda^{((m+1)H-1)}		
	\end{align*}
	Using $\left( 1 + \frac{\alpha}{16H} \right)^{H}\leq\left( 1 + \frac{\alpha}{16H} \right)^{H+1}$ in the last four terms and then clubbing together terms respectively with $C$ and $D$, we get
		\begin{align*}
		S^{(t)} & \leq  \left(1 - \frac{\alpha}{2} \right)  \left( 1 + \frac{\alpha}{16H} \right)^{H+1} S^{(mH)} + A \left( 1 + \frac{\alpha}{16H} \right)^{H+1}  \eta^2 + \frac{\alpha}{64H} \left( 1 + \frac{\alpha}{16H} \right)^{H+1} \sum_{t' = mH}^{(m+1)H-2} S^{(t')} \\
		& \qquad + \left( 1 + \frac{\alpha}{16H} \right)^{H+1} C\eta^2 \sum_{t' = mH}^{t-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{16H} \right)^{H+1} D \eta^2 \sum_{t' = mH}^{t-1} \Lambda^{(t')}.
	\end{align*}
Recursively substituting the values till $mH$ gives us:
	\begin{align*}
		S^{(t)} & \leq   \left(1 - \frac{\alpha}{2} \right)  \left( 1 + \frac{\alpha}{16H} \right)^{2H} S^{(mH)} + A \left( 1 + \frac{\alpha}{16H} \right)^{2H}  \eta^2 \\
		& \qquad + \left( 1 + \frac{\alpha}{16H} \right)^{2H} C\eta^2 \sum_{t' = mH}^{t-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + \left( 1 + \frac{\alpha}{16H} \right)^{2H} D \eta^2 \sum_{t' = mH}^{t-1} \Lambda^{(t')}. 
	\end{align*}
	%where we have used the fact that $\left( 1 + \frac{\alpha}{64H} \right)^{t-1-t'} \leq ( 1+ \frac{\alpha}{16H})^{2H}$ for all $t' \in \{(m+1)H,\hdots,t-1\}$. 
	For $\alpha \leq 1$, we note that $\left( 1 + \frac{\alpha}{16H} \right)^{2H} \leq e^{\frac{\alpha}{8}} \leq 1 + \frac{\alpha}{4}$. Plugging this in the first term on the RHS and using $\left(1 - \frac{\alpha}{2} \right)\left(1 + \frac{\alpha}{4} \right)\leq \left(1 - \frac{\alpha}{4} \right)$, and using $\left( 1 + \frac{\alpha}{16H} \right)^{2H} \leq 1 + \frac{\alpha}{4} \leq 2$ in the rest of the terms gives us the following recursion equation for any $t \in [T]$:
	\begin{align} \label{lem14-eq1}
		S^{(t)} & \leq   \left(1 - \frac{\alpha}{4} \right)  S^{(mH)} + 2 A  \eta^2 
		+ 2 C\eta^2 \sum_{t' = mH}^{t-1} \bbE \verts{ \nabla f (\blx^{(t')}) }^2 + 2 D \eta^2 \sum_{t' = mH}^{t-1} \Lambda^{(t')} 
	\end{align}
	Unrolling the recursion equation in \eqref{lem14-eq1} for $S^{(mH)}$ till $0$, we get:
	\begin{align}\label{lem14-eq11}
		S^{(t)} & \leq   2 A  \eta^2  \sum_{j=0}^{m-1}  \left(1 - \frac{\alpha}{4} \right)^{j} 
		+ 2 C\eta^2  \sum_{j=0}^{t-1}  \left(1 - \frac{\alpha}{4} \right)^{\lfloor \frac{t-j}{H} \rfloor}  \bbE \verts{ \nabla f (\blx^{(j)}) }^2 \notag \\
		& \qquad + 2 D \eta^2 \sum_{j=0}^{t-1} \left(1 - \frac{\alpha}{4} \right)^{\lfloor \frac{t-j}{H} \rfloor}  \Lambda^{(j)}.
	\end{align}
	Note that $\sum_{j=0}^{m-1}  \left(1 - \frac{\alpha}{4} \right)^{j} \leq \frac{4}{\alpha}$. Using this and the bound $\left(1 - \frac{\alpha}{4} \right)^{\lfloor \frac{t-j}{H} \rfloor} \leq  2 \left( 1 - \frac{\alpha}{8H} \right)^{t-j}$ (which we show in Appendix~\ref{app:proof-similar-lem14}) into \eqref{lem14-eq11} gives us:
	\begin{align*}
		S^{(t)} & \leq   \frac{8A\eta^2}{\alpha} 
		+ 4 C\eta^2  \sum_{j=0}^{t-1}  \left(1 - \frac{\alpha}{8H} \right)^{t-j}  \bbE \verts{ \nabla f (\blx^{(j)}) }^2 + 4 D \eta^2 \sum_{j=0}^{t-1} \left(1 - \frac{\alpha}{8H} \right)^{t-j}  \Lambda^{(j)} 
	\end{align*}
	Taking summation from $t=0$ to $T-1$, we get:
	\begin{align} \label{lem14-eq2}
		\sum_{t=0}^{T-1} S^{(t)} & \leq   \frac{8A\eta^2}{\alpha} T
		+ 4 C\eta^2  \sum_{t=0}^{T-1} \sum_{j=0}^{t-1}  \left(1 - \frac{\alpha}{8H} \right)^{t-j}  \bbE \verts{ \nabla f (\blx^{(j)}) }^2 \notag \\
		& \qquad + 4 D \eta^2 \sum_{t=0}^{T-1} \sum_{j=0}^{t-1} \left(1 - \frac{\alpha}{8H} \right)^{t-j}  \Lambda^{(j)} \notag \\
		& \leq \frac{8A\eta^2}{\alpha} T + 4C \eta^2 \sum_{j=0}^{T-1} \sum_{t=j+1}^{T-1}  \left(1 - \frac{\alpha}{8H} \right)^{t-j}  \bbE \verts{ \nabla f (\blx^{(j)}) }^2  + 4 D \eta^2 \sum_{j=0}^{T-1} \sum_{t=j+1}^{T-1} \left(1 - \frac{\alpha}{8H} \right)^{t-j}  \Lambda^{(j)} \notag \\
		& \leq \frac{8A\eta^2}{\alpha} T + \frac{32C \eta^2 H}{\alpha} \sum_{t=0}^{T-1}  \bbE \verts{ \nabla f (\blx^{(t)}) }^2  + \frac{32 D H \eta^2}{\alpha} \sum_{t=0}^{T-1}  \Lambda^{(t')} 
	\end{align}
	To bound the last term in the RHS of \eqref{lem14-eq2}, from the definition of $\Lambda^{(t')}$ in \eqref{eq:bound_v}, note that:
	\begin{align*}
		\sum_{t=0}^{T-1}  \Lambda^{(t')}  = \sum_{t=0}^{T-1} \sum_{j=0}^{t} \beta^{t-j} \bbE \verts{\nabla \bF(\bX^{(j)},\boldsymbol{\xi}^{(j)})}_F^2
	\end{align*}
	From Proposition \ref{prop:mom-update-norm} (from page~\pageref{prop:mom-update-norm}) to bound the stochastic gradient in the RHS of above equation gives us:
	\begin{align*}
		\sum_{t=0}^{T-1}  S^{(t')}  &\leq \sum_{t=0}^{T-1} \sum_{j=0}^{t} \beta^{t-j} \left[ 2(M^2+1)\(L^2\Xi^{(j)} + nG^2+nB^2\bbE\verts{\nabla f(\blx^{(j)})}_2^2\) + n\sigma^2 \right] \\
		& \leq \frac{2(M^2+1)nG^2 + n \sigma^2}{(1-\beta)} T + \frac{2(M^2+1)L^2}{(1-\beta)} \sum_{t=0}^{T-1} \Xi^{(t)} + \frac{2(M^2+1)nB^2}{(1-\beta)} \sum_{t=0}^{T-1} \bbE\verts{\nabla f(\blx^{(t)})}_2^2
	\end{align*}
	Substituting the above bound in \eqref{lem14-eq2}, we have:
	\begin{align*}
		\sum_{t=0}^{T-1} S^{(t)} & \leq \eta^2 \left(\frac{8A\eta^2}{\alpha} + \left( \frac{32 D H}{\alpha} \right)  \left( \frac{2(M^2+1)nG^2 + n \sigma^2}{(1-\beta)}   \right)   \right)T  \\
		& \quad + \eta^2 \left(\frac{32C  H}{\alpha}   + \left( \frac{32 D H }{\alpha} \right) \frac{2(M^2+1)nB^2}{(1-\beta)}   \right) \sum_{t=0}^{T-1}  \bbE \verts{ \nabla f (\blx^{(t)}) }^2 \\
		&   \quad + \frac{64 D H (M^2+1)L^2\eta^2 }{\alpha(1-\beta)}  \sum_{t=0}^{T-1}  \Xi^{(t)} 
	\end{align*}
	Choose $\eta \leq \sqrt{ \frac{  \alpha (1-\beta) }{128 D H (M^2+1)L^2}}$ and using that fact that $\Xi^{(t)} \leq S^{(t)}$ for all $t \in [T]$ and rearranging the summation term gives:
	\begin{align}\label{upper-bound-avg-St}
		\frac{1}{T}\sum_{t=0}^{T-1} S^{(t)} & \leq 2\eta^2 J_1 + 2\eta^2 J_2 \frac{1}{T}\sum_{t=0}^{T-1}  \bbE \verts{ \nabla f (\blx^{(t)}) }^2,
	\end{align}
	where $J_1= \left(\frac{8A\eta^2}{\alpha} + \left( \frac{32 D H}{\alpha} \right)  \left( \frac{2(M^2+1)nG^2 + n \sigma^2}{(1-\beta)}   \right)   \right)$ and $J_2=\left(\frac{32C  H}{\alpha}   + \left( \frac{32 D H }{\alpha} \right) \frac{2(M^2+1)nB^2}{(1-\beta)}   \right)$.
	
%	Choosing $\eta \leq ?? $\TODO{VALUE DECIDED BY RESULT OF LEMMA 11} completes the proof of Lemma.























}








==> suppl_experiments.tex <==
\section{Additional Experiments} \label{suppl_experiments}
In this section, we provide experimental results for comparison of our algorithm SQuARM-SGD to CHOCO-SGD \cite{koloskova_decentralized_2019} and vanilla-SGD for CIFAR-10 dataset \cite{cifar} (along with wall-clock time comparison), and for MNIST dataset to optimize a convex objective. In Subsection \ref{suppl_cifar_acc}, we describe the setup for training on CIFAR-10 dataset, and compare schemes based on their training performance and test-accuracy vs. communication trade-off. Subsection \ref{suppl_cifar_time} provides comparison for wall-clock time when training on CIFAR-10 dataset with a rate-limited communication pipeline between the worker nodes. This is typically the case in edge computing applications where efficient decentralized learning is desired, as significant communication rate (bandwidth) constraints may exist which cause the communication time itself to be a bottleneck.   
Lastly, Subsection \ref{suppl_mnist_acc} provides comparison plots for performance on MNIST dataset for a convex objective.

% {\bf Wall-clock time comparison}
%An important application for efficient decentralized learning arises in edge computing applications which may have significant communication rate (bandwidth) constraints. Typical hardware processors used in large scale learning tasks have a clock speed in GHz, while the allowable communication rate in such settings may be much lower. For example, the average cellular LTE rate is within 1-5 Mbps, which is orders below in magnitude from the computation rate, thus posing the communication time itself as the major bottleneck. Thus, such settings call for need of schemes which are highly communication efficient to save on communication time over bandlimited channels. 


\subsection{Experiments on CIFAR-10 dataset} \label{suppl_cifar_acc}


{\bf Setup.}
We match the setting in CHOCO-SGD \cite{koloskova_decentralized_2019} and perform our experiments on the CIFAR-10 \cite{cifar} dataset and train a ResNet20 \cite{wen2016learning} model with $n=8$ nodes connected in a ring topology. The training is done on TitanRTX GPUs. Learning rate is initialized to $0.1$, following a schedule consisting of a warmup period of 5 epochs followed by piecewise decay of 5 at epoch 200 and 300 and we stop training at epoch 400. The SGD algorithm is implemented with momentum with a factor of 0.9 and mini-batch size of 256. 
SQuARM-SGD consists of $H=5$ local iterations followed by checking for a triggering condition, and then communicating with the composed $SignTopK$ operator, where we take top 1\% elements of each tensor and only transmit the sign and norm of the result. The triggering threshold follows a schedule piecewise constant: initialized to 2.5 and increases by 1.5 after every 20 epochs till 350 epochs are complete; while maintaining that $c_t < \nicefrac{1}{\eta}$ for all $t$. We compare performance of SQuARM-SGD against CHOCO-SGD with $Sign$, $TopK$ compression (taking top 1\% of elements of the tensor) and decentralized vanilla SGD \cite{lian2017can}. 
We also provide a plot for using the composed $SignTopK$ operator without event-triggering titled `SQuARM-SGD (Sign-TopK)' for comparison. 




\begin{figure}[H]
	\subfigure[] { \label{fig:lo-noncvx} \includegraphics[scale=0.45]{suppl_noncvx_loss.png}} \hfill
	\subfigure[] { \label{fig:te-logbits-noncvx} \includegraphics[scale=0.45]{suppl_noncvx_tacc-logtotalbits.png}} \hfill
%	\subfigure[] { \label{fig:lo-time-noncvx} \includegraphics[scale=0.45]{suppl_noncvx_loss_time-plots.png}} \hfill
%	\subfigure[] { \label{fig:te-time-noncvx} \includegraphics[scale=0.45]{suppl_noncvx_tacc_time-plots.png}}
	\caption{These plots are for training a ResNet20 model (non-convex objective) on the CIFAR-10 dataset. Figure~\ref{fig:lo-noncvx} and \ref{fig:te-logbits-noncvx} show training loss vs.\ epochs and Top-1 accuracy vs.\ total number of bits communicated, respectively. 
%		In Figure~\ref{fig:lo-time-noncvx} and Figure~\ref{fig:te-time-noncvx}, we compare training loss vs time (in sec) and Top-1 accuracy vs time (in sec) respectively for the different schemes. 
	}
	\label{fig:figures_suppl_noncvx}
\end{figure}



{\bf Results.}
We plot the global loss function evaluated at the average parameter vector across nodes in Figure \ref{fig:lo-noncvx}, where we observe SQuARM-SGD converging at a similar rate as CHOCO-SGD and vanilla decentralized SGD. Figure \ref{fig:te-logbits-noncvx} shows the performance for a given bit-budget, where we show the Top-1 test accuracy%
 \footnote{Here, Top-1 accuracy corresponds to the percentage of test examples for which the correct label is equal to the label considered most probable by the model.} as a function of the total number of bits communicated. For Top-1 test-accuracy of around 90\%, SQuARM requires about 40$\times$ less bits than CHOCO with $Sign$ or $TopK$ compression, and around 3K$\times$ less bits than vanilla decentralized SGD to achieve the same Top-1 accuracy. \\
 
 
 \subsection{Wall-clock time comparison for CIFAR-10 dataset with rate-limited communication} \label{suppl_cifar_time}
 
 \begin{figure}[H]
%	\subfigure[] { \label{fig:te-logbits-noncvx2}
% 	\includegraphics[scale=0.37]{suppl_noncvx_tacc-logtotalbits.png}} \hfill
 \subfigure[] { \label{fig:te-logbits-logcommtime}
	\includegraphics[scale=0.45]{suppl_noncvx_tacc-logcommtime.png}} \hfill
 	\subfigure[] { \label{fig:te-time-noncvx} \includegraphics[scale=0.45]{suppl_noncvx_tacc_time-plots.png}}
 	\caption{
% 		These plots are for training a ResNet20 model (non-convex objective) on the CIFAR-10 dataset. 
 	Figure~\ref{fig:te-logbits-logcommtime} shows Top-1 accuracy as a function of total communication time through a bandlimited rate pipe of 100Kbps.
 	 Figure~\ref{fig:te-time-noncvx} shows the total time (computation + communication) required to reach a target Top-1 accuracy of $90$\% for the different schemes. 
 }
 	\label{fig:figures_suppl_noncvx2}
 \end{figure}
 

 
  {\bf Setup.} We follow the same setup as stated in the Subsection \ref{suppl_cifar_acc}, and further we assume that the communication between workers is rate-limited to 100Kbps. This is typical {\em average} rate of wireless edge devices sharing a common bandwidth with other devices, therefore devices cannot have sustained high rates.
 
 {\bf Results.}
 Figure~\ref{fig:te-logbits-logcommtime} shows the Top-1 accuracy as a function of time required to communicate bits through a rate pipe constrained to 100Kbps. We observe that, to reach a target accuracy of $90$\%, SQuARM-SGD saves a factor of around $40 \times$ in communication time compared to CHOCO-SGD with $Sign$ or $TopK$ sparsifier, and around  $3$K$\times$ less communication time than vanilla SGD. Thus, there is a significant saving in communication time for SQuARM-SGD compared to other schemes when communicating over typical rate limited channels.
This result is almost a direct translation of the savings in the number of bits needed for training.

 
In Figure~\ref{fig:te-time-noncvx}, we plot Top-1 accuracy vs.\ the wall-clock time, when the communication between workers is over the rate-limited pipelines (limited to 100Kbps). The wall-clock time includes the total time taken in both computation and communication; note that this includes time required to setup the communication (\emph{e.g.,} interrupts in processing) and other overheads, and not just the airtime (time to transmit the bits) for the communication as done in Figure~\ref{fig:te-logbits-logcommtime}. We observe that, to reach a target test-accuracy of around $90$\%, SQuARM-SGD saves a factor of around $30 \times$ in total time compared to CHOCO-SGD with $Sign$ or $TopK$ compression, and around 2.5K$\times$ compared to vanilla-SGD. 
The significant advantage to our method comes due to efficient transmission over the rate constrained pipeline.

Note that one can expect uncompressed schemes to do better in terms of computation time, but as shown in the plots above, the high communication time required in uncompressed schemes on rate-constrained links would far outweigh the advantage due to computation time. As a result, the total time required by SQuARM-SGD (that incorporates compression and infrequent communication) to reach a certain accuracy would be significantly smaller than either the uncompressed schemes or the ones using infrequent communication or both. 
 
 




\subsection{Experiments for convex objective on MNIST dataset} \label{suppl_mnist_acc}
\begin{figure}[ht]
	\centering
	\subfigure[] { \label{fig:lo-cvx} \includegraphics[scale=0.45]{suppl_cvx_testerr.png}} \hfill
	\subfigure[] { \label{fig:te-logbits-cvx} \includegraphics[scale=0.45]{suppl_cvx_testerr_logbits.png}}
	\caption{Figure \ref{fig:lo-cvx} and \ref{fig:te-logbits-cvx} are for convex objective simulated on the MNIST dataset, where we plot test error vs number of communication rounds and test error vs total number of bits communicated, respectively, for different algorithms.}
	\label{fig:figures_suppl_cvx}
\end{figure}
{\bf Setup.}
We run SQuARM-SGD on MNIST dataset and use multi-class cross-entropy loss to model the local objectives $f_i, i\in[n]$. We consider $n=60$ nodes connected in a ring topology, each processing a mini-batch size of 5 per iteration and having heterogeneous distribution of data across classes. We work with $\eta_t = 1/(t+100)$ (based on grid search) and synchronization index $H=5$. For SQuARM-SGD, we use the composed operator $SignTopK$ (\cite{basu_qsparse-local-sgd:_2019}) with $k=10$ (out of 7840 length vector for MNIST dataset)
For our experiments, we set the triggering constant $c_0 = 5000$ in SQuARM-SGD (line 7) and keep it unchanged until a certain number of iterations and then increase it periodically;
while still maintaining that $c_t \eta_t^2$ decreases with $t$ (as $c_t$ is  $o(t)$ ) .




{\bf Results.}
In Figure \ref{fig:lo-cvx}, we observe SQuARM-SGD can reach a target test error in fewer communication rounds while converging at a rate similar to that of vanilla SGD. The advantage to SQuARM-SGD comes from the significant savings in the number of bits communicated to achieve a desired test error, as seen in Figure \ref{fig:te-logbits-cvx}: to achieve a test error of around 0.12, SQuARM-SGD gets 120$\times$ savings as compared to CHOCO-SGD with $Sign$ quantizer, around 10-15$\times$ savings than CHOCO-SGD with $TopK$ sparsifier, and around 1000$\times$ savings than vanilla decentralized SGD.
